Higgs-Boson Masses and Mixing Matrices in the NMSSM: Analysis of On-Shell Calculations

We analyze the Higgs-boson masses and mixing matrices in the NMSSM based on an on-shell (OS) renormalization of the gauge-boson and Higgs-boson masses and the parameters of the top/scalar top sector. We compare the implementation of the OS calculations in the codes NMSSMCALC and NMSSM-FeynHiggs up to $\mathcal{({\alpha}_t{\alpha}_s)}$. We identify the sources of discrepancies at the one- and at the two-loop level. Finally we compare the OS and $\overline{\text{DR}}$ evaluation as implemented in NMSSMCALC. The results are important ingredients for an estimate of the theoretical precision of Higgs-boson mass calculations in the NMSSM.

==> plots/gnuScript <==
set terminal pdf enhanced linewidth 3.5 size 10,6
# font arial 21 size 900,675
# Make the x axis labels easier to read.
set xtics rotate out
# Select histogram data
set style data histogram
# Give the bars a plain fill pattern, and draw a solid line around them.
set style fill solid border
set style histogram clustered
# plot [-1:5][120:135] for [COL=2:4:1] 'dummy.dat' using COL:xticlabels(1) title columnheader

# -------------------- example statement --------------------------

# set terminal pdf enhanced linewidth 3.5 size 10,6
# set xtics rotate out
# set style data histogram
# set style fill solid border
# set style histogram clustered


# set size 1,1
# set output "total_sm.pdf"
# set title "SM-like Higgs" font ",30"
# set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
# set xlabel font ",25"
# set xtics font ", 25" rotate by 0
# set ytics font ", 25" 0,0.5
# set key samplen 4.25 spacing 5.5 top right font ",30"
# plot [0:6][0:6.5] \
#      'smHiggsMaster.dat' using (($3-$7)):xticlabels(2) title	\
#      			 "{Q = M_S}" lt rgb "#33a02c", 		\
#      'smHiggsMaster.dat' using (($4-$8)):xticlabels(2) title	\
#      			 "{Q = m_t}" lt rgb "#1f78b4", 		\


#a6cee3
#1f78b4
#b2df8a
#33a02c

# --------------------------- total -------------------------------

set size 1,1
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set lmargin 16
set bmargin 3.5
set xlabel font ",35"
set xtics font ", 40" rotate by 0 offset 2.5,-1. scale 0
set mytics 4
set ytics font ", 35" 0,1.0
set title font ",40" offset 0,1
set key font ",40"



set output "total_sm.pdf"
set title "SM-like Higgs"
set key samplen 4.25 spacing 8.0 top right
plot [0.5:5.5][0:6.5] \
     'smHiggsMaster.dat' using (($3-$7)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (($4-$8)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     # 			 "{\"out-of-the-box\" {m_t}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {Q_S}" lt rgb "#b2df8a",		\
     # 'smHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {m_t}" lt rgb "#a6cee3"


set output "total_singlet.pdf"
set title "singlet-like Higgs"
set xzeroaxis linewidth 2.5
set ytics font ", 35" -10,0.5
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [0.5:5.5][-0.5:2.] \
     'singletMaster.dat' using (($3-$7)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (($4-$8)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\
     # 'singletMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     # 			 "{\"out-of-the-box\" {m_t}}" lt rgb "#1f78b4",	\
     # 'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {Q_S}" lt rgb "#b2df8a",		\
     # 'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {m_t}" lt rgb "#a6cee3"


set output "total_heavy.pdf"
set title "heavy Higgs"
set xzeroaxis linewidth 2.5
set ylabel "{/Symbol D}m/GeV"
set ytics font ", 35" -10,0.25
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [0.5:5.5][-0.25:2.] \
     'heavyHiggsMaster.dat' using (($3-$7)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (($4-$8)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\
     # 'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     # 			 "{\"out-of-the-box\" {m_t}}" lt rgb "#1f78b4",	\
     # 'heavyHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {Q_S}" lt rgb "#b2df8a",		\
     # 'heavyHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {m_t}" lt rgb "#a6cee3"


set output "asMod_sm.pdf"
set title "SM-like Higgs"
set xzeroaxis linewidth 2.5
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [1.5:5.5][-0.6:1.25] \
     'smHiggsMaster.dat' using (($5-$9)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (($6-$10)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\

set output "asMod_sg.pdf"
set title "singlet-like Higgs"
set xzeroaxis linewidth 2.5
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 bottom left reverse Left
plot [1.5:5.5][-0.75:0.25] \
     'singletMaster.dat' using (($5-$9)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (($6-$10)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\

set output "asMod_hy.pdf"
set title "heavy Higgs"
set xzeroaxis linewidth 2.5
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [1.5:5.5][-0.3:0.5] \
     'heavyHiggsMaster.dat' using (($5-$9)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (($6-$10)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\



# --------------------------- approx -------------------------------

set size 1,1
set output "approx_sm.pdf"
set title "SM-like Higgs" font ",30"
set ylabel "{/Symbol D}m/GeV" font ",30"
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set key samplen 4.25 spacing 7.5 at 2,1.45 font ",30"
plot [0:6][0:1.5] \
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=M_S}" lt rgb "#33a02c",		\
     'smHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title				\
     			 "{{/Symbol D}m_h^{2L}m Q=M_S}" lt rgb "#b2df8a",		\
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=m_t}" lt rgb "#1f78b4",		\
     'smHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{2L}, Q=m_t}" lt rgb "#a6cee3"

set size 1,1
set output "approx_singlet.pdf"
set title "singlet-like Higgs" font ",30"
set ylabel "{/Symbol D}m/GeV" font ",30"
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set key samplen 4.25 spacing 7.5 at 2,1.2 font ",30"
plot [0:6][0:1.3] \
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=M_S}" lt rgb "#33a02c",		\
     'singletMaster.dat' using (abs($5-$9)):xticlabels(2) title				\
     			 "{{/Symbol D}m_h^{2L}m Q=M_S}" lt rgb "#b2df8a",		\
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=m_t}" lt rgb "#1f78b4",		\
     'singletMaster.dat' using (abs($6-$10)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{2L}, Q=m_t}" lt rgb "#a6cee3"

set size 1,1
set output "approx_heavy.pdf"
set title "heavy-like Higgs" font ",30"
set ylabel "{/Symbol D}m/GeV" font ",30"
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set key samplen 4.25 spacing 7.5 at 3,1.45 font ",30"
plot [0:6][0:1.5] \
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=M_S}" lt rgb "#33a02c",		\
     'heavyHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title				\
     			 "{{/Symbol D}m_h^{2L}m Q=M_S}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=m_t}" lt rgb "#1f78b4",		\
     'heavyHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{2L}, Q=m_t}" lt rgb "#a6cee3"




# --------------------------- repara -------------------------------


set output "repara_sm.pdf"
set title "SM-like Higgs"
set key top right
plot [0:6][0:1] \
     'smHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'smHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_singlet.pdf"
set title "Singlet-like Higgs"
set key top left
plot [0:6][0:1] \
     'singletMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'singletMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_heavy.pdf"
set title "Heavy Higgs"
set key top left
plot [0:6][0:1.5] \
     'heavyHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'heavyHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"


# --------------------------- appr -------------------------------

set output "appr_sm.pdf"
set key top right
plot [0:6][0:7] \
     'smHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'smHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_singlet.pdf"
set key top left
plot [0:6][0:2] \
     'singletMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'singletMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_heavy.pdf"
set key top left
plot [0:6][0:2] \
     'heavyHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'heavyHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"




# --------------------------- OSvsRbar -------------------------------


set size 1,1
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set lmargin 16
set bmargin 3.5
set xlabel font ",35"
set xtics font ", 40" rotate by 0 offset 2.5,-1. scale 0
set mytics 4
set ytics font ", 35" 0,1.0
set title font ",40" offset 0,1
set key font ",40"


set output "OSvsDRbar_sm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set mytics 5
set ytics font ", 35" 0,0.5
set key samplen 4.25 spacing 8.0 at 2.5,2.0 font ",40"
plot [1.5:5.5][0:2] \
     'smHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'smHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_sg.pdf"
set title "Singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set mytics 5
set ytics font ", 35" 0,0.25
set key samplen 4.25 spacing 8.0 at 1.6,1.25 font ",40"
plot [1.5:5.5][0:1.25] \
     'singletMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "  {Q=M_S}" lt rgb "#33a02c", \
     'singletMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "  {Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_hy.pdf"
set title "Heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set mytics 5
set ytics font ", 35" 0,0.25
set key samplen 4.25 spacing 8.0 at 1.6,0.75 font ",40"
plot [1.5:5.5][0:0.75] \
     'heavyHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'heavyHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"


# --------------------------- repara 1L -------------------------------


set output "repara_sm_1L.pdf"
set key top right
plot [0:6][0:2] \
     'smHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'smHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_singlet_1L.pdf"
set key top right
plot [0:6][0:2] \
     'singletMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'singletMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_heavy_1L.pdf"
set key top right
plot [0:6][0:2] \
     'heavyHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'heavyHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"


# --------------------------- repara Loop -------------------------------

set output "repara_sm_i.pdf"
set key top left
plot [0:6][0:1.1] \
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'smHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'smHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_singlet_i.pdf"
set key top left
plot [0:6][0:1] \
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'singletMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'singletMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_heavy_i.pdf"
set key top left
plot [0:6][0:0.5] \
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'heavyHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'heavyHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\


set output "repara_sm_ii.pdf"
set key top left
plot [0:6][0:1.5] \
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'smHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'smHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_singlet_ii.pdf"
set key top left
plot [0:6][0:1.2] \
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'singletMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'singletMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_heavy_ii.pdf"
set key top left
plot [0:6][0:1.6] \
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'heavyHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'heavyHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\


# --------------------------- MSSM-limit -------------------------------

set output "total_sm_mssm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set xzeroaxis linewidth 2.5
# set key top left reverse Left
set key at 1.2,-0.5 font ",30" spacing 5 samplen 7

plot [0:6][-1.2:1.2] \
     'smHiggsMaster.dat' using ($13-$15):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using ($5-$7):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'smHiggsMaster.dat' using ($14-$16):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"

set output "total_singlet_mssm.pdf"
set title "singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][-1.2:1.2] \
     'singletMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'singletMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"



set output "total_heavy_mssm.pdf"
set title "heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key at 1.2,0.7 font ",30" spacing 5 samplen 7
plot [0:6][-0.8:0.7] \
     'heavyHiggsMaster.dat' using ($13-$15):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using ($5-$7):xticlabels(2) title	\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster.dat' using ($14-$16):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'heavyHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"


# ---------------------- dedicated charge --------------------------------------

# set size 1,1
# set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
# set lmargin 16
# set bmargin 3.5
# set xlabel font ",35"
# set xtics font ", 40" rotate by 0 offset 2.5,-1. scale 0
# set mytics 4
# set ytics font ", 35" 0,1.0
# set title font ",40" offset 0,1
set key font ",40"

set ytics font ", 35"
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set xtics font ", 40" rotate by 0 offset 4,-1. scale 0


set output "1L_sm.pdf"
set size 1,1
set title "SM-like Higgs" font ",40"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 0.6,-0.45 Left reverse
plot [0.5:4.5][-1.8:1.5] \
     'smHiggsMaster1L.dat' using ($3-$5):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = M_S}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$7):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = M_S}" lt rgb "#33a02c",	\
     '' 		   using ($4-$6):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = m_t}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$8):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = m_t}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\


set output "1L_sm_mssm.pdf"
set title "SM-like Higgs, 1-loop" font ",30"
set ytics 0.25
set mytics 2
set key samplen 4.25 spacing 5.5 at 0.6,-0.3 font ",30" 
plot [0:5][-1:1.25] \
     'smHiggsMaster1L.dat'							\
     			   using ($9-$11):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$5):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#33a02c",	\
     '' 		   using ($10-$12):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$6):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\



set output "2L_sm_mssm.pdf"
set key at -0.4,-0.3 font ",30" spacing 5 samplen 7
set title "SM-like Higgs, 2-loop"
plot [-1:4][-1:1.25] \
     'smRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\
     'smRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#a6cee3",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#1f78b4",	\


set output "1L_sg.pdf"
set title "singlet-like Higgs" font ",40"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 0.6,1. font ",40"
plot [0.5:4.5][-0.5:1.] \
     'singletMaster1L.dat'							\
     			   using ($3-$5):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = M_S}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$7):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = M_S}" lt rgb "#33a02c",	\
     '' 		   using ($4-$6):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = m_t}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$8):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = m_t}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\


set ytics font ", 35"
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set xtics font ", 40" rotate by 0 offset 4,-1. scale 0


set output "1L_hy.pdf"
set title "heavy Higgs" font ",40"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 0.6,1. font ",40" 
plot [0.5:4.5][-0.5:1.] \
     'heavyHiggsMaster1L.dat'							\
     			   using ($3-$5):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = M_S}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$7):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = M_S}" lt rgb "#33a02c",	\
     '' 		   using ($4-$6):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = m_t}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$8):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = m_t}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\




set output "1L_hy_mssm.pdf"
set title "heavy Higgs, 1-loop" font ",30"
set ytics 0.25
set mytics 2
set key samplen 4.25 spacing 5.5 at 0.6,1.2 font ",30" 
plot [0:5][-0.6:1.25] \
     'heavyHiggsMaster1L.dat'							\
     			   using ($9-$11):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$5):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#33a02c",	\
     '' 		   using ($10-$12):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$6):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\

set output "2L_hy_mssm.pdf"
set key at -0.4,1.2 font ",30" spacing 5 samplen 7
set title "heavy Higgs, 2-loop"
plot [-1:4][-0.6:1.25] \
     'hyRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\
     'hyRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#a6cee3",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#1f78b4",	\






# --------------------------- apprRepa -------------------------------

set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
set xlabel font ",25"
set ytics -2,0.25,10
set xtics font ", 25" rotate by 0 
set ytics font ", 25"
set xzeroaxis linewidth 2.5

set output "1L2L_sm_ms.pdf"
set title "SM-like Higgs M_S"
set key at 0.5,1.2 font ",30" spacing 5 samplen 7
plot [0:5][-1.:1.25] \
     'resMZI.dat' using 2:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 5:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"


set output "1L2L_sm_mt.pdf"
set title "SM-like Higgs m_t"
set key at 0.5,1.2 font ",30" spacing 5 samplen 7
plot [0:5][-1.:1.25] \
     'resMZII.dat' using 2:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 5:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"





set output "1L2L_sg_ms.pdf"
set title "singlet-like Higgs M_S"
set key at 0.5,1.4 font ",30" spacing 5 samplen 7
plot [0:5][-1.25:1.5] \
     'resMZI.dat' using 3:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 6:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"

set output "1L2L_sg_mt.pdf"
set title "singlet-like Higgs m_t"
set key at 0.5,1.4 font ",30" spacing 5 samplen 7
plot [0:5][-1.25:1.5] \
     'resMZII.dat' using 3:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 6:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"




set output "1L2L_hy_ms.pdf"
set title "heavy Higgs M_S"
set key at 0.6,1.25 font ",30" spacing 5 samplen 7
plot [0:5][-1.5:1.25] \
     'resMZI.dat' using 4:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 7:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"

set output "1L2L_hy_mt.pdf"
set title "heavy Higgs m_t"
set key at 0.6,1.2 font ",30" spacing 5 samplen 7
plot [0:5][-1.5:1.25] \
     'resMZII.dat' using 4:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 7:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"


set key font ",40"
set title font ",40"

set ytics font ", 35"
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set xtics font ", 40" rotate by 0 offset 4,-1. scale 0


set output "1L2L_sm_short.pdf"
set title "SM-like Higgs" 
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 1.6,1. Left reverse
# set key at 0.6,1. font ",40" spacing 5 samplen 7
plot [1.5:5.5][-1:1.] \
     'resMZI.dat' using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} M_S}" lt rgb "#33a02c",	\
     'resMZII.dat' using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} m_t}" lt rgb "#1f78b4",	\


set output "1L2L_sg_short.pdf"
set title "singlet-like Higgs"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 1.6,-0.7 Left reverse
# set key at 0.7,1.25 font ",30" spacing 5 samplen 7
plot [1.5:5.5][-1.:0.25] \
     'resMZI.dat' using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} M_S}" lt rgb "#33a02c",	\
     'resMZII.dat' using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} m_t}" lt rgb "#1f78b4",	\


set output "1L2L_hy_short.pdf"
set title "heavy Higgs"
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 at 1.6,0.25 Left reverse
# set key at 1.6,0.25 font ",30" spacing 5 samplen 7
plot [1.5:5.5][-0.25:0.25] \
     'resMZI.dat' using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} M_S}" lt rgb "#33a02c",	\
     'resMZII.dat' using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} m_t}" lt rgb "#1f78b4",	\



set output "mssm_sm_ms.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "SM-like Higgs M_S"
plot [0:5][-0.8:1.] \
     'smRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\

set output "mssm_sm_mt.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "SM-like Higgs m_t"
plot [0:5][-0.8:1.] \
     'smRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\
     # 'smHiggsMasterNoTP1.dat' using ($13-$15):xticlabels(2) title 	\
     # 			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     # '' 		 using ($5-$7):xticlabels(2) title		\
     # 			 "{NMSSM}" lt rgb "#b2df8a",		\
     # 'res1L2LI.dat' 	 using ($5 - $6 + $2 - $3 ):xticlabels(1) title 	\
     # 			 "{NMSSM-rtet}" lt rgb "#33a02c",	\



















set output "mssm_hy_ms.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "heavy Higgs M_S"
plot [0:5][-0.8:1.25] \
     'hyRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\


# set output "mssm_hy_ms.pdf"
# set key at 0.5,0.75 font ",30" spacing 5 samplen 7
# set title "heavy Higgs M_S"
# plot [0:5][-0.5:0.75] \
#      'heavyHiggsMasterNoTP1.dat' using ($13-$15):xticlabels(2) title 	\
#      			 "{MSSM-limit}" lt rgb "#33a02c",	\
#      '' 		 using ($5-$7):xticlabels(2) title		\
#      			 "{NMSSM}" lt rgb "#b2df8a",		\

set output "mssm_hy_mt.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "heavy Higgs m_t"
plot [0:5][-0.8:1.25] \
     'hyRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\

# set output "mssm_hy_mt.pdf"
# set title "heavy Higgs m_t"
# plot [0:5][-0.5:0.75] \
#      'heavyHiggsMasterNoTP1.dat' using ($14-$16):xticlabels(2) title 	\
#      			 "{MSSM-limit}" lt rgb "#1f78b4",	\
#      '' 		 using ($6-$8):xticlabels(2) title 	\
#      			 "{NMSSM}" lt rgb "#a6cee3"






# ------------------------------------------------------------
# ------------------------------------------------------------

# --------------------- histograms ---------------------------


# set terminal pdf enhanced linewidth 3.5 size 10,6
set terminal pdf enhanced linewidth 3.5 size 7,4

set style data histogram
set style histogram columnstacked

set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"

# set linetype 1 lt rgb "#33a02c"
# set linetype 2 lt rgb "#1f78b4"

set style fill solid noborder
set boxwidth 0.75
set xzeroaxis linewidth 2.5


set output "diff_detail_sm.pdf"
set title "SM-like Higgs" font ",30"
# set key autotitle columnheader at 2.,-0.5 font ",30" spacing 5 samplen 7
# plot [0:8][-1:1]  \
#      'smDiffMasterI.dat'  using 3:key(1),\
#      'smDiffMasterII.dat' using 3,       \
#      'blank.dat'	  using 2,	 \
#      'smDiffMasterI.dat'  using 4,       \
#      'smDiffMasterII.dat' using 4,       \
#      'blank.dat'	  using 2,	 \
#      'smDiffMasterI.dat'  using 5,       \
#      'smDiffMasterII.dat' using 5,       \
#      'blank.dat'	  using 2,	 \
#      'smDiffMasterI.dat'  using 6,       \
#      'smDiffMasterII.dat' using 6

# set output "diff_detail_sm2.pdf"
# set title "SM-like Higgs" font ",30"
set key autotitle columnheader at 1.7,4 font ",30" spacing 5 samplen 7
plot [0:8][-2:4]  \
     'smMZI.dat'  using 3:key(1),	\
     'smMZII.dat' using 3,		\
     'blank.dat'  using 2,		\
     'smMZI.dat'  using 4,		\
     'smMZII.dat' using 4,		\
     'blank.dat'  using 2,		\
     'smMZI.dat'  using 5,		\
     'smMZII.dat' using 5,		\
     'blank.dat'  using 2,		\
     'smMZI.dat'  using 6,		\
     'smMZII.dat' using 6



set output "diff_detail_singlet.pdf"
set title "singlet-like Higgs" font ",30"
set key autotitle columnheader at 2,-3.0 font ",30" spacing 5 samplen 7
plot [0:8][-4.5:2]  \
     'singMZI.dat'  using 3:key(1),	\
     'singMZII.dat' using 3,		\
     'blank.dat'    using 2,		\
     'singMZI.dat'  using 4,		\
     'singMZII.dat' using 4,		\
     'blank.dat'    using 2,		\
     'singMZI.dat'  using 5,		\
     'singMZII.dat' using 5,		\
     'blank.dat'    using 2,		\
     'singMZI.dat'  using 6,		\
     'singMZII.dat' using 6

     # 'singDiffMasterI.dat'  using 3:key(1),\
     # 'singDiffMasterII.dat' using 3,       \
     # 'blank.dat'	    using 2,  	   \
     # 'singDiffMasterI.dat'  using 4,       \
     # 'singDiffMasterII.dat' using 4,       \
     # 'blank.dat'	    using 2,  	   \
     # 'singDiffMasterI.dat'  using 5,       \
     # 'singDiffMasterII.dat' using 5,       \
     # 'blank.dat'	    using 2,       \
     # 'singDiffMasterI.dat'  using 6,       \
     # 'singDiffMasterII.dat' using 6



set output "diff_detail_heavy.pdf"
set title "heavy Higgs" font ",30"
set key autotitle columnheader at 2,-0.6 font ",30" spacing 5 samplen 7
plot [0:8][-1.5:3.]  \
     'heavyMZI.dat'  using 3:key(1),	\
     'heavyMZII.dat' using 3,		\
     'blank.dat'     using 2,		\
     'heavyMZI.dat'  using 4,		\
     'heavyMZII.dat' using 4,		\
     'blank.dat'     using 2,		\
     'heavyMZI.dat'  using 5,		\
     'heavyMZII.dat' using 5,		\
     'blank.dat'     using 2,		\
     'heavyMZI.dat'  using 6,		\
     'heavyMZII.dat' using 6

     # 'heavyDiffMasterI.dat'  using 3:key(1),\
     # 'heavyDiffMasterII.dat' using 3,       \
     # 'blank.dat'	     using 2,       \
     # 'heavyDiffMasterI.dat'  using 4,       \
     # 'heavyDiffMasterII.dat' using 4,       \
     # 'blank.dat'	     using 2,       \
     # 'heavyDiffMasterI.dat'  using 5,       \
     # 'heavyDiffMasterII.dat' using 5,       \
     # 'blank.dat'	     using 2,       \
     # 'heavyDiffMasterI.dat'  using 6,       \
     # 'heavyDiffMasterII.dat' using 6


     # 'heavyDiffMasterI.dat'  using 2:key(1),\
     # 'heavyDiffMasterII.dat' using 2,       \
     # 'blank.dat'	       using 2,       \
     



# ------------------------------------------------------------


==> plots/gnuScript_ <==
set terminal pdf enhanced linewidth 3.5 size 10,6
# font arial 21 size 900,675
# Make the x axis labels easier to read.
set xtics rotate out
# Select histogram data
set style data histogram
# Give the bars a plain fill pattern, and draw a solid line around them.
set style fill solid border
set style histogram clustered
# plot [-1:5][120:135] for [COL=2:4:1] 'dummy.dat' using COL:xticlabels(1) title columnheader

# -------------------- example statement --------------------------

# set terminal pdf enhanced linewidth 3.5 size 10,6
# set xtics rotate out
# set style data histogram
# set style fill solid border
# set style histogram clustered


# set size 1,1
# set output "total_sm.pdf"
# set title "SM-like Higgs" font ",30"
# set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
# set xlabel font ",25"
# set xtics font ", 25" rotate by 0
# set ytics font ", 25" 0,0.5
# set key samplen 4.25 spacing 5.5 top right font ",30"
# plot [0:6][0:6.5] \
#      'smHiggsMaster.dat' using (($3-$7)):xticlabels(2) title	\
#      			 "{Q = M_S}" lt rgb "#33a02c", 		\
#      'smHiggsMaster.dat' using (($4-$8)):xticlabels(2) title	\
#      			 "{Q = m_t}" lt rgb "#1f78b4", 		\


#a6cee3
#1f78b4
#b2df8a
#33a02c

# --------------------------- total -------------------------------

set size 1,1
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set lmargin 16
set bmargin 3.5
set xlabel font ",35"
set xtics font ", 40" rotate by 0 offset 2.5,-1. scale 0
set mytics 4
set ytics font ", 35" 0,1.0
set title font ",40" offset 0,1
set key font ",40"



set output "total_sm.pdf"
set title "SM-like Higgs"
set key samplen 4.25 spacing 8.0 top right
plot [0.5:5.5][0:6.5] \
     'smHiggsMaster.dat' using (($3-$7)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (($4-$8)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     # 			 "{\"out-of-the-box\" {m_t}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {Q_S}" lt rgb "#b2df8a",		\
     # 'smHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {m_t}" lt rgb "#a6cee3"


set output "total_singlet.pdf"
set title "singlet-like Higgs"
set xzeroaxis linewidth 2.5
set ytics font ", 35" -10,0.5
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [0.5:5.5][-0.5:2.] \
     'singletMaster.dat' using (($3-$7)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (($4-$8)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\
     # 'singletMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     # 			 "{\"out-of-the-box\" {m_t}}" lt rgb "#1f78b4",	\
     # 'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {Q_S}" lt rgb "#b2df8a",		\
     # 'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {m_t}" lt rgb "#a6cee3"


set output "total_heavy.pdf"
set title "heavy Higgs"
set xzeroaxis linewidth 2.5
set ylabel "{/Symbol D}m/GeV"
set ytics font ", 35" -10,0.25
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [0.5:5.5][-0.25:2.] \
     'heavyHiggsMaster.dat' using (($3-$7)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (($4-$8)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\
     # 'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     # 			 "{\"out-of-the-box\" {m_t}}" lt rgb "#1f78b4",	\
     # 'heavyHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {Q_S}" lt rgb "#b2df8a",		\
     # 'heavyHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     # 			 "{/Symbol a}_s mod {m_t}" lt rgb "#a6cee3"


set output "asMod_sm.pdf"
set title "SM-like Higgs"
set xzeroaxis linewidth 2.5
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [1.5:5.5][-0.5:1.25] \
     'smHiggsMaster.dat' using (($5-$9)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (($6-$10)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\

set output "asMod_sg.pdf"
set title "singlet-like Higgs"
set xzeroaxis linewidth 2.5
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 bottom left reverse Left
plot [1.5:5.5][-0.75:0.25] \
     'singletMaster.dat' using (($5-$9)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (($6-$10)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\

set output "asMod_hy.pdf"
set title "heavy Higgs"
set xzeroaxis linewidth 2.5
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 top left reverse Left
plot [1.5:5.5][-0.3:0.5] \
     'heavyHiggsMaster.dat' using (($5-$9)):xticlabels(2) title			\
     			 "{Q = M_S}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (($6-$10)):xticlabels(2) title 		\
     			 "{Q = m_t}" lt rgb "#1f78b4",	\



# --------------------------- approx -------------------------------

set size 1,1
set output "approx_sm.pdf"
set title "SM-like Higgs" font ",30"
set ylabel "{/Symbol D}m/GeV" font ",30"
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set key samplen 4.25 spacing 7.5 at 2,1.45 font ",30"
plot [0:6][0:1.5] \
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=M_S}" lt rgb "#33a02c",		\
     'smHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title				\
     			 "{{/Symbol D}m_h^{2L}m Q=M_S}" lt rgb "#b2df8a",		\
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=m_t}" lt rgb "#1f78b4",		\
     'smHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{2L}, Q=m_t}" lt rgb "#a6cee3"

set size 1,1
set output "approx_singlet.pdf"
set title "singlet-like Higgs" font ",30"
set ylabel "{/Symbol D}m/GeV" font ",30"
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set key samplen 4.25 spacing 7.5 at 2,1.2 font ",30"
plot [0:6][0:1.3] \
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=M_S}" lt rgb "#33a02c",		\
     'singletMaster.dat' using (abs($5-$9)):xticlabels(2) title				\
     			 "{{/Symbol D}m_h^{2L}m Q=M_S}" lt rgb "#b2df8a",		\
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=m_t}" lt rgb "#1f78b4",		\
     'singletMaster.dat' using (abs($6-$10)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{2L}, Q=m_t}" lt rgb "#a6cee3"

set size 1,1
set output "approx_heavy.pdf"
set title "heavy-like Higgs" font ",30"
set ylabel "{/Symbol D}m/GeV" font ",30"
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set key samplen 4.25 spacing 7.5 at 3,1.45 font ",30"
plot [0:6][0:1.5] \
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=M_S}" lt rgb "#33a02c",		\
     'heavyHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title				\
     			 "{{/Symbol D}m_h^{2L}m Q=M_S}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{1L}, Q=m_t}" lt rgb "#1f78b4",		\
     'heavyHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title			\
     			 "{{/Symbol D}m_h^{2L}, Q=m_t}" lt rgb "#a6cee3"




# --------------------------- repara -------------------------------


set output "repara_sm.pdf"
set title "SM-like Higgs"
set key top right
plot [0:6][0:1] \
     'smHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'smHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_singlet.pdf"
set title "Singlet-like Higgs"
set key top left
plot [0:6][0:1] \
     'singletMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'singletMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_heavy.pdf"
set title "Heavy Higgs"
set key top left
plot [0:6][0:1.5] \
     'heavyHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'heavyHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"


# --------------------------- appr -------------------------------

set output "appr_sm.pdf"
set key top right
plot [0:6][0:7] \
     'smHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'smHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_singlet.pdf"
set key top left
plot [0:6][0:2] \
     'singletMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'singletMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_heavy.pdf"
set key top left
plot [0:6][0:2] \
     'heavyHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'heavyHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"




# --------------------------- OSvsRbar -------------------------------


set size 1,1
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set lmargin 16
set bmargin 3.5
set xlabel font ",35"
set xtics font ", 40" rotate by 0 offset 2.5,-1. scale 0
set mytics 4
set ytics font ", 35" 0,1.0
set title font ",40" offset 0,1
set key font ",40"


set output "OSvsDRbar_sm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set mytics 5
set ytics font ", 35" 0,0.5
set key samplen 4.25 spacing 8.0 at 2.5,2.0 font ",40"
plot [1.5:5.5][0:2] \
     'smHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'smHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_sg.pdf"
set title "Singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set mytics 5
set ytics font ", 35" 0,0.25
set key samplen 4.25 spacing 8.0 at 1.6,1.25 font ",40"
plot [1.5:5.5][0:1.25] \
     'singletMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "  {Q=M_S}" lt rgb "#33a02c", \
     'singletMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "  {Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_hy.pdf"
set title "Heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set mytics 5
set ytics font ", 35" 0,0.25
set key samplen 4.25 spacing 8.0 at 1.6,0.75 font ",40"
plot [1.5:5.5][0:0.75] \
     'heavyHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'heavyHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"


# --------------------------- repara 1L -------------------------------


set output "repara_sm_1L.pdf"
set key top right
plot [0:6][0:2] \
     'smHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'smHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_singlet_1L.pdf"
set key top right
plot [0:6][0:2] \
     'singletMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'singletMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_heavy_1L.pdf"
set key top right
plot [0:6][0:2] \
     'heavyHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'heavyHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"


# --------------------------- repara Loop -------------------------------

set output "repara_sm_i.pdf"
set key top left
plot [0:6][0:1.1] \
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'smHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'smHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_singlet_i.pdf"
set key top left
plot [0:6][0:1] \
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'singletMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'singletMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_heavy_i.pdf"
set key top left
plot [0:6][0:0.5] \
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'heavyHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'heavyHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\


set output "repara_sm_ii.pdf"
set key top left
plot [0:6][0:1.5] \
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'smHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'smHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_singlet_ii.pdf"
set key top left
plot [0:6][0:1.2] \
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'singletMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'singletMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_heavy_ii.pdf"
set key top left
plot [0:6][0:1.6] \
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'heavyHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'heavyHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\


# --------------------------- MSSM-limit -------------------------------

set output "total_sm_mssm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"
set xzeroaxis linewidth 2.5
# set key top left reverse Left
set key at 1.2,-0.5 font ",30" spacing 5 samplen 7

plot [0:6][-1.2:1.2] \
     'smHiggsMaster.dat' using ($13-$15):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using ($5-$7):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'smHiggsMaster.dat' using ($14-$16):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"

set output "total_singlet_mssm.pdf"
set title "singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][-1.2:1.2] \
     'singletMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'singletMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"



set output "total_heavy_mssm.pdf"
set title "heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key at 1.2,0.7 font ",30" spacing 5 samplen 7
plot [0:6][-0.8:0.7] \
     'heavyHiggsMaster.dat' using ($13-$15):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using ($5-$7):xticlabels(2) title	\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster.dat' using ($14-$16):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'heavyHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"


# ---------------------- dedicated charge --------------------------------------

# set size 1,1
# set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
# set lmargin 16
# set bmargin 3.5
# set xlabel font ",35"
# set xtics font ", 40" rotate by 0 offset 2.5,-1. scale 0
# set mytics 4
# set ytics font ", 35" 0,1.0
# set title font ",40" offset 0,1
set key font ",40"

set ytics font ", 35"
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set xtics font ", 40" rotate by 0 offset 4,-1. scale 0


set output "1L_sm.pdf"
set size 1,1
set title "SM-like Higgs" font ",40"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 0.6,-0.45 Left reverse
plot [0.5:4.5][-1.8:1.5] \
     'smHiggsMaster1L.dat' using ($3-$5):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = M_S}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$7):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = M_S}" lt rgb "#33a02c",	\
     '' 		   using ($4-$6):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = m_t}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$8):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = m_t}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\


set output "1L_sm_mssm.pdf"
set title "SM-like Higgs, 1-loop" font ",30"
set ytics 0.25
set mytics 2
set key samplen 4.25 spacing 5.5 at 0.6,-0.3 font ",30" 
plot [0:5][-1:1.25] \
     'smHiggsMaster1L.dat'							\
     			   using ($9-$11):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$5):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#33a02c",	\
     '' 		   using ($10-$12):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$6):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\



set output "2L_sm_mssm.pdf"
set key at -0.4,-0.3 font ",30" spacing 5 samplen 7
set title "SM-like Higgs, 2-loop"
plot [-1:4][-1:1.25] \
     'smRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\
     'smRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#a6cee3",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#1f78b4",	\


set output "1L_sg.pdf"
set title "singlet-like Higgs" font ",40"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 0.6,1. font ",40"
plot [0.5:4.5][-0.5:1.] \
     'singletMaster1L.dat'							\
     			   using ($3-$5):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = M_S}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$7):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = M_S}" lt rgb "#33a02c",	\
     '' 		   using ($4-$6):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = m_t}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$8):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = m_t}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\


set ytics font ", 35"
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set xtics font ", 40" rotate by 0 offset 4,-1. scale 0


set output "1L_hy.pdf"
set title "heavy Higgs" font ",40"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 0.6,1. font ",40" 
plot [0.5:4.5][-0.5:1.] \
     'heavyHiggsMaster1L.dat'							\
     			   using ($3-$5):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = M_S}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$7):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = M_S}" lt rgb "#33a02c",	\
     '' 		   using ($4-$6):xticlabels(2) title			\
     		           "{{/Symbol a}_{G_F}, Q = m_t}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$8):xticlabels(2) title 	 		\
     			   "{{/Symbol a}(M_Z), Q = m_t}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\




set output "1L_hy_mssm.pdf"
set title "heavy Higgs, 1-loop" font ",30"
set ytics 0.25
set mytics 2
set key samplen 4.25 spacing 5.5 at 0.6,1.2 font ",30" 
plot [0:5][-0.6:1.25] \
     'heavyHiggsMaster1L.dat'							\
     			   using ($9-$11):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#b2df8a",	\
     '' 	           using ($3-$5):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#33a02c",	\
     '' 		   using ($10-$12):xticlabels(2) title			\
     		           "{MSSM-limit}" lt rgb "#a6cee3",	\
     '' 	           using ($4-$6):xticlabels(2) title 	 		\
     			   "{NMSSM}" lt rgb "#1f78b4",	\
     # '' 	           using ($9-$11):xticlabels(2) title			\
     # 			   "{NFH MSSM-limit}" lt rgb "#1f78b4",  		\
     # '' 	           using ($9-$13):xticlabels(2) title			\
     # 			   "{NFH {/Symbol a}(M_Z) MSSM-limit}" lt rgb "#a6cee3",\

set output "2L_hy_mssm.pdf"
set key at -0.4,1.2 font ",30" spacing 5 samplen 7
set title "heavy Higgs, 2-loop"
plot [-1:4][-0.6:1.25] \
     'hyRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\
     'hyRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#a6cee3",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#1f78b4",	\






# --------------------------- apprRepa -------------------------------

set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
set xlabel font ",25"
set ytics -2,0.25,10
set xtics font ", 25" rotate by 0 
set ytics font ", 25"
set xzeroaxis linewidth 2.5

set output "1L2L_sm_ms.pdf"
set title "SM-like Higgs M_S"
set key at 0.5,1.2 font ",30" spacing 5 samplen 7
plot [0:5][-1.:1.25] \
     'resMZI.dat' using 2:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 5:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"


set output "1L2L_sm_mt.pdf"
set title "SM-like Higgs m_t"
set key at 0.5,1.2 font ",30" spacing 5 samplen 7
plot [0:5][-1.:1.25] \
     'resMZII.dat' using 2:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 5:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"





set output "1L2L_sg_ms.pdf"
set title "singlet-like Higgs M_S"
set key at 0.5,1.4 font ",30" spacing 5 samplen 7
plot [0:5][-1.25:1.5] \
     'resMZI.dat' using 3:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 6:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"

set output "1L2L_sg_mt.pdf"
set title "singlet-like Higgs m_t"
set key at 0.5,1.4 font ",30" spacing 5 samplen 7
plot [0:5][-1.25:1.5] \
     'resMZII.dat' using 3:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 6:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"




set output "1L2L_hy_ms.pdf"
set title "heavy Higgs M_S"
set key at 0.6,1.25 font ",30" spacing 5 samplen 7
plot [0:5][-1.5:1.25] \
     'resMZI.dat' using 4:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 7:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"

set output "1L2L_hy_mt.pdf"
set title "heavy Higgs m_t"
set key at 0.6,1.2 font ",30" spacing 5 samplen 7
plot [0:5][-1.5:1.25] \
     'resMZII.dat' using 4:xticlabels(1) title			\
     		  "{{/Symbol D}m_h^{1L}}" lt rgb "#33a02c",	\
     ''		  using 7:xticlabels(1) title		\
     		  "{{/Symbol D}m_h^{2L}}" lt rgb "#b2df8a",		\
     ''		  using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m_h^{appr}}" lt rgb "#1f78b4",	\
     # 'smHiggsMaster.dat' using ($6-$8):xticlabels(2) title 	\
     # 			 "{CII NMSSM {Q=m_t}}" lt rgb "#a6cee3"


set key font ",40"
set title font ",40"

set ytics font ", 35"
set ylabel "{/Symbol D}m/GeV" font ",40" offset -5.5
set xtics font ", 40" rotate by 0 offset 4,-1. scale 0


set output "1L2L_sm_short.pdf"
set title "SM-like Higgs" 
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 1.6,1. Left reverse
# set key at 0.6,1. font ",40" spacing 5 samplen 7
plot [1.5:5.5][-1:1.] \
     'resMZI.dat' using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} M_S}" lt rgb "#33a02c",	\
     'resMZII.dat' using ($5-$2):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} m_t}" lt rgb "#1f78b4",	\


set output "1L2L_sg_short.pdf"
set title "singlet-like Higgs"
set ytics 0.5
set mytics 5
set key samplen 4.25 spacing 8.0 at 1.6,-0.7 Left reverse
# set key at 0.7,1.25 font ",30" spacing 5 samplen 7
plot [1.5:5.5][-1.:0.25] \
     'resMZI.dat' using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} M_S}" lt rgb "#33a02c",	\
     'resMZII.dat' using ($6-$3):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} m_t}" lt rgb "#1f78b4",	\


set output "1L2L_hy_short.pdf"
set title "heavy Higgs"
set ytics 0.25
set mytics 5
set key samplen 4.25 spacing 8.0 at 1.6,0.25 Left reverse
# set key at 1.6,0.25 font ",30" spacing 5 samplen 7
plot [1.5:5.5][-0.25:0.25] \
     'resMZI.dat' using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} M_S}" lt rgb "#33a02c",	\
     'resMZII.dat' using ($7-$4):xticlabels(1) title 	\
     		  "{{/Symbol D}m^{appr} m_t}" lt rgb "#1f78b4",	\



set output "mssm_sm_ms.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "SM-like Higgs M_S"
plot [0:5][-0.8:1.] \
     'smRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\

set output "mssm_sm_mt.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "SM-like Higgs m_t"
plot [0:5][-0.8:1.] \
     'smRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\
     # 'smHiggsMasterNoTP1.dat' using ($13-$15):xticlabels(2) title 	\
     # 			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     # '' 		 using ($5-$7):xticlabels(2) title		\
     # 			 "{NMSSM}" lt rgb "#b2df8a",		\
     # 'res1L2LI.dat' 	 using ($5 - $6 + $2 - $3 ):xticlabels(1) title 	\
     # 			 "{NMSSM-rtet}" lt rgb "#33a02c",	\



















set output "mssm_hy_ms.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "heavy Higgs M_S"
plot [0:5][-0.8:1.25] \
     'hyRes1L2LI.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\


# set output "mssm_hy_ms.pdf"
# set key at 0.5,0.75 font ",30" spacing 5 samplen 7
# set title "heavy Higgs M_S"
# plot [0:5][-0.5:0.75] \
#      'heavyHiggsMasterNoTP1.dat' using ($13-$15):xticlabels(2) title 	\
#      			 "{MSSM-limit}" lt rgb "#33a02c",	\
#      '' 		 using ($5-$7):xticlabels(2) title		\
#      			 "{NMSSM}" lt rgb "#b2df8a",		\

set output "mssm_hy_mt.pdf"
set key at 0.5,-0.5 font ",30" spacing 5 samplen 7
set title "heavy Higgs m_t"
plot [0:5][-0.8:1.25] \
     'hyRes1L2LII.dat' 	 using ($7 - $8):xticlabels(1) title 	\
     			 "{MSSM-limit}" lt rgb "#b2df8a",	\
     ''			 using ($4 - $6 - (( $4 - $5 ) - ( $2 - $3 )) ):xticlabels(1) title 	\
     			 "{NMSSM}" lt rgb "#33a02c",	\

# set output "mssm_hy_mt.pdf"
# set title "heavy Higgs m_t"
# plot [0:5][-0.5:0.75] \
#      'heavyHiggsMasterNoTP1.dat' using ($14-$16):xticlabels(2) title 	\
#      			 "{MSSM-limit}" lt rgb "#1f78b4",	\
#      '' 		 using ($6-$8):xticlabels(2) title 	\
#      			 "{NMSSM}" lt rgb "#a6cee3"






# ------------------------------------------------------------
# ------------------------------------------------------------

# --------------------- histograms ---------------------------


# set terminal pdf enhanced linewidth 3.5 size 10,6
set terminal pdf enhanced linewidth 3.5 size 7,4

set style data histogram
set style histogram columnstacked

set ylabel "{/Symbol D}m/GeV" font ",30" offset -2.5
set xlabel font ",25"
set xtics font ", 25" rotate by 0
set ytics font ", 25"

# set linetype 1 lt rgb "#33a02c"
# set linetype 2 lt rgb "#1f78b4"

set style fill solid noborder
set boxwidth 0.75
set xzeroaxis linewidth 2.5


set output "diff_detail_sm.pdf"
set title "SM-like Higgs" font ",30"
# set key autotitle columnheader at 2.,-0.5 font ",30" spacing 5 samplen 7
# plot [0:8][-1:1]  \
#      'smDiffMasterI.dat'  using 3:key(1),\
#      'smDiffMasterII.dat' using 3,       \
#      'blank.dat'	  using 2,	 \
#      'smDiffMasterI.dat'  using 4,       \
#      'smDiffMasterII.dat' using 4,       \
#      'blank.dat'	  using 2,	 \
#      'smDiffMasterI.dat'  using 5,       \
#      'smDiffMasterII.dat' using 5,       \
#      'blank.dat'	  using 2,	 \
#      'smDiffMasterI.dat'  using 6,       \
#      'smDiffMasterII.dat' using 6

# set output "diff_detail_sm2.pdf"
# set title "SM-like Higgs" font ",30"
set key autotitle columnheader at 1.7,4 font ",30" spacing 5 samplen 7
plot [0:8][-2:4]  \
     'smMZI.dat'  using 3:key(1),	\
     'smMZII.dat' using 3,		\
     'blank.dat'  using 2,		\
     'smMZI.dat'  using 4,		\
     'smMZII.dat' using 4,		\
     'blank.dat'  using 2,		\
     'smMZI.dat'  using 5,		\
     'smMZII.dat' using 5,		\
     'blank.dat'  using 2,		\
     'smMZI.dat'  using 6,		\
     'smMZII.dat' using 6



set output "diff_detail_singlet.pdf"
set title "singlet-like Higgs" font ",30"
set key autotitle columnheader at 2,-3.0 font ",30" spacing 5 samplen 7
plot [0:8][-4.5:2]  \
     'singMZI.dat'  using 3:key(1),	\
     'singMZII.dat' using 3,		\
     'blank.dat'    using 2,		\
     'singMZI.dat'  using 4,		\
     'singMZII.dat' using 4,		\
     'blank.dat'    using 2,		\
     'singMZI.dat'  using 5,		\
     'singMZII.dat' using 5,		\
     'blank.dat'    using 2,		\
     'singMZI.dat'  using 6,		\
     'singMZII.dat' using 6

     # 'singDiffMasterI.dat'  using 3:key(1),\
     # 'singDiffMasterII.dat' using 3,       \
     # 'blank.dat'	    using 2,  	   \
     # 'singDiffMasterI.dat'  using 4,       \
     # 'singDiffMasterII.dat' using 4,       \
     # 'blank.dat'	    using 2,  	   \
     # 'singDiffMasterI.dat'  using 5,       \
     # 'singDiffMasterII.dat' using 5,       \
     # 'blank.dat'	    using 2,       \
     # 'singDiffMasterI.dat'  using 6,       \
     # 'singDiffMasterII.dat' using 6



set output "diff_detail_heavy.pdf"
set title "heavy Higgs" font ",30"
set key autotitle columnheader at 2,-0.6 font ",30" spacing 5 samplen 7
plot [0:8][-1.5:3.]  \
     'heavyMZI.dat'  using 3:key(1),	\
     'heavyMZII.dat' using 3,		\
     'blank.dat'     using 2,		\
     'heavyMZI.dat'  using 4,		\
     'heavyMZII.dat' using 4,		\
     'blank.dat'     using 2,		\
     'heavyMZI.dat'  using 5,		\
     'heavyMZII.dat' using 5,		\
     'blank.dat'     using 2,		\
     'heavyMZI.dat'  using 6,		\
     'heavyMZII.dat' using 6

     # 'heavyDiffMasterI.dat'  using 3:key(1),\
     # 'heavyDiffMasterII.dat' using 3,       \
     # 'blank.dat'	     using 2,       \
     # 'heavyDiffMasterI.dat'  using 4,       \
     # 'heavyDiffMasterII.dat' using 4,       \
     # 'blank.dat'	     using 2,       \
     # 'heavyDiffMasterI.dat'  using 5,       \
     # 'heavyDiffMasterII.dat' using 5,       \
     # 'blank.dat'	     using 2,       \
     # 'heavyDiffMasterI.dat'  using 6,       \
     # 'heavyDiffMasterII.dat' using 6


     # 'heavyDiffMasterI.dat'  using 2:key(1),\
     # 'heavyDiffMasterII.dat' using 2,       \
     # 'blank.dat'	       using 2,       \
     



# ------------------------------------------------------------


==> plots/gnuScript__Ramona_Gr__ber_s_conflicted_copy_2016-11-26_ <==
set terminal pdf enhanced linewidth 3.5
# font arial 21 size 900,675
# Make the x axis labels easier to read.
set xtics rotate out
# Select histogram data
set style data histogram
# Give the bars a plain fill pattern, and draw a solid line around them.
set style fill solid border
set style histogram clustered
# plot [-1:5][120:135] for [COL=2:4:1] 'dummy.dat' using COL:xticlabels(1) title columnheader

# --------------------------- total -------------------------------

#a6cee3
#1f78b4
#b2df8a
#33a02c

# --------------------------- total -------------------------------

set output "total_sm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:8] \
     'smHiggsMaster.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{\"out-of-the-box\" {Q=M_S}}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=M_S}" lt rgb "#b2df8a",		\
     'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     			 "{\"out-of-the-box\" {Q=m_t}}" lt rgb "#1f78b4",	\
     'smHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=m_t}" lt rgb "#a6cee3"

#     title "{/Symbol a}_s mod II" lt rgb "#c2e699" fillstyle pattern {2,7,14} transparent


set output "total_singlet.pdf"
set title "Singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][0:2] \
     'singletMaster.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{\"out-of-the-box\" {Q=M_S}}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=M_S}" lt rgb "#b2df8a",		\
     'singletMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     			 "{\"out-of-the-box\" {Q=m_t}}" lt rgb "#1f78b4",	\
     'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=m_t}" lt rgb "#a6cee3"

set output "total_heavy.pdf"
set title "Heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:1.5] \
     'heavyHiggsMaster.dat' using (abs($3-$7)):xticlabels(2) title		\
     			 "{\"out-of-the-box\" {Q=M_S}}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=M_S}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     			 "{\"out-of-the-box\" {Q=m_t}}" lt rgb "#1f78b4",	\
     'heavyHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=m_t}" lt rgb "#a6cee3"




# --------------------------- repara -------------------------------


set output "repara_sm.pdf"
set title "SM-like Higgs"
set key top right
plot [0:6][0:1] \
     'smHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'smHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_singlet.pdf"
set title "Singlet-like Higgs"
set key top left
plot [0:6][0:1] \
     'singletMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'singletMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_heavy.pdf"
set title "Heavy Higgs"
set key top left
plot [0:6][0:1.5] \
     'heavyHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'heavyHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"


# --------------------------- appr -------------------------------

set output "appr_sm.pdf"
set key top right
plot [0:6][0:7] \
     'smHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'smHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_singlet.pdf"
set key top left
plot [0:6][0:2] \
     'singletMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'singletMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_heavy.pdf"
set key top left
plot [0:6][0:2] \
     'heavyHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'heavyHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"




# --------------------------- OSvsRbar -------------------------------


set output "OSvsDRbar_sm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:10] \
     'smHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'smHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_singlet.pdf"
set title "Singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][0:2.5] \
     'singletMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "  {Q=M_S}" lt rgb "#33a02c", \
     'singletMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "  {Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_heavy.pdf"
set title "Heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:70] \
     'heavyHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'heavyHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"


# --------------------------- repara 1L -------------------------------


set output "repara_sm_1L.pdf"
set key top right
plot [0:6][0:2] \
     'smHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'smHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_singlet_1L.pdf"
set key top right
plot [0:6][0:2] \
     'singletMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'singletMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_heavy_1L.pdf"
set key top right
plot [0:6][0:2] \
     'heavyHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'heavyHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"


# --------------------------- repara Loop -------------------------------

set output "repara_sm_i.pdf"
set key top left
plot [0:6][0:1.1] \
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'smHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'smHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_singlet_i.pdf"
set key top left
plot [0:6][0:1] \
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'singletMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'singletMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_heavy_i.pdf"
set key top left
plot [0:6][0:0.5] \
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'heavyHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'heavyHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\


set output "repara_sm_ii.pdf"
set key top left
plot [0:6][0:1.5] \
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'smHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'smHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_singlet_ii.pdf"
set key top left
plot [0:6][0:1.2] \
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'singletMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'singletMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_heavy_ii.pdf"
set key top left
plot [0:6][0:1.6] \
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'heavyHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'heavyHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\


# --------------------------- MSSM-limit -------------------------------

set output "total_sm_mssm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left reverse Left
plot [0:6][0:1.2] \
     'smHiggsMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'smHiggsMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'smHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"


set output "total_singlet_mssm.pdf"
set title "singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][0:1.2] \
     'singletMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'singletMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"



set output "total_heavy_mssm.pdf"
set title "heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left reverse Left
plot [0:6][0:1.2] \
     'heavyHiggsMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title	\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'heavyHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"


==> plots/gnuScript___Ramona_Gr__ber_s_conflicted_copy_2016-11-26_ <==
set terminal pdf enhanced linewidth 3.5 
# font arial 21 size 900,675
# Make the x axis labels easier to read.
set xtics rotate out
# Select histogram data
set style data histogram
# Give the bars a plain fill pattern, and draw a solid line around them.
set style fill solid border
set style histogram clustered
# plot [-1:5][120:135] for [COL=2:4:1] 'dummy.dat' using COL:xticlabels(1) title columnheader

# --------------------------- total -------------------------------

#a6cee3
#1f78b4
#b2df8a
#33a02c

# --------------------------- total -------------------------------

set output "total_sm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:8] \
     'smHiggsMaster.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{\"out-of-the-box\" {Q=M_S}}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=M_S}" lt rgb "#b2df8a",		\
     'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     			 "{\"out-of-the-box\" {Q=m_t}}" lt rgb "#1f78b4",	\
     'smHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=m_t}" lt rgb "#a6cee3"

#     title "{/Symbol a}_s mod II" lt rgb "#c2e699" fillstyle pattern {2,7,14} transparent


set output "total_singlet.pdf"
set title "Singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][0:2] \
     'singletMaster.dat' using (abs($3-$7)):xticlabels(2) title			\
     			 "{\"out-of-the-box\" {Q=M_S}}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=M_S}" lt rgb "#b2df8a",		\
     'singletMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     			 "{\"out-of-the-box\" {Q=m_t}}" lt rgb "#1f78b4",	\
     'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=m_t}" lt rgb "#a6cee3"

set output "total_heavy.pdf"
set title "Heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:1.5] \
     'heavyHiggsMaster.dat' using (abs($3-$7)):xticlabels(2) title		\
     			 "{\"out-of-the-box\" {Q=M_S}}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=M_S}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2) title 		\
     			 "{\"out-of-the-box\" {Q=m_t}}" lt rgb "#1f78b4",	\
     'heavyHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 		\
     			 "{/Symbol a}_s mod {Q=m_t}" lt rgb "#a6cee3"




# --------------------------- repara -------------------------------


set output "repara_sm.pdf"
set title "SM-like Higgs"
set key top right
plot [0:6][0:1] \
     'smHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'smHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_singlet.pdf"
set title "Singlet-like Higgs"
set key top left
plot [0:6][0:1] \
     'singletMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'singletMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"

set output "repara_heavy.pdf"
set title "Heavy Higgs"
set key top left
plot [0:6][0:1.5] \
     'heavyHiggsMaster.dat' using (abs($7-$9)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, I",	\
     'heavyHiggsMaster.dat' using (abs($8-$10)):xticlabels(2)			\
     			 title "|m_{h}|^{{/Symbol a}(M_Z)}-m_{h}|^{G_F}|, II"


# --------------------------- appr -------------------------------

set output "appr_sm.pdf"
set key top right
plot [0:6][0:7] \
     'smHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'smHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'smHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_singlet.pdf"
set key top left
plot [0:6][0:2] \
     'singletMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'singletMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'singletMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"

set output "appr_heavy.pdf"
set key top left
plot [0:6][0:2] \
     'heavyHiggsMaster.dat' using (abs($3-$7)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($3-$9)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, I",	\
     'heavyHiggsMaster.dat' using (abs($4-$8)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}_{G_F}, FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II",	\
     'heavyHiggsMaster.dat' using (abs($4-$10)):xticlabels(2)			\
     title "|m_{h}|^{{/Symbol a}(M_Z), FH}-m_{h}|^{{/Symbol a}(M_Z), NC}|, II"




# --------------------------- OSvsRbar -------------------------------


set output "OSvsDRbar_sm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:10] \
     'smHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'smHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_singlet.pdf"
set title "Singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][0:2.5] \
     'singletMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "  {Q=M_S}" lt rgb "#33a02c", \
     'singletMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "  {Q=m_t}" lt rgb "#1f78b4"

set output "OSvsDRbar_heavy.pdf"
set title "Heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top right
plot [0:6][0:70] \
     'heavyHiggsMaster.dat' using (abs($3-$11)):xticlabels(2) title \
          "{Q=M_S}"  lt rgb "#33a02c", \
     'heavyHiggsMaster.dat' using (abs($4-$12)):xticlabels(2) title \
          "{Q=m_t}" lt rgb "#1f78b4"


# --------------------------- repara 1L -------------------------------


set output "repara_sm_1L.pdf"
set key top right
plot [0:6][0:2] \
     'smHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'smHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_singlet_1L.pdf"
set key top right
plot [0:6][0:2] \
     'singletMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'singletMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"

set output "repara_heavy_1L.pdf"
set key top right
plot [0:6][0:2] \
     'heavyHiggsMaster1L.dat' using (abs($3-$5)):xticlabels(2) title "vanilla I",		\
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "{/Symbol a}(M_Z) I",	\
     'heavyHiggsMaster1L.dat' using (abs($4-$6)):xticlabels(2) title "vanilla II",		\
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "{/Symbol a}(M_Z) II"


# --------------------------- repara Loop -------------------------------

set output "repara_sm_i.pdf"
set key top left
plot [0:6][0:1.1] \
     'smHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'smHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'smHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_singlet_i.pdf"
set key top left
plot [0:6][0:1] \
     'singletMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'singletMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'singletMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\

set output "repara_heavy_i.pdf"
set key top left
plot [0:6][0:0.5] \
     'heavyHiggsMaster1L.dat' using (abs($3-$7)):xticlabels(2) title "1L I",	\
     'heavyHiggsMaster.dat' using (abs($5-$9)):xticlabels(2) title "2L I"
#    'heavyHiggsMasterLO.dat' using (abs($3-$5)):xticlabels(2) title "LO I",	\


set output "repara_sm_ii.pdf"
set key top left
plot [0:6][0:1.5] \
     'smHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'smHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'smHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_singlet_ii.pdf"
set key top left
plot [0:6][0:1.2] \
     'singletMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'singletMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'singletMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\

set output "repara_heavy_ii.pdf"
set key top left
plot [0:6][0:1.6] \
     'heavyHiggsMaster1L.dat' using (abs($4-$8)):xticlabels(2) title "1L II",	\
     'heavyHiggsMaster.dat' using (abs($6-$10)):xticlabels(2) title "2L II"
#    'heavyHiggsMasterLO.dat' using (abs($4-$6)):xticlabels(2) title "LO II",	\


# --------------------------- MSSM-limit -------------------------------

set output "total_sm_mssm.pdf"
set title "SM-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left reverse Left
plot [0:6][0:1.2] \
     'smHiggsMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'smHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'smHiggsMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'smHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"


set output "total_singlet_mssm.pdf"
set title "singlet-like Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left
plot [0:6][0:1.2] \
     'singletMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'singletMaster.dat' using (abs($5-$7)):xticlabels(2) title		\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'singletMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'singletMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"



set output "total_heavy_mssm.pdf"
set title "heavy Higgs"
set ylabel "{/Symbol D}m/GeV"
set key top left reverse Left
plot [0:6][0:1.2] \
     'heavyHiggsMaster.dat' using (abs($13-$15)):xticlabels(2) title 	\
     			 "{CI MSSM-limit {Q=M_S}}" lt rgb "#33a02c",	\
     'heavyHiggsMaster.dat' using (abs($5-$7)):xticlabels(2) title	\
     			 "{CI NMSSM {Q=M_S}}" lt rgb "#b2df8a",		\
     'heavyHiggsMaster.dat' using (abs($14-$16)):xticlabels(2) title 	\
     			 "{CII MSSM-limit {Q=m_t}}" lt rgb "#1f78b4",	\
     'heavyHiggsMaster.dat' using (abs($6-$8)):xticlabels(2) title 	\
     			 "{CII NMSSM {Q=M_S}}" lt rgb "#a6cee3"


==> sections/calculation__Ramona_Gr__ber_s_conflicted_copy_2016-11-26_.tex <==
\section{Mass prediction for the \cp-even Scalars}
\label{sec:Results}

In  a first  step  the  masses and  mixing  matrices  of the  \cp-even
Higgs-sector  are  evaluated  in  the TP  scenarios  with  both  codes
``out-of-the-box''.   We   used  the  following   choices  for  the
renormalisation schemes in the top/stop and Higgs sectors:

\begin{itemize}
\item on-shell renormalisation scheme  adopted for the top/stop sector
  and the mass of the charged Higgs as input in \NC, labelled ``\NCs\ \OS'',
\item \DRbar\  renormalisation scheme adopted for  the top/stop sector
  and $\Al$ in \NC, labelled ``\NCs\ \DRbar'',
\item on-shell renormalisation scheme  adopted for the top/stop sector
  and the mass of the charged Higgs in \NFH, labelled ``\NFHs''.
\end{itemize}
\noindent
The numerical  results for  the masses given  in tab.~\ref{tab:resOB},
the   results   for   the   mixing-matrix  elements   are   given   in
tabs.~\ref{tab:originalZH13_A}  and~\ref{tab:originalZH13_B}. For  the
identification  of the  singlet--like fields  we follow  the procedure
applied  in~\cite{Staub:2015aea},  where  the  field  $h_i$  with  the
largest  singlet-admixture  \ZH{i3}  at   zero  external  momentum  is
identified    with   the    dominantly    singlet-like   field.     In
fig.~\ref{fig:total}  the  absolute   difference  between  the  masses
obtained with the different ``out-of-the-box'' codes with the on-shell
option are shown by the \htPD{dark green and blue} bars.  The absolute
difference between the on-shell and  \DRbar\ options in \NC\ are shown
in fig.~\ref{fig:OSvsDRbar}.


\subsection{Comparing the \OS\ Codes}

%
\begin{table}[htb]
  \scriptsize \centering
  \begin{tabular}{llcccccccccc}
    &
    & \multicolumn{2}{c}{TP1} & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
    & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
    \\\toprule
    & $Q$ & $1500$ & $172.9$ & $1500$ & $172.9$ & $1500$ & $172.9$
    & $1500$ & $172.9$ & $1500$ & $172.9$
    \\\midrule\midrule
    \multirow{3}[6]{*}{$h_1$} 
    & \NCs\ \DRbar
    & \bf 120.34 & \bf 122.18 & \bf 118.57 & --- 
    & \it 90.88 & \it 87.78 & \bf 126.37 & \bf 125.76 & \it 120.32 & \it 118.65
    \\\cmidrule{2-12}
    & \NCs\ \OS
    & \bf 121.84 & \bf 113.46 & \bf 120.42 & --- 
    & \it 90.37 & \it 90.19 & \bf 127.42 & \bf 128.91 & \it 120.06 & \it 118.73
    \\\cmidrule{2-12}
    & \NFHs
    & \bf 115.70 & \bf 113.19 & \bf 114.12 & ---
    & \it 90.13 & \it 90.72 & \bf 127.13 & \bf 128.24 & \it 119.00 & \it 119.03
    \\
    \midrule
    \midrule
    \multirow{3}[6]{*}{$h_2$} 
    & \NCs\ \DRbar
    & \it 1797.46 & \it 1797.46 & \it 5951.36 & --- 
    & \bf 124.86 & \bf 124.68 & \it 142.59 & \it 141.28 & \bf 123.14 & \bf 125.26
    \\\cmidrule{2-12}
    & \NCs\ \OS
    & \it 1797.45 & \it 1797.54 & \it 5951.36 & --- 
    & \bf 125.69 & \bf 124.09 & \it 142.14 & \it 139.74 & \bf 123.86 & \bf 122.22
    \\\cmidrule{2-12}
    & \NFHs
    & \it 1797.45 & \it 1797.60 & \it 5951.36 & --- 
    & \bf 124.07 & \bf 123.31 & \it 141.95 & \it 139.97 & \bf 122.33 & \bf 121.82
    \\
    \midrule
    \midrule
    \multirow{3}[6]{*}{$h_3$} 
    & \NCs\ \DRbar
    & 2756.37 & 2754.11 & 6371.31 & --- & 652.48 & 652.64 & 467.42 & 467.01 & 627.00 & 628.77
    \\\cmidrule{2-12}
    & \NCs\ \OS
    & 2747.84 & 2692.84 & 6374.51 & --- & 650.84 & 645.37 & 465.70 & 461.34 & 626.06 & 626.43
    \\\cmidrule{2-12}
    & \NFHs
    & 2747.91 & 2692.84 & 6374.59 & --- & 650.40 & 645.40 & 464.91 & 461.32 & 626.46 & 626.47
    \\\bottomrule
  \end{tabular}
  \caption{Masses  for  the  \cp-even  scalars for  TP1-5  when  using
    \NC\  (\NCs) and  \NFH\  (\NFHs)  ``out-of-the-box''.  The  values
    correspond  to  the  two-loop  result obtained  with  the  default
    version  of  \NFH, and  the  on-shell  or \DRbar\  renormalisation
    scheme for the top/stop-sectors in \NC, labelled ``\NCs\ \OS'' and
    ``\NCs\ \DRbar'', respectively.  The masses for the SM-like scalar
    are written  in bold fonts,  those for the singlet-like  scalar in
    italics.}
  \label{tab:resOB}
\end{table}

When comparing the Higgs masses obtained  with \NFH\ and \NC\ with the
on-shell options, we  find that for the SM-like  fields the difference
between  the  mass predictions  of  both  codes  can  be as  large  as
6~\giga\electronvolt,  where the  largest  differences  occur for  the
MSSM-like scenarios TP1  and TP2 for the evaluation at  the high scale
$Q$.   For the  evaluations at  the  low scale  $m_t$ the  differences
between  the  codes  do  not exceed  300~\mega\electronvolt\  for  the
MSSM-like scenarios  TP1 and TP2, and  1.9~\giga\electronvolt\ for the
remaining scenarios TP3-5.   The difference between the  masses of the
heaviest fields,  which are  always doublet-like in  all TP-scenarios,
remain relatively  small with  less than  1.3~\giga\electronvolt.  For
scenarios with a  singlet-like field that is heavier  than the SM-like
field the  difference remains below 1~\giga\electronvolt,  while for a
lighter   singlet-field   the  differences   can   be   as  large   as
1.5~\giga\electronvolt.

\begin{figure}[phtb]
  \centering
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_sm.pdf}
  \;\;
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_singlet.pdf}
  \\
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_heavy.pdf}
  \caption{Difference  between  the  Higgs   masses  of  the  SM-like,
    singlet-like and heavy Higgs (from  top to bottom) at the two-loop
    level calculated with different versions of \NC\ and \FH.}
  \label{fig:total}
\end{figure}


\subsection{Comparing \NC\ with the \OS\ \& \DRbar\ Option}

For  the  comparison  of  the  results obtained  with  a  on-shell  or
\DRbar\ renormalised top/stop  sector we find that for  most TP points
the  result  agrees  with the  \htPD{3--5~\giga\electronvolt}\  effect
expected in the MSSM~\htPD{CITEME!}   for the doublet-like fields. For
the    SM-like     field    the     effect    is    as     large    as
2.5~\giga\electronvolt\  and for  the  heaviest \cp-even  field up  to
10~\giga\electronvolt.  The scenario TP1 is a notable exception with a
difference rising up to almost 9~\giga\electronvolt\ for the lightest,
SM-like  field  and  up  to 60~\giga\electronvolt\  for  the  heaviest
\cp-even field and  has to be discussed  separately.  The singlet-like
field is less affected by the renormalisation scheme of the top/sector
than the (MS)SM-like fields\footnote{For  TP5 the singlet admixture to
  the two lighter fields varies  significantly when evaluated at $m_t$
  for an on-shell or \DRbar\ renormalised top/stop sector.  \htPD{Thus
    the  dark  green  bar  for TP5  in  fig.~\ref{fig:total}  for  the
    lightest field shows  the impact of the  renormalisation scheme of
    the   electromagnetic   couplings   $\alpha$   on   a   dominantly
    singlet-like field, while the dark green bar shows the impact on a
    doublet-like field.  The reverse is  true for the  second lightest
    field.}}.


\begin{figure}[phtb]
  \centering
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/OSvsDRbar_sm.pdf}
  \;\;
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/OSvsDRbar_singlet.pdf}
  \\
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/OSvsDRbar_heavy.pdf}
  \caption{Difference  between  the  Higgs   masses  of  the  SM-like,
    singlet-like and heavy Higgs (from  top to bottom) at the two-loop
    level calculated in \NC\ with the  \OS\ and \DRbar\ option for the
    renormalisation in the top-/stop-sector.}
  \label{fig:OSvsDRbar}
\end{figure}


\subsection{Mixing Matrix Elements}

%
\begin{table}[htb]
  %% \hspace*{-2.7cm}
  %% \renewcommand*\arraystretch{0.9}
  \scriptsize \centering
  \begin{tabular}{lllccccccccc}
    & & & \multicolumn{3}{c}{TP1} & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
    \\\toprule
    $i$ & $Q$ &
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    \\\midrule\midrule
    \multirow{6}[4]{*}{$1$} & \multirow{3}[0]{*}{$ M_{\rm S}$}
    & \NCs\ \DRbar 
    & {0.1039} & {0.9946} & {0.0076}  
    & {0.1034} & {0.9946} & {0.0004}
    & {0.2177} & {0.1923} & {0.9569}
    \\ 
    & & \NCs\ \OS  
    & {0.1039} & {0.9946} & {0.0076}
    & {0.1034} & {0.9946} & {0.0004}
    & {0.2127} & {0.1753} & {0.9613}
    \\ 
    & & \NFHs
    & 0.1040 & 0.9946 & 0.0071
    & 0.1034 & 0.9946 & 0.0004
    & 0.2049 & 0.1786 & 0.9623
    \\\cmidrule{2-12}
    & \multirow{3}[0]{*}{$m_t$}
    & \NCs\ \DRbar
    & {0.1008} & {0.9949} & {0.0073}
    & {---} & {---} & {---}
    & {0.2212} & {0.2142} & {0.9514}
    \\
    & & \NCs\ \OS
    & {0.1006} & {0.9949} & {0.0074}
    & {---} & {---} & {---} 
    & {0.1881} & {0.1016} & {0.9769}
    \\ 
    & & \NFHs 
    & 0.1008 & 0.9949 & 0.0071
    & {---} & {---} & {---}
    & 0.1765 & 0.0881 & 0.9804
    \\\midrule\midrule
    \multirow{6}[4]{*}{$2$} & \multirow{3}[0]{*}{$ M_{\rm S}$}
    & \NCs\ \DRbar
    & {0.0075} & {0.0068} & {0.9999}
    & {0.0095} & {0.0006} & {1.}
    & {0.2811} & {0.9265} & {0.2502}
    \\
    & & \NCs\ \OS
    & {0.0076} & {0.0068} & {0.9999}
    & {0.0095} & {0.0006} & {1.}
    & {0.2854} & {0.9297} & {0.2327}
    \\ 
    & & \NFHs
    & 0.0071 & 0.0064 & 1.
    & 0.0089 & 0.0005 & 1.
    & 0.2884 & 0.9285 & 0.2337
    \\\cmidrule{2-12}
    & \multirow{3}[0]{*}{$m_t$}
    & \NCs\ \DRbar 
    & {0.0075} & {0.0066} & {0.9999}
    & {---} & {---} & {---} 
    & {0.2677} & {0.9248} & {0.2705} 
    \\
    & & \NCs\ \OS
    & {0.0079} & {0.0066} & {0.9999}
    & {---} & {---} & {---}
    & {0.2925} & {0.9437} & {0.1545}
    \\
    & & \NFHs
    & 0.0076 & 0.0064 & 1.
    & {---} & {---} & {---}
    & 0.2978 & 0.9445 & 0.1385
    \\\midrule\midrule
    \multirow{6}[4]{*}{$3$} & \multirow{3}[0]{*}{$M_{\rm S}$}
    & \NCs\ \DRbar
    & {0.9946} & {0.1040} & {0.0068}
    & {0.9946} & {0.1034} & {0.0095}
    & {0.9347} & {0.3234} & {0.1476}
    \\ 
    & & \NCs\ \OS
    & {0.9946} & {0.1040} & {0.0068}
    & {0.9946} & {0.1034} & {0.0095}\
    & {0.9345} & {0.3238} & {0.1477}
    \\ 
    & & \NFHs 
    & 0.9946 & 0.1040 & 0.0064
    & 0.9946 & 0.1034 & 0.0089
    & 0.9353 & 0.3255 & 0.1388
    \\\cmidrule{2-12}
    & \multirow{3}[0]{*}{$m_t$}
    & \NCs\ \DRbar
    & {0.9949} & {0.1008} & {0.0068}
    & {---} & {---} & {---}
    & {0.9378} & {0.3145} & {0.1472}
    \\
    & & \NCs\ \OS
    & {0.9949} & {0.1007} & {0.0072}
    & {---} & {---} & {---}
    & {0.9376} & {0.3148} & {0.1478}
    \\
    & & \NFHs 
    & 0.9949 & 0.1008 & 0.0069
    & {---} & {---} & {---}
    & 0.9382 & 0.3164 & 0.1404
    \\\bottomrule
  \end{tabular}
  \caption{Mixing matrix elements as obtained by the \NC\ vanilla
    version for $Q=M_{SUSY}$ and  $Q=m_t$, below the respective values
    the $\DRbar$ numbers (only option 7 in \NC\ changed). }
  \label{tab:originalZH13_A}
\end{table}


\begin{table}[hbt]
  %% \hspace*{-2.7cm}
  %% \renewcommand*\arraystretch{0.9}
  \scriptsize \centering
  \begin{tabular}{lllcccccc|c} 
    & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5} & TP5
    \\\toprule
    $i$ & $Q$ &
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & $|Z_{i3}^{\rm 1L}|$
    \\\midrule\midrule
    \multirow{6}[4]{*}{$1$} & \multirow{3}[0]{*}{$M_{\rm S}$}
    & \NCs\ \DRbar 
    & {0.4869} & {0.7849} & {0.3832}
    & {0.2967} & {0.4433} & {0.8459} & 0.3685
    \\
    & & \NCs\ \OS
    & {0.4852} & {0.7639} & {0.4255}
    & {0.2709} & {0.3426} & {0.9092} &  0.9762
    \\ 
    & & \NFHs 
    & 0.4889 & 0.8201 & 0.2973
    & 0.3543 & 0.7777 & 0.5193 & 0.9794
    %% & 0.2615 & 0.3397 & 0.9034 & 
    \\\cmidrule{2-9}
    & \multirow{3}[0]{*}{$m_t$}
    & \NCs\ \DRbar
    & {0.4774} & {0.8045} & {0.3534}
    & {0.3129} & {0.5451} & {0.7778} & 0.9595
    \\
    & & \NCs\ \OS
    & {0.4765} & {0.8549} & {0.2053}
    & {0.0785} & {0.6226} & {0.7786} & 0.9455
    \\ 
    & & \NFHs
    & 0.4703 & 0.8758 & 0.1086
    & 0.3478 & 0.8777 & 0.3296 & 0.9449
    %% & 0.2903 & 0.4685 & 0.8344 & 0.9449
    \\\midrule\midrule
    \multirow{6}[4]{*}{$2$} & \multirow{3}[0]{*}{$M_{\rm S}$}
    & \NCs\ \DRbar 
    & {0.0447} & {0.4158} & {0.9084}
    & {0.2055} & {0.8354} & {0.5099} & 0.9162
    \\ 
    & & \NCs\ \OS
    & {0.0679} & {0.4522} & {0.8893}
    & {0.2390} & {0.8813} & {0.4076} & 0.1501
    \\ 
    & & \NFHs
    & 0.0086 & 0.3363 & 0.9417
    & 0.0556 & 0.5368 & 0.8419 & 0.1387
    %% & 0.2460 & 0.8816 & 0.4028 & 0.1387
   \\\cmidrule{2-9}
    & \multirow{3}[0]{*}{$m_t$}
    & \NCs\ \DRbar
    & {0.0232} & {0.3906} & {0.9203}
    & {0.1594} & {0.7772} & {0.6088}& 0.2344
    \\
    & & \NCs\ \OS
    & {0.0526} & {0.2608} & {0.9640}
    & {0.3418} & {0.7169} & {0.6077} & 0.2857
    \\
    & & \NFHs
    & 0.0907 & 0.1703 & 0.9812
    & 0.0265 & 0.3606 & 0.9324 & 0.2918
    %% & 0.1939 & 0.8251 & 0.5307 & 0.2918
    \\\midrule\midrule
    \multirow{6}[4]{*}{$3$} & \multirow{3}[0]{*}{$M_{\rm S}$}
    &\NCs\ \DRbar 
    & {0.8723} & {0.4594} & {0.1674}
    & {0.9326} & {0.3251} & {0.1568} & 0.1572
    \\ 
    & & \NCs\ \OS 
    & {0.8718} & {0.4604} & {0.1676}
    & {0.9325} & {0.3254} & {0.1569} & 0.1560
    \\ 
    & & \NFHs 
    & 0.8723 & 0.4630 & 0.1574
    & 0.9335 & 0.3272 & 0.1470 & 0.1468
    %% & 0.9333 & 0.3276 & 0.1470 & 0.1468
    \\\cmidrule{2-9}
    & \multirow{3}[0]{*}{$m_t$}
    &\NCs\ \DRbar
    & {0.8784} & {0.4476} & {0.1678}
    & {0.9363} & {0.3144} & {0.1563}& 0.1565
    \\ 
    & & \NCs\ \OS
    & {0.8776} & {0.4485} & {0.1691}
    & {0.9365} & {0.3138} & {0.1565} & 0.1561
    \\ 
    & & \NFHs
    & 0.8778 & 0.4517 & 0.1595
    & 0.9372 & 0.3156 & 0.1486 & 0.1482
    %% & 0.9371 & 0.3159 & 0.1487 & 0.1482
   \\\bottomrule
  \end{tabular}
  %
  \caption{Mixing matrix elements as obtained by the \NC\ vanilla
    version for $Q=M_{SUSY}$ and  $Q=m_t$, below the respective values
    the  $\DRbar$  numbers  (only  option  7  in  \NC\  changed).
    \htPD{NB: The last column specifies the 1-loop singlet-admixture in
      order to  estimate the  impact of  the \NFH-approximation  on the
      different results.}}
  \label{tab:originalZH13_B}
\end{table}



The  results for  the mixing-matrix  elements for  the \cp-even  Higgs
fields     are     presented     in     tabs.~\ref{tab:originalZH13_A}
and~\ref{tab:originalZH13_B}. The  matrix elements denoted  by \ZH{ij}
correspond  to  the unitary  matrices  that  diagonalise the  two-loop
corrected mass matrix for zero external momentum,
%
\begin{align}
  \mathcal{M}_{hh}{\left(k^2=0\right)}
  =
  \ZH{}
  \left[\mathbf{M}_{\phi\phi} + \hat{\Sigma}{\left(k^2=0\right)}\right]
  \left(\ZH{}\right)^\dagger = \text{diag}{\left\{m_{h_1}, m_{h_2}, m_{h_3}\right\}},
  \label{eq:2LoopZH}
\end{align}
\noindent
where  the  $m_{h_i}$ denote  the  two-loop  corrected masses  of  the
\cp-even  Higgs fields.   For the  scenarios TP1-3  the mixing  matrix
elements  agree within  1\%,  independent of  the  used treatment  of
$\alpha$ or the chosen renormalisation scheme for the top/stop sector.
For TP4  and TP5 significant  differences can be observed  between all
three results,  with differences  up to  $\approx 30\%$  between \NFH,
which  utilises $\alpha_{G_F}$,  and  \NC\ with  the on-shell  option,
which  utilises  $\alpha{(M_Z)}$.    The  largest  differences  appear
generally  for the  admixture  of  the singlet  scalar.   In order  to
confirm that  these results are  not caused by  the MSSM-approximation
employed  in \NFH,  we  compared  the mixing  matrix  elements at  the
one-loop  level  and found  similar  and  in  some cases  even  larger
differences.  The difference  between the mixing of \NC\  run with the
on-shell and \DRbar\ option for the top/stop sector of $\lesssim 20\%$
is generally smaller than between \NC\ and \NFH.

\htPD{ \htRG{ \sout{If  the mixing-matrix elements  \ZH{} are used to  identify the
  SM-like and singlet-like  scalar, we found that  different codes can
  lead  to a  different  identification of  the  SM-like field.   This
  effect is of particular importance  for the singlet-admixture to the
  fields  $h_i$,   which  can   considerably  depend  on   the  chosen
  renormalisation scheme. In scenarios with two fields that carry both
  a significant singlet-admixture,  like TP4 and TP5,  this effect can
  lead to  a different phenomenology.  E.g.   in TP5 the field  with a
  mass  around  $125~\giga\electronvolt$  can be  either \htRG{mainly}
   singlet-  or
  doublet-like depending on the applied renormalisation schemes.}}
\htRG{We found that the effect of the renormalisation scheme on the mixing can be by far larger than the 
effect on the mass prediction, where the relative difference never exceeded 5\%.
 This is in particular the case for TP4 and TP5, 
 where we have large singlet admixtures. 
 In this case we find even factor of two differences in the mixing matrix elements
 for different renormalisation schemes.
 We remark that this can lead to different conclusions whether a 
 parameter point is excluded or not by LHC data.
}
 % However, we found  that the effect of the  renormalisation scheme on
 % the mixing is by far larger  than the effect on the mass prediction,
 % where the relative difference never exceeded 5\%.
  %% As  can be  seen  in eq.~\eqref{eq:2LoopZH},  only  products of  the
  %% \ZH{ij} enter the calculation.  However, this effect does not have a
  %% similarily severe impact on the mass prediction, 
}





\section{Breaking down the Differences}
\label{sec:Discussion}

The observed differences between the two codes ``out-of-the-box'' seem
to  be unusually  large, especially  for  the comparison  at the  high
scale.  We  found that these  differences are caused by  MSSM-like and
genuine  NMSSM  effects.   In  this  section  these  effects  will  be
identified  in   order  to  isolate   the  impact  of   the  different
renormalisation schemes.
%
\begin{table}[htb]
  \scriptsize \centering
  \begin{tabular}{llcccccccccc}
    &
    & \multicolumn{2}{c}{TP1} & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
    & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
    \\\toprule
    &$Q$ & $1500$ & $172.9$ & $1500$ & $172.9$ & $1500$ & $172.9$
    & $1500$ & $172.9$ & $1500$ & $172.9$
    \\\midrule\midrule
    \multirow{3}[6]{*}{$h_1$} & \NCs\ $\alpha_s$ mod
    & \bf 116.26 & \bf 113.76 & \bf 114.66 & --- 
    & \it 90.24 & \it 90.20 & \bf 126.05 & \bf 129.00 & 118.17 & \bf 118.80
    \\\cmidrule{2-12}
    & \NFHs\ $\alpha_{G_F}$
    & \bf 115.70 & \bf 113.19 & \bf 114.12 & ---
    & 90.13 & 90.72 & \bf 127.13 & \bf 128.24 & 119.00 & \bf 119.03
    \\\cmidrule{2-12}
    & \NFHs\ $\alpha{(M_Z)}$
    & \bf 116.28 & \bf 113.80 & \bf 114.66 & ---
    & 90.18 & 89.81 & \bf 126.49 & \bf 128.39 & 118.82 & \bf 119.33
    \\
    \midrule
    \midrule
    \multirow{3}[6]{*}{$h_2$} & \NCs\ $\alpha_s$ mod
    & \it 1797.45 & \it 1797.54 & \it 5951.36 & --- 
    & \bf 123.48 & \bf 124.21 & \it 141.86 & \it 139.75 & \bf 122.33 & 122.31
    \\\cmidrule{2-12}
    & \NFHs\ $\alpha_{G_F}$
    & \it 1797.45 & \it 1797.60 & \it 5951.36 & --- 
    & \bf 124.07 & \bf 123.31 & \it 141.95 & \it 139.97 & \bf 122.33 & 121.82
    \\\cmidrule{2-12}
    & \NFHs\ $\alpha{(M_Z)}$
    & \it 1797.45 & \it 1797.60 & \it 5951.36 & --- 
    & \bf 123.78 & \bf 123.59 & \it 141.85 & \it 139.19 & \bf 122.23 & 121.52
    \\
    \midrule
    \midrule
    \multirow{3}[6]{*}{$h_3$} & \NCs\ $\alpha_s$ mod
    & 2747.83 & 2692.84 & 6374.51 & --- & 650.80 & 645.37 & 645.37 & 461.35 & 626.02 & 626.43
    \\\cmidrule{2-12}
    & \NFHs\ $\alpha_{G_F}$
    & 2747.91 & 2692.84 & 6374.59 & --- & 650.40 & 645.40 & 464.91 & 461.32 & 626.46 & 626.47
    \\\cmidrule{2-12}
    & \NFHs\ $\alpha{(M_Z)}$
    & 2747.84 & 2692.75 & 6374.52 & --- & 650.52 & 644.46 & 465.24 & 460.49 & 625.60 & 625.21
    \\\bottomrule
  \end{tabular}
  \caption{Masses  for  the  \cp-even  scalars for  TP1-5  when  using
    modified versions of \NC\ (\NCs) and \NFH\ (\NFHs). Both codes are
    modified to use  the identical numerical value  of $\alpha_s$.  In
    \NFH\    the   default    reparametrisation   to    $\alpha_{G_F}$
    (\NFH\    $\alpha_{G_F}$)    and    the    reparametrisation    to
    $\alpha{(M_Z)}$  (\NFH\  $\alpha{(M_Z)}$)  is  used.   The  values
    correspond  to  the two-loop  result  obtained  with the  on-shell
    renormalisation scheme  for the top/stop-sectors.  The  masses for
    the  SM-like scalar  are  written  in bold  fonts,  those for  the
    singlet-like scalar in italics. \htRG{ARE WE SURE THAT FOR TP5 AT SCALE MT THE LIGHTEST IS SM-LIKE? CHECK!}}
  \label{tab:resASmod}
\end{table}


\subsection{Treatment of $\alpha_s$}
\label{sec:AsTreatment}

For the MSSM-like scenarios TP1  and TP2 the different renormalisation
prescription for  the electromagnetic  coupling and mixing  effects of
the singlet are suppressed due to very small values of $\lambda$.  The
different treatment of the strong  coupling constant $\alpha_s$ is the
main source of the difference between  the two codes for these points.
In tab.~\ref{tab:resASmod}  the mass predictions are  recalculated for
the  case that  \NC\  is  modified such,  that  always the  hard-coded
\MSbar-value   of   the   strong   coupling   at   the   scale   \MTO,
$\alpha_s^{\MSbar}{(\MTO)} =  0.10697$ as  obtained with  the routines
of~\cite{Chetyrkin:2000yt}, is used\footnote{The  results of \NFH\ are
  not affected by this procedure, since $\alpha_s^{\MSbar}{(\MTO)}$ is
  the standard value  that is used.}. For  graphical representation of
the absolute differences  see the \htPD{light green and  blue} bars in
fig.~\ref{fig:total}.  When both codes use the same numerical value of
$\alpha_s$ a much better agreement  between their mass predictions can
be observed.  The difference between the mass predictions never exceed
1.5~\giga\electronvolt\ for all masses in the TP-scenarios.


\subsection{TP1}

In  fig.~\ref{fig:OSvsDRbar}  a  huge   difference  between  the  mass
prediction in scenario TP1 can be found when comparing the results for
both MSSM-like \cp-even Higgs fields  obtained at the scale \MTO\ with
the  on-shell and  \DRbar\ options  in  \NC. The  difference is  much
larger than the impact of  the different renormalisation schemes would
suggest   for  an   MSSM-like  scenario.    The  same   difference  is
significantly smaller, if  the masses are evaluated at  the high scale
$M_{\rm S} = 1500~\giga\electronvolt$.  These different results at two
different scales  is somewhat surprising since  the physical situation
before and after the evolution  of the scenario parameters are naively
expected to be identical.

We found that the large, absolute difference between the two codes and
their predictions is  a result of an imperfect  parameter evolution in
{\tt  FlexibleSUSY}.   In  this   specific  scenario  the  gluino-mass
parameter $M_3$ at the high scale  $M_{\rm S }$ is very large compared
to  the  remaining  mass  spectrum.   Thus  for  a  correct  parameter
evolution from  $M_{\rm S}$ down to  \MTO\ the heavy gluino  should be
decoupled~\cite{Muhlleitner:2008yw}\htPD{,   in    order   to   [avoid
    higher-order effects due to] \ldots }.  If the heavy gluino is not
decoupled,  as  in  {\tt  FlexibleSUSY}, the  obtained  parameters  at
\MTO\  do not  describe the  same physical  situation as  the original
parameters at  $M_{\rm S}$.   The comparison of  the Higgs  masses for
``TP1'' at both scales thus do not describe the difference between the
two  calculations  but  a  difference between  two  distinct  physical
scenarios\footnote{It  is important  to  note that  this behaviour  is
  unrelated   to  the   choice  of   renormalisation  scheme   in  the
  calculation.  It has also been  observed for calculations using only
  \DRbar\   methods~\cite{Braathen:2016mmb}~\htPD{Cite  also   Georg's
    talk?}.}.

We found also that the parameters  obtained at \MTO\ define a scenario
that is highly  sensitive on variations of the  stop parameters.  This
is especially  true for $A_t$,  which is  large compared to  the other
soft-breaking   parameters  of   the  scenario.    E.g.   changes   of
$\left|\Delta{A_t}\right| \approx 100~\giga\electronvolt$ can yield to
a    change    of   the    mass    of    the   lightest    field    of
$\left|\Delta{m_{h_1}}\right| \approx 2~\giga\electronvolt$. Since the
observed  effect  originates  from  the  parameter  evolution  and  is
independent    from   the    Higgs-mass   calculation    itself   (see
tab.~\ref{tab:AlgorithmComparison}), the  scenario TP1 in  the present
form is not viable for estimating theoretical uncertainties.

\htPD{PD: Is this correct and extensive enough?}



\subsection{MSSM-Approximation in \NFH}

In \NFH\  an approximation  at the two-loop  level plus  a fixed-order
reparametrisation is  applied.  The  MSSM-approximation gives  rise to
differences to \NC\ that are of two-loop order.  The reparametrisation
gives rise to a differences of one-loop and higher-orders. In order to
estimate  the  size  of  these  effects we  compared  the  results  of
\NC\ with  the results of  \NFH\ utilising a reparametrisation  of the
electromagnetic  coupling   constant  to  $\alpha{(M_Z)}$.    \NC\  is
modified to  use the same numerical  value $\alpha_s^{\MSbar}{(\MTO)}$
as  \NFH, as  described in  sec.~\ref{sec:AsTreatment}.  The  obtained
results   are  given   in   tab.~\ref{tab:resASmod}.   The   imperfect
fixed-order    reparametrisation    to   $\alpha{(M_Z)}$    and    the
MSSM-approximation together result  in a total effect of  no more than
660~\mega\electronvolt\ for the  masses of the \cp-even  fields in the
discussed TP-scenarios.


\subsection{Genuine NMSSM Effect from Charge Renormalisation}

The renormalisation of the electromagnetic coupling $\alpha$ induces a
one-loop  effect in  the NMSSM,  while  the same  procedure induces  a
two-loop effect in  the MSSM.  In order to  disentangle this MSSM-like
two-loop  effect  from  the  genuine NMSSM  one-loop  effect,  the  TP
scenarios at both  scales $M_{\rm S}$ and $m_t$ are  also evaluated in
their  MSSM  limit,  where  $\lambda   =  \kappa  \rightarrow  0$.   A
comparison of  the obtained Higgs  masses with \NC\ with  the on-shell
option and \NFH\ in the MSSM-limit quantifies the MSSM two-loop effect
induced by the renormalisation of  $\alpha$.  This comparison is shown
as the  dark blue and  green bars in fig.~\ref{fig:MSSMLimit}  for the
two MSSM-like fields, whereas the  same comparison for the original TP
scenarios are shown in lighter  blue and green. The difference between
the two green and the blue bars for each scenario denote the impact of
the genuine NMSSM effect at each scale.

For the MSSM-like scenarios TP1 and TP2 the genuine MSSM effect on the
mass  of  the  SM-like field  is  small  with  a  tiny impact  on  the
evaluation   at   the  high   scale   and   an  impact   of   $\approx
100~\mega\electronvolt$ at  the scale $m_t$. For  the scenarios TP3-5,
which feature a larger value of $\lambda$, this effect can increase up
to $\approx 400~\mega\electronvolt$ at either scale.

\htPD{PS: Should we also discuss the mass of the heavy Higgs here?}


\begin{figure}[phtb]
  \centering
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_sm_mssm.pdf}
  \;\;
  \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_heavy_mssm.pdf}
  \caption{as is}
  \label{fig:MSSMLimit}
\end{figure}

\htPD{PS: Is the fig.~\ref{fig:MSSMLimit} enough of do we need another
  table?}



==> sections/calculation_sven.tex <==
\begin{table}[h]
  \scriptsize \centering
  \begin{tabular}{llcccccccccc}
    &
    & \multicolumn{2}{c}{TP1} & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
    & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
    \\\toprule
    & $Q$ & $\MS$ & $\mt$ & $\MS$ & $\mt$ & $\MS$ & $\mt$
    & $\MS$ & $\mt$ & $\MS$ & $\mt$
    \\\midrule\midrule
    \multirow{2}[4]{*}{$h_1$} 
    & \NCs\ \OS
    & \bf 121.84 & \bf 113.47 & \bf 120.42 & --- 
    & \it 89.92 & \it 88.81 & \bf 126.44 & \bf 126.65 & \it 119.54 & \it 117.63
    \\\cmidrule{2-12}
    & \NFHs
    & \bf 115.70 & \bf 113.20 & \bf 114.12 & ---
    & \it 89.67 & \it 89.36 & \bf 126.17 & \bf 126.29 & \it 118.47 & \it 117.95
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_2$} 
    & \NCs\ \OS
    & \it 1797.45 & \it 1797.57 & \it 5951.36 & --- 
    & \bf 126.16 & \bf 125.80 & \it 143.32 & \it 142.73 & \bf 124.44 & \bf 123.51
    \\\cmidrule{2-12}
    & \NFHs
    & \it 1797.45 & \it 1797.62 & \it 5951.36 & --- 
    & \bf 124.55 & \bf 125.02 & \it 143.11 & \it 142.68 & \bf 122.93 & \bf 123.10
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_3$} 
    & \NCs\ \OS
    & 2755.73 & 2752.14 & 6370.77 & --- & 652.60 & 652.70 & 467.89 & 467.35 & 627.18 & 628.72
    \\\cmidrule{2-12}
    & \NFHs
    & 2755.79 & 2752.25 & 6370.85 & --- & 652.17 & 652.65 & 467.10 & 467.33 & 626.59 & 628.76
    \\\bottomrule
  \end{tabular}
 \caption{Masses of the \cp-even scalars for TP1-5 when using the
 indicated versions of \NC\ and \NFH\ as specified in
 \refse{sec:outofthebox}. %
 The masses of the SM-like scalar are written in bold fonts, those
 of the singlet-like scalar in italics.}
  \label{tab:resOB}
\end{table}

\section{Predictions for masses and mixing matrices of the \cp-even scalars}
\label{sec:Results}

In this section we analyze the differences in the predictions for the
\cp-even Higgs boson masses and mixing matrices from \NFH\ and \NC. We
start by a comparison of the ``out-of-the-box'' results including the
corrections of up to \order{\alt\als}, where sizable differences show
up. In order to understand the origin of these differeces we then
perform a comparison at the one-loop level, where we find that part of
the differences can be attributed to the different renormalization of
the electroweak sector in the two codes. After ``removing'' this
difference we continue with an analysis at the two-loop level, where
we investigate the effect of the strong coupling constant and the
genuine NMSSM corrections to the Higgs boson self-energies. Finally we
compare the results obtained with the OS version of \NC\ with the
\DRbar\ calculation. The \htMM{identification of the} various sources
of differences between the \htMM{different} calculations are important
ingredients for a reliable estimate of the 
intrinsic uncertainties in the Higgs-boson mass and mixing matrix
calculations in the NMSSM

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{``Out-of-the-box'' results}
\label{sec:outofthebox}

In the first step of our  comparison the masses and mixing matrices of
the \cp-even Higgs-sector are evaluated in the TP scenarios \htPD{with
  the ``out-of-the-box''  versions of  \NC\ and \NFH,  restricting the
  two-loop  corrections   in  the  latter   to  $\mathcal{O}{(\alpha_t
    \alpha_s)}$  (cf.  sec.~\ref{sec:calcho})}.   For  the results  of
\NC\  we  used  the   ``out-of-the-box''  version  with  the  on-shell
renormalisation scheme for  the top/stop sector and  the charged Higgs
mass (see  \refse{sec:drbaros}), labelled ``\NCs\ OS''.   For \NFH\ we
used the  ``out-of-the-box'' version,  but included only  the two-loop
corrections  of   \order{\alt\als},  labelled  \NFHs.    The  obtained
numerical results for  the masses are given  in \refta{tab:resOB}, the
results for the  mixing-matrix elements, see \refeq{Uh},  are given in
\refta{tab:originalZH13_A}.
%
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
 \scriptsize \centering
 \begin{tabular}{lllccccccccc}
 & & & \multicolumn{3}{c}{TP1} & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$ \MS$}
 & \NCs\ \OS 
 & {0.1039} & {0.9946} & {0.0076}
 & {0.1034} & {0.9946} & {0.0004}
 & {0.2199} & {0.1994} & {0.9549}
 \\ 
 & & \NFHs
 & 0.1039 & 0.9946 & 0.0071
 & 0.1034 & 0.9946 & 0.0004
 & 0.2134 & 0.2064 & 0.9549
 \\\cmidrule{2-12}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.1006} & {0.9949} & {0.0073}
 & {---} & {---} & {---} 
 & {0.2236} & {0.2210} & {0.9493}
 \\ 
 & & \NFHs 
 & 0.1006 & 0.9949 & 0.0071
 & {---} & {---} & {---}
 & 0.2245 & 0.2264 & 0.9478
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$ \MS$}
 & \NCs\ \OS
 & {0.0075} & {0.0068} & {0.9999}
 & {0.0096} & {0.0006} & {1.}
 & {0.2797} & {0.9249} & {0.2575}
 \\ 
 & & \NFHs
 & 0.0071 & 0.0064 & 1.
 & 0.0090 & 0.0005 & 1.
 & 0.2820 & 0.9228 & 0.2625
 \\\cmidrule{2-12}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.0075} & {0.0066} & {0.9999}
 & {---} & {---} & {---}
 & {0.2659} & {0.9232} & {0.2775}
 \\
 & & \NFHs
 & 0.0072 & 0.0064 & 1.
 & {---} & {---} & {---}
 & 0.2656 & 0.9216 & 0.2831
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.9946} & {0.1040} & {0.0068}
 & {0.9946} & {0.1034} & {0.0096}\
 & {0.9346} & {0.3237} & {0.1476}
 \\ 
 & & \NFHs 
 & 0.9946 & 0.1039 & 0.0064
 & 0.9946 & 0.1034 & 0.009
 & 0.9354 & 0.3253 & 0.1388
 \\\cmidrule{2-12}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.9949} & {0.1006} & {0.0068}
 & {---} & {---} & {---}
 & {0.9377} & {0.3144} & {0.1476}
 \\
 & & \NFHs 
 & 0.9949 & 0.1006 & 0.0065
 & {---} & {---} & {---}
 & 0.9376 & 0.3153 & 0.1467
 \\\bottomrule\bottomrule\\
 \end{tabular}
 %
 \\
 %
 \begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.4813} & {0.7432} & {0.4648}
 & {0.2845} & {0.3943} & {0.8738}
 \\ 
 & & \NFHs 
 & 0.4873 & 0.8022 & 0.3448
 & 0.3540 & 0.7764 & 0.5214
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.4766} & {0.7886} & {0.3885}
 & {0.3393} & {0.6991} & {0.6294}
 \\ 
 & & \NFHs
 & 0.4788 & 0.8104 & 0.3377
 & 0.3390 & 0.7204 & 0.6051
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.0895} & {0.4858} & {0.8694}
 & {0.2224} & {0.8594} & {0.4603}
 \\ 
 & & \NFHs
 & 0.0334 & 0.3775 & 0.9254
 & 0.0564 & 0.5387 & 0.8406
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.0411} & {0.4215} & {0.9059}
 & {0.0882} & {0.6425} & {0.7612}
 \\
 & & \NFHs
 & 0.0171 & 0.3761 & 0.9264
 & 0.0819 & 0.6181 & 0.7818
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS 
 & {0.8720} & {0.4600} & {0.1673}
 & {0.9325} & {0.3253} & {0.1568}
 \\ 
 & & \NFHs 
 & 0.8726 & 0.4625 & 0.1571
 & 0.9335 & 0.3270 & 0.1469
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.8782} & {0.4477} & {0.1685}
 & {0.9365} & {0.3137} & {0.1564}
 \\ 
 & & \NFHs
 & 0.8778 & 0.4493 & 0.1662
 & 0.9372 & 0.3146 & 0.1505
 \\\bottomrule
 \end{tabular}
 %
 \caption{Absolute values for the mixing matrix elements of the
 \cp-even scalar sector for TP1-5 when using the indicated versions
 of \NC\ and \NFH\ as specified in the text. \htC{SH: check
 relative signs between codes}}
 \label{tab:originalZH13_A}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


For the identification of the singlet-like field we follow the
procedure applied in~\cite{Staub:2015aea}, where the field $h_i$ with
the largest singlet-admixture \ZH{i3} is identified with the
dominantly singlet-like field.

%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_sm.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_singlet.pdf}
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_heavy.pdf}
 \caption{Difference $\Delta{m} = m_h^{\NCs} - m_h^{\NFHs}$ between
 the Higgs masses of the SM-like, singlet-like and heavy Higgs at
 the two-loop level calculated at the scales \MS\ and \MTO. }
 \label{fig:total}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In \reffi{fig:total} the difference $\Delta{m} = m_h^{\NCs} -
m_h^{\NFHs}$ between the mass predictions obtained with the codes
``\NCs\ OS'' and ``\NFHs'' are shown. All values are given for two
input scales $Q$, the SUSY mass scale $Q = \MS$ in darker bars and the
top-quark mass scale $Q= \MTO = 172.9~\gev$ in lighter bars.


When comparing the Higgs masses obtained with \NFH\ and \NC%% \ with the
, we find that for the SM-like field the difference between the mass
predictions of both codes can be larger than
6~\gev\ for the scenarios TP1 and TP2 and the evaluation
at the high scale $M_S$. For the evaluations at the low scale $\mt$,
however, the differences between the codes do not exceed
1~\gev\ for all scenarios. %
The difference between the masses of the heaviest fields, which are
always doublet-like in all TP-scenarios, remain relatively small with
less than 1.3~\gev. For scenarios with a singlet-like
field that is heavier than the SM-like field the absolute
difference between the mass predictions for the singlet-like
field remains below 1~\gev, while for a lighter
singlet-field the differences can be as large as
1.9~\gev. The mixing matrix elements \htMM{of the SM-like Higgs boson}
obtained by the two codes agree within $\approx 2\%$ for the scenarios TP1-3. 
\htMM{For the singlet-like Higgs boson the differences in the mixing
  matrix elements, on the other hand, can be substantial. In case of
  the heavy Higgs $h_3$ the matrix elements differ by at most
  10\%.}
For TP4 and TP5 significant differences can be observed between the
two results, with differences of up to $\approx~40\%$.

In general, we find that the differences for mixing matrix elements
seem to be by far larger than for the mass predictions, where the relative
differences never exceeded 5\%. This is in particular the case for TP4
and TP5, where we have large singlet admixtures to the SM-like Higgs
field with a mass around 125~\gev. In this case we even find a factor
of two differences in the mixing matrix elements. In these scenarios
the Higgs masses and mixing matrices seem to be very sensitive to
changes of the parameters. We remark that this can lead to different
conclusions whether a parameter point is excluded or not by LHC data.
\htC{Maggie: Are you sure about the
entries for the singlet nature in TP5? Here
$h_1$ is singlet-like for FeynHiggs and not for NMSSMCALC. For $h_2$
NMSSMCALC is singlet-like and not FeynHiggs.}

The observed differences between the mass predictions obtained at the
two-loop level appear to be unusually large, especially for the
comparison at the high scale \MS. In the following we will analyze the
differences in more detail, starting with a discussion of the chosen
test-point TP1 and a study of the diffferences at the one-loop level.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The test-point TP1}

In  \refta{tab:resOB}   very  large   differences  between   the  mass
prediction in the  MSSM-like scenario TP1 can be  found when comparing
the results for both MSSM-like \cp-even Higgs fields obtained with the
same code at either  the scale $\MS$ or \MTO. They can  be as large as
$\approx 8.5~\gev$ for the SM-like  scalar and \NC\ and \htPD{$\approx
  3~\gev$  for the  heavy  scalar and  both  codes}.  These  different
results  at  two different  scales  may  at  first sight  be  somewhat
surprising since the physical situation before and after the evolution
of the parameters of the scenario is naively expected to be identical.
We found that  the large, absolute difference  between the predictions
at  either the  scale \MTO\  or  $\MS$ is  a result  of the  parameter
evolution performed by {\tt  FlexibleSUSY}.  In this specific scenario
at the high scale $\MS$ the  gluino-mass parameter $M_3 = 3~{\rm TeV}$
(cf.   tab.~\ref{tab:TPDefinition})  is  very large  compared  to  the
remaining mass spectrum.  Thus for  a correct parameter evolution from
$\MS$   down  to   \MTO\  the   heavy  gluino   should  be   decoupled
consistently~\cite{Muhlleitner:2008yw}.   If the  heavy gluino  is not
decoupled  consistently,  the  obtained low-scale  scenario  does  not
correspond to the physics situation described by the parameters at the
high scale.   The comparison of the  Higgs masses for ``TP1''  at both
scales  thus  does  not  describe   the  difference  between  the  two
calculations   but  a   difference  between   two  distinct   physical
scenarios.\footnote{It  is important  to note  that this  behaviour is
  unrelated  to  the  choice  of the  renormalisation  scheme  in  the
  calculation. This has also been observed for calculations using only
  \DRbar\ methods~\cite{Braathen:2016mmb}. \htC{PD:  Cite also Georg's
    talk?/Maggie: I would say it is not necessary.}}% .

We found also that the parameters  obtained at \MTO\ define a scenario
that is highly sensitive to variations of the stop parameters. This is
especially true  for $A_t$, which  \htMM{at the input scale  $M_S$} is
large compared to the other  soft-breaking parameters of the scenario.
For    example,    at    the    low    scale    \MTO\    changes    of
$\left|\Delta{A_t}\right| \approx 100~\gev$ can  yield a change of the
mass   of   the   lightest   field   of   $|\Delta{m_{h_1}}|   \approx
2~\gev$. \htC{Maggie: Why  don't you write 'of the  SM-like field' and
  instead write 'of the lightest  field'? PD: Lightest field instantly
  clarifies which number is meant.}

Since the observed effects are independent of the Higgs-mass
calculation itself (see \reffi{fig:Alg}), the scenario TP1 in the
present form is not viable for estimating theoretical
uncertainties. Thus we will omit this scenario in the following.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Renormalisation of \boldmath{$\alpha$}}
\label{sec:1LReparametrisation}

\htC{Maggie: We have to unify the notation, e.g. renormalization or
  renormalisation etc.} \\
In order to disentangle the different effects in the renormalization,
coupling constants and higher order corrections, we start by comparing
the one-loop results for the Higgs-boson masses and mixing
matrices. Here we use the versions '\NCs\ OS' and '\NFHs' as described
in the previous section, but restricted to the pure one-loop
contribution to the Higgs-boson self-energies. The only difference
between the calculations stems from the different renormalisation
prescription of the electromagnetic coupling constant $\alpha$, see
\refta{tab:DiffNcNfhVanilla}. The numerical results for the \cp-even
Higgs-boson masses are given in \refta{tab:resOB1L}.

%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
 \scriptsize \centering
 \begin{tabular}{llcccccccc}
 &
 & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
 & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
 \\\toprule
 & $Q$ 
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 \\\midrule\midrule
 \multirow{3}[6]{*}{$h_1$} 
 & \NCs\ \OS
 & \bf 140.67 & ---
 & \it 90.47 & \it 90.12 & \bf 132.48 & \bf 134.10 & \it 120.93 & \it 120.57
 \\\cmidrule{2-10}
 & \NFHs
 & \bf 139.68 & ---
 & \it 90.30 & \it 89.98 & \bf 132.96 & \bf 133.42 & \it 120.82 & \it 120.51
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \bf 140.67 & ---
 & \it 90.38 & \it 89.96 & \bf 132.73 & \bf 133.22 & \it 120.91 & \it 120.53
 \\
 \midrule
 \midrule
 \multirow{3}[6]{*}{$h_2$} 
 & \NCs\ \OS
 & \it 5951.36 & --- 
 & \bf 136.35 & \bf 138.25 & \it 146.45 & \it 146.84 & \bf 135.56 & \bf 138.27
 \\\cmidrule{2-10}
 & \NFHs
 & \it 5951.36 & --- 
 & \bf 136.73 & \bf 137.04 & \it 146.82 & \it 146.05 & \bf 136.30 & \bf 137.06
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \it 5951.36 & --- 
 & \bf 136.74 & \bf 137.19 & \it 146.59 & \it 145.89 & \bf 136.32 & \bf 137.26
 \\
 \midrule
 \midrule
 \multirow{3}[6]{*}{$h_3$} 
 & \NCs\ \OS
 & 6370.75 & --- & 652.80 & 653.13 & 468.63 & 468.32 & 627.34 & 629.19
 \\\cmidrule{2-10}
 & \NFHs
 & 6370.83 & --- & 652.49 & 653.04 & 468.01 & 468.30 & 626.94 & 629.14
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & 6370.88 & --- & 652.62 & 653.18 & 468.37 & 468.60 & 627.08 & 629.23
 \\\bottomrule
 \end{tabular}
 \caption{One-loop masses for the \cp-even scalars for TP2--5 when
 using the indicated versions of \NC\ and \NFH\ as specified in the
 text. The masses of the SM-like scalar are written in bold fonts,
 those of the singlet-like scalar in italics.}
 \label{tab:resOB1L}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
 \scriptsize \centering
 \begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.1034} & {0.9946} & {0.0004}
 & {0.2048} & {0.1503} & {0.9672} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$ 
 & 0.1034 & 0.9946 & 0.0004
 & 0.1981 & 0.1443 & 0.9695
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {---} & {---} & {---}
 & {0.2048} & {0.1553} & {0.9664} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & {---} & {---} & {---}
 & 0.2054 & 0.1601 & 0.9655
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.0096} & {0.0006} & {1.0000}
 & {0.2935} & {0.9332} & {0.2071}
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.0092 & 0.0005 & 1.0000
 & 0.2971 & 0.9337 & 0.1997
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {---} & {---} & {---}
 & {0.2836} & {0.9356} & {0.2104} 
 \\
 & & \NFHs\ $\alpha{(\MZ)}$
 & {---} & {---} & {---}
 & 0.2837 & 0.9344 & 0.2153
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS 
 & {0.9946} & {0.1034} & {0.0096}
 & {0.9338} & {0.3263} & {0.1470} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$ 
 & 0.9946 & 0.1034 & 0.0092
 & 0.9341 & 0.3276 & 0.1421
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {---} & {---} & {---}
 & {0.9368} & {0.3172} & {0.1475} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & {---} & {---} & {---}
 & 0.9366 & 0.3182 & 0.1466
 \\\bottomrule\bottomrule\\
 \end{tabular}
 %
 \begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.4394} & {0.5717} & {0.6929}
 & {0.2079} & {0.1294} & {0.9695} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$ 
 & 0.4446 & 0.5948 & 0.6697
 & 0.1998 & 0.1211 & 0.9723
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.4422} & {0.6086} & {0.6588}
 & {0.2117} & {0.1484} & {0.9660} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.4538 & 0.6467 & 0.6131
 & 0.2151 & 0.1624 & 0.9630
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.2285} & {0.6749} & {0.7017}
 & {0.2983} & {0.9356} & {0.1889}
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.2188 & 0.6529 & 0.7252
 & 0.3026 & 0.9362 & 0.1788
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.1982} & {0.6500} & {0.7336}
 & {0.2832} & {0.9367} & {0.2060} 
 \\
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.1730 & 0.6110 & 0.7725
 & 0.2812 & 0.9340 & 0.2203
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS 
 & {0.8688} & {0.4666} & {0.1658}
 & {0.9315} & {0.3285} & {0.1559} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.8686 & 0.4689 & 0.1602
 & 0.9319 & 0.3300 & 0.1504
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.8747} & {0.4550} & {0.1668}
 & {0.9354} & {0.3172} & {0.1563} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.8742 & 0.4566 & 0.1654
 & 0.9352 & 0.3182 & 0.1552
 \\\bottomrule
 \end{tabular}
 \label{tab:Mixing1L}
 \caption{One-loop mixing matrix elements for TP2-5 when using the
 indicated versions of \NC\ and \NFH\ as specified in the text.}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_sm.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_sg.pdf}
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_hy.pdf}
 \caption{One-loop difference $\Delta m = m_h^{\NCs} - m_h^{\NFHs}$ at
   the  scales  $\MS$  (green)  and  $\mt$  (blue)  between  \NC\  and
   \NFH\  with the  reparametrisation to  $\alpha_{G_F}$ (bright)  and
   $\alpha{(\MZ)}$ (dark).
 %% \htC{Maggie: Why do  we show the result for TP1  here, although we
 %%   said that we will not consider it any more?  E.g. in Table 6 you
 %%   do not give any values for TP2. We have to unify this.}
 }
 \label{fig:resOB1L}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The   differences    between   the   one-loop   results,    shown   in
\reffi{fig:resOB1L}  by  \htPD{light  green bars},  are  much  smaller
compared to  observed differences at  the two-loop level.   They never
exceed 1.0~\gev\ for all masses in  all scenarios. In order to account
for this  well understood difference  we now employ a  modification of
\NFH,  where the  the  electromagnetic coupling  is reparametrised  to
$\alpha{(\MZ)}$.  \htMM{In  order to account for  this well understood
  difference   between    the   two   renormalisation    schemes   for
  $\alpha_{G_F}$  and  $\alpha{(\MZ)}$ up  to  one-loop  order we  now
  employ  a  modification  of  \NFH,  where  the  the  electromagnetic
  coupling is reparametrised to $\alpha{(\MZ)}$.  \\ Or: We now employ
  a modification  of \NFH, where  the the electromagnetic  coupling is
  reparametrised to  $\alpha{(\MZ)}$.  The  reparametrisation accounts
  for the  well understood difference between  the two renormalisation
  schemes  for  $\alpha_{G_F}$  and  $\alpha{(\MZ)}$  up  to  one-loop
  order.}  \\  The remaining differences are  thus electroweak effects
that are formally of two-loop  and higher-orders. The mass predictions
for this version are given in \refta{tab:resOB1L}, where the described
reparametrised      version       of      \NFH\       is      labelled
``\NFHs\   $\alpha{(\MZ)}$''.  When   compared  to   the  results   of
``\NCs\  OS'' at  the scale  $\MS$ the  results of  the reparametrised
version  ``\NFHs\  $\alpha{(\MZ)}$'' are  in  better  or equally  well
agreement as the results of the previous version ``\NFHs'' without the
reparametrisation.  \htC{Maggie: Strictly speaking for TP3 and TP5 and
  the SM-like  Higgs the agreement  has become  a tiny bit  worse! Ok,
  maybe we can ignore this.}  This can  be seen by the dark green bars
in \reffi{fig:resOB1L}.  For the  comparison at $Q  = \MTO$,  shown as
blue bars in  \reffi{fig:resOB1L} for the SM-like Higgs  boson also an
improvement   is  achieved   by   the   reparametrization  of   $\al$.
\htC{Maggie: No,  not for TP4! We  have to comment on  this.}  For the
other  two  Higgs  bosons  the  result is  less  conclusive.   In  the
scenarios TP3 and TP4  the reparametrisation to $\alpha{(\MZ)}$ yields
a worse  agreement \htMM{\sout{with the  result of ``\NCs\  OS''}} for
the the two heavier Higgs-fields at the scale $\mt$.  \htC{Maggie: For
  TP3 the 'getting  worse' in the difference is tiny.  If we call this
  worse here, we have to do so  also for the SM-like Higgs at $M_S$ in
  TP3 and  TP5!  And we did  not even mention the  'getting worse' for
  the SM-like  Higgs at  $m_t$ for TP4.}   The mentioned  two-loop and
higher-order  effects  from  the  charge renormalisation  seem  to  be
\htMM{\sout{enhanced} more important} in these cases.

\htC{Maggie: {\bf Very important:} We have to comment on the mixing
  angles. Otherwise the table has to be taken off. In a paper you
  should never give tables or plots on which you do not comment.}

In order to verify that the observed differences between the versions
``\NCs\ OS'' and ``\NFHs\ $\alpha{(\MZ)}$'' are indeed explained by
two-loop and higher-order effects from the reparametrisation
procedure, we compared the predictions of the two versions in the
MSSM-limit of the TP scenarios. In the MSSM-limit, where $\lambda =
\kappa \rightarrow 0$, the renormalisation of $\alpha$ drops out as
well as the reparametrisation \htC{Maggie: Don't you mean to say that
  $\alpha$ drops out?}. We found that in the MSSM-limit both
codes agree within the level of $\approx~10~\mev$ for all masses.
\htC{Maggie: And how can the remaining 10 MeV be explained?}

The reparametrisation to $\alpha{(\MZ)}$ in \NFH\ \htMM{overall} yields a better
agreement with \NC. The effect on the mass prediction for the SM-like
Higgs, however, is much smaller than some of the large differences
observed for the two-loop mass prediction in \reffi{fig:total}. 
\htC{Maggie: Don't you mean Fig. 2?}
In the subsequent sections a comparison between \NC\ and \NFH\htMM{,
  where in the latter $\alpha$ has been} reparametrised
to $\alpha{(\MZ)}$, will be performed at the two-loop level in order to
identify the differences that are not caused by the renormalisation of
the electromagnetic coupling constant $\alpha$.



%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
 \scriptsize \centering
 \begin{tabular}{llcccccccccc}
 &
 & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
 & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
 \\\toprule
 &$Q$ 
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 & $\MS$ & $\mt$& $\MS$ & $\mt$
 \\\midrule\midrule
 \multirow{2}[4]{*}{$h_1$} & \NCs\ $\als$ mod
 & \bf 114.65 & --- 
 & \it 89.76 & \it 88.82 & \bf 125.13 & \bf 126.73 & \it 117.68 & \it 117.70
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \bf 114.65 & ---
 & \it 89.72 & \it 89.31 & \bf 125.56 & \bf 125.74 & \it 118.31 & \it 117.77
 \\
 \midrule
 \midrule
 \multirow{2}[4]{*}{$h_2$} & \NCs\ $\als$ mod
 & \it 5951.36 & --- 
 & \bf 123.98 & \bf 125.91 & \it 142.98 & \it 142.76 & \bf 122.87 & \bf 123.60
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \it 5951.36 & --- 
 & \bf 124.26& \bf 124.88 & \it 142.98 & \it 142.59 & \bf 122.81 & \bf 123.08
 \\
 \midrule
 \midrule
 \multirow{2}[4]{*}{$h_3$} & \NCs\ $\als$ mod
 & 6370.77 & --- & 652.29 & 652.70 & 467.76 & 467.36 & 627.14 & 628.72
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & 6370.90 & --- & 652.29 & 652.81 & 467.43 & 467.61 & 626.73 & 628.84
 \\\bottomrule
 \end{tabular}
 \caption{Masses for the \cp-even scalars for TP2--5 when using
 modified versions of \NC\ in the OS option \NCs\ \OS\ (denoted
 shortly by \NCs) and \NFH\ (\NFHs). Both codes are modified to use
 the identical numerical value of $\als$. In \NFH\ the
 reparametrisation to $\alpha{(\MZ)}$ (\htMM{\sout{\NFH\
     $\alpha{(\MZ)}$} \NFHs\ $\alpha{(\MZ)}$}) is
 used. The values correspond to the two-loop result obtained with
 the OS renormalisation scheme for the top/stop-sectors. The
 masses for the SM-like scalar are written in bold fonts, those for
 the singlet-like scalar in italics.
}
 \label{tab:resASmod}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
\scriptsize \centering
\begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.1034} & {0.9946} & {0.0004}
 & {0.2242} & {0.2136} & {0.9509} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.1034 & 0.9946 & 0.0004
 & 0.2229 & 0.2270 & 0.9480
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {---} & {---} & {---}
 & {0.2233} & {0.2202} & {0.9495} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & {---} & {---} & {---}
 & 0.2342 & 0.2610 & 0.9365
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.0096} & {0.0006} & {1.0000}
 & {0.2757} & {0.9219} & {0.2721}
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.0092 & 0.0005 & 1.0000
 & 0.2751 & 0.9183 & 0.2846
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {---} & {---} & {---}
 & {0.2661} & {0.9234} & {0.2767} 
 \\
 & & \NFHs\ $\alpha(\MZ)$
 & {---} & {---} & {---}
 & 0.2566 & 0.9125 & 0.3185
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.9946} & {0.1034} & {0.0096}
 & {0.9347} & {0.3232} & {0.1478} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.9946 & 0.1034 & 0.0092
 & 0.9352 & 0.3243 & 0.1423
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {---} & {---} & {---}
 & {0.9377} & {0.3145} & {0.1476} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & {---} & {---} & {---}
 & 0.9377 & 0.3149 & 0.1467
 \\\bottomrule\bottomrule\\
\end{tabular}
%
\begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.4837} & {0.7636} & {0.4276}
 & {0.1411} & {0.7294} & {0.6694} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.4872 & 0.8045 & 0.3398
 & 0.3319 & 0.6217 & 0.7094
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {0.4766} & {0.7877} & {0.3905}
 & {0.3382} & {0.6915} & {0.6383} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.4779 & 0.8321 & 0.2813
 & 0.3476 & 0.7708 & 0.5339
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.0683} & {0.4542} & {0.8883}
 & {0.3318} & {0.6022} & {0.7261}
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.0270 & 0.3751 & 0.9266
 & 0.1379 & 0.7120 & 0.6885
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {0.0421} & {0.4232} & {0.9051}
 & {0.0922} & {0.6507} & {0.7537} 
 \\
 & & \NFHs\ $\alpha(\MZ)$
 & 0.0122 & 0.3266 & 0.9451
 & 0.0482 & 0.5540 & 0.8311
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.8725} & {0.4589} & {0.1675}
 & {0.9327} & {0.3245} & {0.1570} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.8729 & 0.4606 & 0.1611
 & 0.9332 & 0.3264 & 0.1506
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {0.8781} & {0.4478} & {0.1685}
 & {0.9365} & {0.3138} & {0.1564} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.8783 & 0.4482 & 0.1662
 & 0.9364 & 0.3147 & 0.1554
 \\\bottomrule
 \end{tabular}
 \label{tab:Mixing2L}
\caption{Two-loop mixing matrix elements for TP2-5 when using the
  indicated versions of \NC\ and \NFH\ as specified in the
  text. \htC{RG: Ich denke in tab 8 haben wir bei TP5 und \NC\ das
    falsche Higgs als SM-like, oder? Maggie: Wenn man das nimmt, das
    am n\"achsten bei 125 GeV ist, dann nicht. Kann es sein, dass hier
  die Mischungsmatrixelemente verwechselt wurden. Andererseits sind
  sie sowieso f\"ur $h_1$ und $h_2$ in den Singulett Komponenten etwa
  gleich gro{\ss}.}
}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Treatment of the strong coupling constant \boldmath{$\als$}}
\label{sec:AsTreatment}

In the following we analyze the effects of the different treatment of
$\als$ in both codes. In \refta{tab:resASmod} the mass predictions at
\order{\alt\als} are given for the case that \NC\ is modified such,
that always the hard-coded \MSbar-value of the strong coupling at the
scale \MTO, $\als^{\MSbar}{(\MTO)} = 0.10697$ as obtained with the
routines of~\cite{Chetyrkin:2000yt}, is used. The results of \NFH\ are
not affected by this procedure, since $\als^{\MSbar}{(\MTO)}$ is the
standard value that is used. The modified version of \NC\ is labelled
``\NCs\ $\als$ mod'' in the following. \htSH{As discussed above, for
 \NFH\ we continue to use the version reparametrized to $\al(\MZ)$.}
The graphical representation of
the differences is depicted in \reffi{fig:asMod}.
When both codes use the same numerical value of
$\als$ a better agreement with much smaller relative differences
between their mass predictions can be observed. The differences
between the mass predictions never exceed 1.5~\gev, \htC{Maggie: 1.1?}
and mostly stay 
below $0.5~\gev$ for all masses in all TP-scenarios. In the MSSM-limit
we found again agreement within $\approx 10~\mev$
between the codes \htMM{now} at \order{\alt\als}.

%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/asMod_sm.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/asMod_sg.pdf}
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/asMod_hy.pdf}
 \caption{Difference $\Delta{m} = m_h^{\NCs\ \alpha_s\ \text{mod}} - m_h^{\NFHs}$ between
 the Higgs masses of the SM-like, singlet-like and heavy Higgs at
 the two-loop level calculated at the scales \MS\ and \MTO.}
 \label{fig:asMod}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We conclude that the main source of the observed difference is the
different treatment of the strong coupling constant $\als$ (see
\refta{tab:DiffNcNfhVanilla}). Although the renormalisation
prescription and scale dependence of $\als$ represents an effect
formally of three-loop order, their effects on the Higgs mass
predictions can be sizeable \htC{PD: Citations for effect in MSSM...?}.
\htSH{The corresponding mixing matrix elements are given in
\refta{tab:Mixing2L}. We can see that \ldots}\htC{SH: $\to$ PD?!}

%% \htC{MM: The claim 'much' better is not true for
%% the heavy Higgs. This should be rephrased. Question: Where is the
%% fair blue bar for TP1 in the heavy Higgs plot? PD: It's zero, I will
%% add a comment in the description of the plot.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{MSSM-Approximation beyond one-loop in \NFH}

In \NFH\ the NMSSM contributions beyond one-loop are approximated by
the respective corrections from the MSSM at present.%
\footnote{\htSH{They will be replaced by the NMSSM calculations once they are
    available in the required scheme.}}%
~At 
\order{\alt\als} this has the disadvantage that the genuine NMSSM
contributions are missing, as will be discussed below. On the other
hand, it is known that other higher-order corrections beyond
\order{\alt\als} can have a sizable impact on the light \cp-even
Higgs-boson mass that can easily be of \order{5 \gev}~\cite{Drechsel:2016jdg}. 
These contributions \htSH{consist of further leading and subleading two-loop
  corrections~\cite{Brignole:2001jy,Brignole:2002bz,Degrassi:2002fi,Dedes:2003km,Borowka:2014wla,Borowka:2015ura}
as well as the resummation of large logarithms to all orders for high SUSY
mass scales~\cite{Hahn:2013ria,Bahl:2016brp}. They} are already
approximately taken into account in \NFH. 



%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L2L_sm_short.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L2L_sg_short.pdf}
 \;\;
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L2L_hy_short.pdf}
 \\
 %
 \caption{$\Delta{m}_h^{\rm appr} = \Delta{m}_h^{\rm 2L} -
 \Delta{m}_h^{\rm 1L}$: size of the effect of the MSSM-approximation
 employed at \order{\alt\als} in \NFH. The used version of
 \NFH\ employs the reparametrisation to $\alpha{(\MZ)}$. }
 \label{fig:ApproxMSSM}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


At \order{\alt\als} the missing genuine NMSSM
two-loop corrections in \NFH\ give rise to differences to \NC. In
order to estimate their impact we compare the two-loop mass
predictions between '\NCs\ $\als$ mod' and '\NFHs\ $\alpha{(\MZ)}$' 
given in \refta{tab:resASmod}. The effect of the MSSM-approximation
$\Delta{m}^{\rm appr}_h$ can be obtained obtained by
%
\begin{align}
 \Delta{m}^{\rm appr}_h = \Delta{m}^{\rm 2L}_h - \Delta{m}^{\rm 1L}_h,
\end{align}
\noindent
where the $\Delta{m}^{n{\rm L}}_h$ are the differences between the
result of \NC\ and \NFH\ at the $n$-th loop order obtained from the
results given in tabs.~\ref{tab:resOB1L} (where we take the '\NFHs\
$\alpha{(\MZ)}$' value for \NFH) and~\ref{tab:resASmod}. By
this construction the effects of the fixed-order reparametrisation are
separated from the effects of the MSSM-approximation. The results of
these comparisons are given in \reffi{fig:ApproxMSSM}. As expected the
approximation has the largest effects for the scenarios TP3--5 with
large values of $\lambda$. For the SM-like Higgs-field
$\Delta{m}_h^{\rm appr}$ \htSH{does not exceed $\pm 750 (500)~\mev$
at the scale $\MS (\mt)$, shown as dark green (blue) bars.
For the singlet-like Higgs-boson it stays below $750\,\mev$ for both scales,
and for heavy Higgs fields its size can reduces to values of
below $\pm 200\,\mev$.}
This resembles the expected impact of the approximation as
described in ref.~\cite{Drechsel:2016jdg}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> sections/codes__Ramona_Gr__ber_s_conflicted_copy_2016-11-26_.tex <==
\section{The two codes: \NC\ and \FH}
\label{sec:Codes}

%\htPD{PD:     Should    we     rather    ``copy''     the    structure
%  of~\cite{Staub:2015aea} for this section?}
%
%\htPD{
%\begin{itemize}
%\item describe differences
%\item for summary see tab.~\ref{tab:DiffNcNfhVanilla}
%\end{itemize}
%}

\htSH{In this section we will give a brief overview about the higher-order
corrections to Higgs-boson masses included in \FH\ and \NC, including the
different renormalization schemes employed.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Incorporation of higher-order contributions}
\label{sec:calcho}

The masses of the \cp-even Higgs  bosons are obtained from the complex
poles of  the full propagator  matrix.  The inverse  propagator matrix
for    the     three    \cp-even     Higgs    bosons     $h_i$    from
eq.~\eqref{eq:MixMatrices} is a $3 \times 3$ matrix that reads
%
\begin{align}
  \Delta^{-1}{\left(k^2\right)} = \mathi
  \left[k^2\mathds{1} - \mathbf{M}_{hh}
    + \mathbf{\hat{\Sigma}}_{hh}{\left(k^2\right)}
    \right].
\end{align}
\noindent
Here  $\mathbf{M}_{hh}$ denotes  the diagonalised  mass matrix  of the
\cp-even Higgs fields at  tree level, and $\mathbf{\hat{\Sigma}}_{hh}$
denotes the matrix of their renormalised self-energy corrections.  The
three complex poles of the propagator in the \cp-even Higgs sector are
given  by the  values  of  the external  momentum  $k$  for which  the
determinant of the inverse propagator-matrix vanishes,
%
\begin{align}
  \det\left[
    \Delta^{-1}{\left(k^2\right)}
    \right]_{k^2 = m_{h_i}^2 - \mathi \Gamma_{h_i} m_{h_i}} \overset{!}{=} 0
  , \ i \in \{1,2,3\}.
\end{align}
\noindent
The real parts  of the three poles are identified  with the the square
of the Higgs-boson masses $m_{h_i}$  in the \cp-even sector, while the
complex  parts   include  their  total  widths   $\Gamma_{h_i}$.   The
renormalised   self-energy   matrix  $\mathbf{\hat{\Sigma}}_{hh}$   at
one-loop  order is  evaluated in  \NC~\cite{Ender:2011qh, Graf:2012hh}
and  \FH~\cite{Drechsel:2016jdg}  by  taking  into  account  the  full
contributions     from    the     NMSSM \htSH{(differences in the
  renormalization schemes are discussed below)}.      
At two-loop order
\NC includes the leading (S)QCD corrections from
the top/stop sector of \order{\alt\als} in the 
NMSSM~\htRG{\cite{Muhlleitner:2014vsa}},
while \FH\ includes all available  corrections from the MSSM, that are
included   in   the   MSSM-version   of   \FH~\cite{Heinemeyer:1998yj,
  Hahn:2009zz,   Heinemeyer:1998np,   Degrassi:2002fi,   Frank:2006yh,
  Hahn:2013ria, Bahl:2016brp, feynhiggs-www}, as an approximation%
\footnote{Updates beyond  the \FH\ version  2.10.2, that was  used for
  this   comparison,   also   include  momentum   dependent   two-loop
  contributions \htRG{\cite{Borowka:2014wla, Degrassi:2014pfa}} 
\htSH{and improved resummations of large logarithmic
  corrections~\cite{Bahl:2016brp}. These updates are not relevant for the
  comparison between the two codes up to \order{\alt\als}.}}%
,
%
\begin{subequations}
  \label{eq:SEapprox}
  \begin{align}
    \NC:\
    &\mathbf{\hat{\Sigma}}_{hh}^{\tt NC}{\left(k^2\right)}
    \htSH{=}
    \left.
    \mathbf{\hat{\Sigma}}^{(\text{1L})}_{hh}{\left(k^2\right)}
    \right|^{\text{NMSSM}} +
    \left.
    \mathbf{\hat{\Sigma}}^{(\text{2L})}_{hh}{\left(k^2\right)}
    \right|_{k^2=0}^{\text{NMSSM }\mathcal{O}{\left(\alpha_t\alpha_s\right)}},
    \\
    \FH:\
    &\mathbf{\hat{\Sigma}}_{hh}^{\tt FH}{\left(k^2\right)}
    \htSH{=}
    \left.
    \mathbf{\hat{\Sigma}}^{(\text{1L})}_{hh}{\left(k^2\right)}
    \right|^{\text{NMSSM}} +
    \Big[
      \left.\mathbf{\hat{\Sigma}}^{(\text{2L})}_{hh}{\left(k^2\right)}
      \right|^{\mathcal{O}{\left(\alpha_t\alpha_s\right)}}+
      \order{\left(\alpha_b \alpha_s, \alpha_t^2,\alpha_t\alpha_b\right)}
    \nonumber\\
 & \mbox{}\hspace{80mm} + \mbox{resummed logs} \Big]_{k^2=0}^{\text{MSSM}}.
  \end{align}
\end{subequations}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Renormalisation Scheme: Higgs- and electroweak sectors}
\label{sec:RenSchemeHEW}

\htRG{\sout{In order to derive the  counterterms entering the one-loop
corrections 
to the Higgs-boson masses}} The  independent parameters appearing in the
linear   and    bilinear   terms    of   the   Higgs    potential   in
\refeq{eq:HiggsPot}  have to  be  renormalised \htSH{in order to evaluate
  higher-order corrections to the Higgs-boson masses}.  \NC\  and \FH\  offer
different  choices  for the  set  of  independent parameters  and  the
applied renormalisation schemes.  \htPD{Reference to explanation.} For
the presented  work the  set of common  independent parameters  in the
Higgs sector for the comparison of the OS versions of both codes
reads
%
\begin{align}
  \underbrace{\MZ,\ \MW,\ \MHp, T_{\htSH{\phi_i}},\ \TB}_{\text{on-shell}},\
  \underbrace{\lambda,\ \mueff,\ \kappa,\ \Ak}_{\DRbar},
\end{align}
\noindent
with the applied  renormalisation scheme. 
\htRG{In \NC\ the scheme can be varied: if $\MHp$
is set as input parameter, it will be renormalised OS, if instead the 
trilinear soft-SUSY breaking parameter $A_{\lambda}$ is used as input 
parameter it is renormalised $\DRbar$.}
% When the  \DRbar\ option for
%the  Higgs sector  is used  in \NC,  the charged  Higgs mass  \MHp\ is
%exchanged  with  the  trilinear   breaking  parameter  \Al,  which  is
%subsequently  renormalised \DRbar.   
The gauge-boson  masses, however,
are  still  renormalised OS  and  the  tadpole coefficients  are
renormalised to vanish.
% when the \DRbar\ option for the Higgs sector is chosen.

\htRG{Using the former option, $\MHp$ as input,} up to the one-loop level
 the  two codes differ only by their treatment
of  the  renormalisation of  the  coupling  constant $\alpha$  in  the
electromagnetic  sector. While  for \NC\  $\alpha$ is  renormalised to
$\alpha(\MZ)$, \FH\ employs a  dependent renormalisation scheme 
\htSH{(employing a \DRbar\ renormalization of $v$)} with a
subsequent  reparametrisation~\cite{Drechsel:2016jdg}   to  the  value
$\alpha_{G_F}$, derived  from the Fermi  constant $G_F$ \htSH{(to match
  exactly the MSSM evaluation)}.  In  the \htSH{Higgs-boson mass calculation
  in the MSSM-limit} the  charge renormalisation  constant  drops  out at  the
discussed levels of  the calculation and thus its impact  is an effect
genuine to the NMSSM. 
\htSH{The differences between \NC\ and \FH\ in the higher-order contribution
  to the Higgs-boson self-energies are summarized in
  \refta{tab:DiffNcNfhVanilla}.}

\begin{table}[h]
  \centering
  \begin{tabular}{lcccc}
    & \NC & & \NFH
    \\\toprule
    \multirow{2}{*}{1-loop} & 
    $\alpha{\left(M_Z\right)}$ & \multirow{2}{*}{$\leftrightarrow$} & $\alpha_{G_F}$
    \\
    & renormalised &  & reparametrised
    \\
    \midrule
    \multirow{2}{*}{2-loop} & 
    $\alpha_s^{\overline{\text{DR}}}{\left(Q_{\rm input}\right)}$ & 
    $\leftrightarrow$ &
    $\alpha^{\overline{\text{MS}}}_s{\left(m_t\right)}$
    \\
    &
    \multirow{2}{*}{NMSSM $\mathcal{O}{\left(\alpha_t\alpha_s\right)}$} &
    \multirow{2}{*}{$\leftrightarrow$} &
    MSSM $\mathcal{O}{\left(\alpha_t\alpha_s,\alpha_t^2, \alpha_b\alpha_s, \alpha_t\alpha_b\right)}$
    \\
    & & &
    + \htSH{\sout{SM}} resummed logarithms
    \\\bottomrule
  \end{tabular}
  \caption{Calculational  differences between  the original  (vanilla)
    versions of \NC\ and \NFH\ as  used for this comparison.  The used
    values  for the  electromagnetic and  strong couplings  is stated,
    where $\alpha_{G_F}$ denotes the electromagnetic coupling constant
    calculated from the Fermi constant.}
  \label{tab:DiffNcNfhVanilla}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Renormalisation Scheme: Top/Stop Sector}
\label{sec:RenSchemeTST}

\htPD{as previous section, but for top/stop sector}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Treatment of QCD corrections}

In   \NC\    the   $\DRbar$-value   of   strong    coupling   constant
$\alpha_s^{\DRbar}$  is  calculated at  the  input  scale $Q$  of  the
parameters  specified   in  the  SLHA  input-file   with  the  results
of~\cite{Chetyrkin:2000yt,Baer:2002ek}.      \htPD{In    \NFH\     the
  $\MSbar$-value  of strong  coupling constant  $\alpha_s^{\MSbar}$ is
  calculated  at  the  scale  \MTO\,  independent  of  the  parameters
  specified in the SLHA input-file.}%
\footnote{\htSH{This has partially be changed starting from version 
\texttt{2.12.1}.}}%
~In both codes the obtained value
is consequently used for the calculation of the on-shell shift and the
evaluation of the two-loop contributions to the Higgs mass.


==> sections/files19Nov/NMSSM19Nov.tex <==
\section{The relevant NMSSM sectors }
\label{sec:NMSSM}
The  superpotential   of  the  NMSSM  for  the   third  generation  of
fermions/sfermions reads
%
\begin{align}
\label{eq:superpot}
  W = 
  \yt \left(\hat{H}_2\cdot \hat{Q}_3 \right)\hat{u}_3 
  - Y_d \left(\hat{H}_1\cdot \hat{Q}_3 \right)\hat{d}_3 
  - Y_\tau \left(\hat{H}_1\cdot \hat{L}_3 \right)\hat{e}_3
  + \lambda \hat{S} \left(\hat{H}_2 \cdot \hat{H}_1 \right) + \frac{1}{3} \kappa \hat{S}^3,
\end{align}
\noindent
with the quark and lepton superfields $\hat{Q}_3$, $\hat{u}_3$,
$\hat{d}_3$, $\hat{L}_3$ and $\hat{e}_3$, exemplary for
 all three generations, and the Higgs superfields $\hat{H}_1$,
$\hat{H}_2$ and $\hat{S}$. The $\SUL$-invariant product is
denoted by a dot. Since we will focus on the \cp-conserving
 NMSSM, all the Yukawa-type  couplings $\yt$, $Y_d$, $Y_\tau$,
 $\lambda$ and $\kappa$ can be chosen as real parameters. The
scalar  components $H_1$,  $H_2$  and $S$  of the  Higgs
doublet and singlet superfields can be  decomposed into  \cp-even  and
\cp-odd neutral  scalars 
$\phi_x$ and $\chi_x$ ($x=1,2,s$), respectively, and charged
states $\phi^\pm_i$ ($i=1,2$). After expansion around their
 vacuum expectation values (vevs) $\langle H_i \rangle$ ($i=1,2$) and
 $\langle S \rangle$, they read
%
\begin{align}
 H_1 = \begin{pmatrix} \langle H_1\rangle +\frac{1}{\sqrt{2}}\left(
  \phi_1 \pm i\chi_1\right) \\ 
  \pm \phi_1^- \end{pmatrix} , \quad
 H_2 = \begin{pmatrix} \phi_2^+ \\ \langle H_2 \rangle + \frac{1}{\sqrt{2}}\left(\phi_2+i\chi_2\right) \end{pmatrix} , \quad
 S = \langle S \rangle +\frac{1}{\sqrt{2}}\left( \phi_s+i\chi_s\right) .
\end{align}
\noindent
The plus or minus signs in the doublet $H_1$ refer to the conventions
used in \NC\ and \NFH, respectively. Due to
\cp-conservation the vevs are real. Since $\hat{S}$ transforms as
a singlet, the $D$-terms remain identical to the ones from the MSSM.
Compared to the \cp-conserving  MSSM the superpotential of the
\cp-conserving NMSSM contains additional dimensionless parameters
$\lambda$ and $\kappa$, while the $\mu$-term is absent. This term is
effectively generated via the vacuum expectation-value of the singlet
field,
%
\begin{align}
 \mueff = \lambda \left<S\right> .
\end{align}
\noindent
It should be noted that there are two common conventions for
defining the vacuum expectation values, 
$\left<S\right> = v_s/\sqrt{2}$ and 
$\left|\left<H_i\right>\right|  = v_i/\sqrt{2}$, or 
$\left<S\right> = v_s$ and $\left|\left<H_i\right>\right| = v_i$,
respectively. Both are allowed
by the SLHA conventions~\cite{Allanach:2008qq, Skands:2003cj}.  The
latter convention is used by \FH, while the first is used by \NC. As
in the MSSM it is convenient to define the ratio
%
\begin{align}
 \tb = \frac{v_2}{v_1} .
\end{align}
\noindent
Soft SUSY-breaking in the NMSSM gives rise to the in the \cp-conserving case
real trilinear soft SUSY-breaking parameters $A_\lambda$ and $A_\kappa$, as
well as to the 
soft-breaking mass term $m_S^2$ of the scalar singlet field, so
 that together with the soft SUSY-breaking mass terms $m_1$ and $m_2$
for the doublet fields we have
%
\begin{align}
 \mathcal{L}_{\text{soft}} = 
 - m_1^2 H_{1i}^\dagger H_{1i} - m_2^2 H_{2i}^\dagger H_{2i} - m_S^2 |S|^2 
 - \left[
  \lambda A_\lambda S \left(H_2 \cdot H_1\right) + \frac{1}{3} \kappa A_\kappa S^3
  + \text{h.c.}
  \right]
\end{align}
\noindent
The Higgs potential $V_H$ can be written in powers of the fields,
%
\begin{align}
 \label{eq:HiggsPot}
 &V_H =
 \ldots - T_{\phi_1} \phi_1 - T_{\phi_2} \phi_2 - T_{\phi_S} \phi_s \\
 &\quad + \frac{1}{2} \begin{pmatrix} \phi_1,\phi_2, \phi_s \end{pmatrix}
 \mathbf{M}_{\phi\phi} \begin{pmatrix} \phi_1 \\ \phi_2 \\ \phi_s \end{pmatrix} +
 %
 \frac{1}{2} \begin{pmatrix} \chi_1, \chi_2, \chi_s \end{pmatrix}
 \mathbf{M}_{\chi\chi}
 \begin{pmatrix} \chi_1 \\ \chi_2 \\ \chi_s \end{pmatrix} +
 %
 \begin{pmatrix} \phi^-_1,\phi^-_2 \end{pmatrix}
 \mathbf{M}_{\phi^\pm\phi^\pm}
 \begin{pmatrix} \phi^+_1 \\ \phi^+_2 \end{pmatrix} + \ldots,
 \nonumber
\end{align}
\noindent
where the coefficients bilinear in the fields are the mass matrices
$\text{\textbf{M}}_{\phi\phi}$,  $\text{\textbf{M}}_{\chi\chi}$  and
$\text{\textbf{M}}_{\phi^\pm\phi^\pm}$. 

For the \cp-conserving case the mixing into the mass and \cp\
eigenstates can be described at
 lowest order by the following unitary transformations
%
\begin{align}
 \label{eq:MixMatrices}
 \begin{pmatrix} h_1 \\ h_2 \\ h_3 \end{pmatrix}
 = \mathbf{U}_{e(0)}
 \begin{pmatrix} \phi_1 \\ \phi_2 \\ \phi_s \end{pmatrix}, \quad
 \begin{pmatrix} A_1 \\ A_2 \\ G^0 \end{pmatrix}
 = \mathbf{U}_{o(0)}
 \begin{pmatrix} \chi_1 \\ \chi_2 \\ \chi_s \end{pmatrix}, \quad
 \begin{pmatrix} H^\pm \\ G^\pm \end{pmatrix}
 = \mathbf{U}_{c(0)}
 \begin{pmatrix} \phi^\pm_1 \\ \phi^\pm_2 \end{pmatrix} .
\end{align}
\noindent
The new fields correspond to the five neutral Higgs bosons $h_i$ and
$A_j$, the charged pair $H^\pm$, and the Goldstone bosons $G^0$ and
$G^\pm$. The matrices $\mathbf{U}_{\{e,o,c\}(0)}$ transform the Higgs
fields such that the mass matrices are diagonalised at tree level,
%
\begin{align}
 \mathbf{M}_{hh} =
 \mathbf{U}_{e(0)} \mathbf{M}_{\phi\phi} \mathbf{U}_{e(0)}^\dagger
 ,\
 \mathbf{U}_{o(0)} \mathbf{M}_{\chi\chi} \mathbf{U}_{o(0)}^\dagger
 ,\
 \mathbf{U}_{c(0)} \mathbf{M}_{\phi^\pm\phi^\pm} \mathbf{U}_{c(0)}^\dagger.
\end{align}
%
%\htC{RG: Later on we don't connect the $U$ to $Z$.  Furthermore, it
% seems to me that the $U$ is defined as the opposite of the mixing
% matrix in SLHA. I think it would be more clear if we redefine $U\to
% U^{\dagger}$. PD: Conventions should be now fine with
% SLHA according to arXiv:0801.0045 eq.~(62), just with a dagger
% instead of transpose.}


==> sections/files19Nov/calculation19Nov.tex <==
\begin{table}[h]
  \scriptsize \centering
  \begin{tabular}{llcccccccccc}
    &
    & \multicolumn{2}{c}{TP1} & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
    & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
    \\\toprule
    & $Q$ & $\MS$ & $\mt$ & $\MS$ & $\mt$ & $\MS$ & $\mt$
    & $\MS$ & $\mt$ & $\MS$ & $\mt$
    \\\midrule\midrule
    \multirow{2}[4]{*}{$h_1$} 
    & \NCs\ \OS
    & \bf 121.84 & \bf 113.47 & \bf 120.42 & --- 
    & \it 89.92 & \it 88.81 & \bf 126.44 & \bf 126.65 & \it 119.54 & \it 117.63
    \\\cmidrule{2-12}
    & \NFHs
    & \bf 115.70 & \bf 113.20 & \bf 114.12 & ---
    & \it 89.67 & \it 89.36 & \bf 126.17 & \bf 126.29 & \it 118.47 & \it 117.95
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_2$} 
    & \NCs\ \OS
    & \it 1797.45 & \it 1797.57 & \it 5951.36 & --- 
    & \bf 126.16 & \bf 125.80 & \it 143.32 & \it 142.73 & \bf 124.44 & \bf 123.51
    \\\cmidrule{2-12}
    & \NFHs
    & \it 1797.45 & \it 1797.62 & \it 5951.36 & --- 
    & \bf 124.55 & \bf 125.02 & \it 143.11 & \it 142.68 & \bf 122.93 & \bf 123.10
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_3$} 
    & \NCs\ \OS
    & 2755.73 & 2752.14 & 6370.77 & --- & 652.60 & 652.70 & 467.89 & 467.35 & 627.18 & 628.72
    \\\cmidrule{2-12}
    & \NFHs
    & 2755.79 & 2752.25 & 6370.85 & --- & 652.17 & 652.65 & 467.10 & 467.33 & 626.59 & 628.76
    \\\bottomrule
  \end{tabular}
 \caption{Masses for the \cp-even scalars for TP1-5 when using the
 indicated versions of \NC\ and \NFH\ as specified in
 \refse{sec:outofthebox}. %
 The masses of the SM-like scalar are written in bold fonts, those
 of the singlet-like scalar in italics.}
  \label{tab:resOB}
\end{table}

\section{Predictions for masses and mixing matrices of the \cp-even Scalars}
\label{sec:Results}

In this section we analyze the differences in the prediction for the
\cp-even Higgs boson masses and mixing matrices from \NFH\ and \NC. We
start by a comparison of the ``out-of-the-box'' results including the
corrections up to \order{\alt\als}, where sizable differences show
up. In order to understand the origin of these differeces we then
perform a comparison at the one-loop level, where we find that part of
the differences can be attributed to the different renormalization of
the electroweak sector in the two codes. After ``removing'' this
difference we continue with an analysis at the two-loop level, where
we investigate the effect of the strong coupling constant and the
genuine NMSSM corrections to the Higgs boson self-energies. Finally we
compare the results obtained with the OS version of \NC\ with the
\DRbar\ calculation. The various sources of differences between the
calculation are important ingrediences for a reliable estimate of the
intrinsic uncertainties in the Higgs boson mass and mixing matrix
calculations in the NMSSM

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{``Out-of-the-box'' results}
\label{sec:outofthebox}

In the first step of our comparison the masses and mixing matrices of
the \cp-even Higgs-sector are evaluated in the TP scenarios. For the
results of \NC\ we used the ``out-of-the-box'' version with the
on-shell renormalisation scheme for the top/stop sector and the
charged Higgs mass (see \refse{sec:drbaros}), labelled
``\NCs\ OS''. For \NFH\ we used the ``out-of-the-box'' version, but
included only the two-loop corrections of \order{\alt\als}, labelled
\NFHs. The obtained numerical results for the masses are given in
\refta{tab:resOB}, the results for the mixing-matrix elements, see
\refeq{Uh}, are given in \refta{tab:originalZH13_A}.
%
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
 \scriptsize \centering
 \begin{tabular}{lllccccccccc}
 & & & \multicolumn{3}{c}{TP1} & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$ \MS$}
 & \NCs\ \OS 
 & {0.1039} & {0.9946} & {0.0076}
 & {0.1034} & {0.9946} & {0.0004}
 & {0.2127} & {0.1753} & {0.9613}
 \\ 
 & & \NFHs
 & 0.1039 & 0.9946 & 0.0071
 & 0.1034 & 0.9946 & 0.0004
 & 0.2134 & 0.2064 & 0.9549
 \\\cmidrule{2-12}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.1006} & {0.9949} & {0.0074}
 & {---} & {---} & {---} 
 & {0.1881} & {0.1016} & {0.9769}
 \\ 
 & & \NFHs 
 & 0.1006 & 0.9949 & 0.0071
 & {---} & {---} & {---}
 & 0.2245 & 0.2264 & 0.9478
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$ \MS$}
 & \NCs\ \OS
 & {0.0076} & {0.0068} & {0.9999}
 & {0.0096} & {0.0006} & {1.}
 & {0.2854} & {0.9297} & {0.2327}
 \\ 
 & & \NFHs
 & 0.0071 & 0.0064 & 1.
 & 0.0090 & 0.0005 & 1.
 & 0.2820 & 0.9228 & 0.2625
 \\\cmidrule{2-12}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.0079} & {0.0066} & {0.9999}
 & {---} & {---} & {---}
 & {0.2925} & {0.9437} & {0.1545}
 \\
 & & \NFHs
 & 0.0072 & 0.0064 & 1.
 & {---} & {---} & {---}
 & 0.2656 & 0.9216 & 0.2831
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.9946} & {0.1040} & {0.0068}
 & {0.9946} & {0.1034} & {0.0096}\
 & {0.9345} & {0.3238} & {0.1477}
 \\ 
 & & \NFHs 
 & 0.9946 & 0.1039 & 0.0064
 & 0.9946 & 0.1034 & 0.009
 & 0.9354 & 0.3253 & 0.1388
 \\\cmidrule{2-12}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.9949} & {0.1007} & {0.0072}
 & {---} & {---} & {---}
 & {0.9376} & {0.3148} & {0.1478}
 \\
 & & \NFHs 
 & 0.9949 & 0.1006 & 0.0065
 & {---} & {---} & {---}
 & 0.9376 & 0.3153 & 0.1467
 \\\bottomrule\bottomrule\\
 \end{tabular}
 %
 \\
 %
 \begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.4852} & {0.7639} & {0.4255}
 & {0.2709} & {0.3426} & {0.9092}
 \\ 
 & & \NFHs 
 & 0.4873 & 0.8022 & 0.3448
 & 0.3540 & 0.7764 & 0.5214
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.4765} & {0.8549} & {0.2053}
 & {0.0785} & {0.6226} & {0.7786}
 \\ 
 & & \NFHs
 & 0.4788 & 0.8104 & 0.3377
 & 0.3390 & 0.7204 & 0.6051
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.0679} & {0.4522} & {0.8893}
 & {0.2390} & {0.8813} & {0.4076}
 \\ 
 & & \NFHs
 & 0.0334 & 0.3775 & 0.9254
 & 0.0564 & 0.5387 & 0.8406
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.0526} & {0.2608} & {0.9640}
 & {0.3418} & {0.7169} & {0.6077}
 \\
 & & \NFHs
 & 0.0171 & 0.3761 & 0.9264
 & 0.0819 & 0.6181 & 0.7818
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS 
 & {0.8718} & {0.4604} & {0.1676}
 & {0.9325} & {0.3254} & {0.1569}
 \\ 
 & & \NFHs 
 & 0.8726 & 0.4625 & 0.1571
 & 0.9335 & 0.3270 & 0.1469
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.8776} & {0.4485} & {0.1691}
 & {0.9365} & {0.3138} & {0.1565}
 \\ 
 & & \NFHs
 & 0.8778 & 0.4493 & 0.1662
 & 0.9372 & 0.3146 & 0.1505
 \\\bottomrule
 \end{tabular}
 %
 \caption{Absolute values for the mixing matrix elements of the
 \cp-even scalar sector for TP1-5 when using the indicated versions
 of \NC\ and \NFH\ as specified in the text. \htC{SH: check
 relative signs between codes}}
 \label{tab:originalZH13_A}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


For the identification of the singlet-like field we follow the
procedure applied in~\cite{Staub:2015aea}, where the field $h_i$ with
the largest singlet-admixture \ZH{i3} is identified with the
dominantly singlet-like field.

%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_sm.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_singlet.pdf}
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/total_heavy.pdf}
 \caption{Difference $\Delta{m} = m_h^{\NCs} - m_h^{\NFHs}$ between
 the Higgs masses of the SM-like, singlet-like and heavy Higgs at
 the two-loop level calculated at the scales \MS\ and \MTO. }
 \label{fig:total}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In \reffi{fig:total} the difference $\Delta{m} = m_h^{\NCs} -
m_h^{\NFHs}$ between the mass predictions obtained with the codes
``\NCs\ OS'' and ``\NFHs'' are shown. All values are given for two
input scales $Q$, the SUSY mass scale $Q = \MS$ in darker bars and the
top-quark mass scale $Q= \MTO = 172.9~\gev$ in lighter bars.


When comparing the Higgs masses obtained with \NFH\ and \NC%% \ with the
, we find that for the SM-like field the difference between the mass
predictions of both codes can be larger than
6~\gev\ for the scenarios TP1 and TP2 and the evaluation
at the high scale $M_S$. For the evaluations at the low scale $\mt$,
however, the differences between the codes do not exceed
1~\gev\ for all scenarios. %
The difference between the masses of the heaviest fields, which are
always doublet-like in all TP-scenarios, remain relatively small with
less than 1.3~\gev. For scenarios with a singlet-like
field that is heavier than the SM-like field the absolute
difference between the mass predictions for the singlet-like
field remains below 1~\gev, while for a lighter
singlet-field the differences can be as large as
1.9~\gev. The mixing matrix elements obtained by the two
codes agree within $\approx 2\%$ for the scenarios TP1-3%%

. For TP4 and TP5 significant differences can be observed between the
two results, with differences of up to $\approx~40\%$.

In general, we find that the differences for mixing matrix elements
seem be by far larger than for the mass prediction, where the relative
difference never exceeded 5\%. This is in particular the case for TP4
and TP5, where we have large singlet admixtures to the SM-like Higgs
field with a mass around 125~\gev. In this case we even find a factor
of two differences in the mixing matrix elements. In these scenarios
the Higgs masses and mixing matrices seem to be very sensitive to
changes of the parameters. We remark that this can lead to different
conclusions whether a parameter point is excluded or not by LHC data.

The observed differences between the mass predictions obtained at the
two-loop level appear to be unusually large, especially for the
comparison at the high scale \MS. In the following we will analyze the
differences in more detail, starting with a discussion of the chosen
test-point TP1 and a study of the diffferences at the one-loop level.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{The test point TP1}

In \refta{tab:resOB} very large differences between the mass
prediction in the MSSM-like scenario TP1 can be found when comparing
the results for both MSSM-like \cp-even Higgs fields obtained with the
same code at either the scale $\MS$ or \MTO. They can be as large as
$\approx 8.5~\gev$ for the SM-like scalar and \NC\ and $\approx
55~\gev$ for the heavy scalar and both codes. These different results
at two different scales may at first sight be somewhat surprising
since the physical situation before and after the evolution of the
parameters of the scenario is naively expected to be identical. We
found that the large, absolute difference between the predictions at
either the scale \MTO\ or $\MS$ is a result of the parameter evolution
performed by {\tt FlexibleSUSY}. In this specific scenario the
gluino-mass parameter $M_3$ at the high scale $\MS$ is very large
compared to the remaining mass spectrum. Thus for a correct parameter
evolution from $\MS$ down to \MTO\ the heavy gluino should be
decoupled consistently~\cite{Muhlleitner:2008yw}. If the heavy gluino
is not decoupled consistently, the obtained low-scale scenario does
not correspond to the physics situation described by the parameters at
the high scale. The comparison of the Higgs masses for ``TP1'' at both
scales thus do not describe the difference between the two
calculations but a difference between two distinct physical
scenarios%%
\footnote{It is important to note that this behaviour is unrelated to
 the choice of the renormalisation scheme in the calculation. This
 has also been observed for calculations using only
 \DRbar\ methods~\cite{Braathen:2016mmb}. \htC{PD: Cite also Georg's
 talk?}}% .

We found also that the parameters obtained at \MTO\ define a scenario
that is highly sensitive to variations of the stop parameters. This is
especially true for $A_t$, which is large compared to the other
soft-breaking parameters of the scenario. For example, at the low
scale \MTO\ changes of $\left|\Delta{A_t}\right| \approx 100~\gev$
\htC{MM: Do you change At at the high or at the low scale here by 100
 GeV?} can yield a change of the mass of the lightest field of
$|\Delta{m_{h_1}}| \approx 2~\gev$.

Since the observed effects are independent of the Higgs-mass
calculation itself (see \reffi{fig:Alg}), the scenario TP1 in the
present form is not viable for estimating theoretical
uncertainties. Thus we will omit this scenario in the following.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Renormalisation of \boldmath{$\alpha$}}
\label{sec:1LReparametrisation}

In order to disentangle the different effects in the renormalization,
coupling constants and higher order corrections, we start by comparing
the one-loop results for the Higgs-boson masses and mixing
matrices. Here we use the versions '\NCs\ OS' and '\NFHs' as described
in the previous section, but restricted to the pure one-loop
contribution to the Higgs-boson self-energies. The only difference
between the calculatins stem from the different renormalisation
prescription of the electromagnetic coupling constant $\alpha$, see
\refta{tab:DiffNcNfhVanilla}. The numerical results for the \cp-even
Higgs-boson masses are given in \refta{tab:resOB1L}.

%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
 \scriptsize \centering
 \begin{tabular}{llcccccccc}
 &
 & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
 & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
 \\\toprule
 & $Q$ 
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 \\\midrule\midrule
 \multirow{3}[6]{*}{$h_1$} 
 & \NCs\ \OS
 & \bf 140.67 & ---
 & \it 90.47 & \it 90.12 & \bf 132.48 & \bf 134.10 & \it 120.93 & \it 120.57
 \\\cmidrule{2-10}
 & \NFHs
 & \bf 139.68 & ---
 & \it 90.30 & \it 89.98 & \bf 132.96 & \bf 133.42 & \it 120.82 & \it 120.51
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \bf 140.67 & ---
 & \it 90.38 & \it 89.96 & \bf 132.73 & \bf 133.22 & \it 120.91 & \it 120.53
 \\
 \midrule
 \midrule
 \multirow{3}[6]{*}{$h_2$} 
 & \NCs\ \OS
 & \it 5951.36 & --- 
 & \bf 136.35 & \bf 138.25 & \it 146.45 & \it 146.84 & \bf 135.56 & \bf 138.27
 \\\cmidrule{2-10}
 & \NFHs
 & \it 5951.36 & --- 
 & \bf 136.73 & \bf 137.04 & \it 146.82 & \it 146.05 & \bf 136.30 & \bf 137.06
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \it 5951.36 & --- 
 & \bf 136.74 & \bf 137.19 & \it 146.59 & \it 145.89 & \bf 136.32 & \bf 137.26
 \\
 \midrule
 \midrule
 \multirow{3}[6]{*}{$h_3$} 
 & \NCs\ \OS
 & 6370.75 & --- & 652.80 & 653.13 & 468.63 & 468.32 & 627.34 & 629.19
 \\\cmidrule{2-10}
 & \NFHs
 & 6370.83 & --- & 652.49 & 653.04 & 468.01 & 468.30 & 626.94 & 629.14
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & 6370.88 & --- & 652.62 & 653.18 & 468.37 & 468.60 & 627.08 & 629.23
 \\\bottomrule
 \end{tabular}
 \caption{One-loop masses for the \cp-even scalars for TP2--5 when
 using the indicated versions of \NC\ and \NFH\ as specified in the
 text. The masses of the SM-like scalar are written in bold fonts,
 those of the singlet-like scalar in italics.}
 \label{tab:resOB1L}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
 \scriptsize \centering
 \begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.1034} & {0.9946} & {0.0004}
 & {0.2048} & {0.1503} & {0.9672} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$ 
 & 0.1034 & 0.9946 & 0.0004
 & 0.1981 & 0.1443 & 0.9695
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {---} & {---} & {---}
 & {0.2048} & {0.1553} & {0.9664} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & {---} & {---} & {---}
 & 0.2054 & 0.1601 & 0.9655
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.0096} & {0.0006} & {1.0000}
 & {0.2935} & {0.9332} & {0.2071}
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.0092 & 0.0005 & 1.0000
 & 0.2971 & 0.9337 & 0.1997
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {---} & {---} & {---}
 & {0.2836} & {0.9356} & {0.2104} 
 \\
 & & \NFHs\ $\alpha{(\MZ)}$
 & {---} & {---} & {---}
 & 0.2837 & 0.9344 & 0.2153
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS 
 & {0.9946} & {0.1034} & {0.0096}
 & {0.9338} & {0.3263} & {0.1470} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$ 
 & 0.9946 & 0.1034 & 0.0092
 & 0.9341 & 0.3276 & 0.1421
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {---} & {---} & {---}
 & {0.9368} & {0.3172} & {0.1475} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & {---} & {---} & {---}
 & 0.9366 & 0.3182 & 0.1466
 \\\bottomrule\bottomrule\\
 \end{tabular}
 %
 \begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.4394} & {0.5717} & {0.6929}
 & {0.2079} & {0.1294} & {0.9695} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$ 
 & 0.4446 & 0.5948 & 0.6697
 & 0.1998 & 0.1211 & 0.9723
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.4422} & {0.6086} & {0.6588}
 & {0.2117} & {0.1484} & {0.9660} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.4538 & 0.6467 & 0.6131
 & 0.2151 & 0.1624 & 0.9630
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS
 & {0.2285} & {0.6749} & {0.7017}
 & {0.2983} & {0.9356} & {0.1889}
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.2188 & 0.6529 & 0.7252
 & 0.3026 & 0.9362 & 0.1788
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.1982} & {0.6500} & {0.7336}
 & {0.2832} & {0.9367} & {0.2060} 
 \\
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.1730 & 0.6110 & 0.7725
 & 0.2812 & 0.9340 & 0.2203
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ \OS 
 & {0.8688} & {0.4666} & {0.1658}
 & {0.9315} & {0.3285} & {0.1559} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.8686 & 0.4689 & 0.1602
 & 0.9319 & 0.3300 & 0.1504
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ \OS
 & {0.8747} & {0.4550} & {0.1668}
 & {0.9354} & {0.3172} & {0.1563} 
 \\ 
 & & \NFHs\ $\alpha{(\MZ)}$
 & 0.8742 & 0.4566 & 0.1654
 & 0.9352 & 0.3182 & 0.1552
 \\\bottomrule
 \end{tabular}
 \label{tab:Mixing1L}
 \caption{One-loop mixing matrix elements for TP2-5 when using the
 indicated versions of \NC\ and \NFH\ as specified in the text.}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_sm.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_sg.pdf}
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_hy.pdf}
 \caption{One-loop difference $\Delta m = m_h^{\NCs} - m_h^{\NFHs}$ at
 the scales $\MS$ (green) and $\mt$ (blue) between \NC\ and
 \NFH\ with the reparametrisation to $\alpha_{G_F}$ (bright) and
 $\alpha{(\MZ)}$ (dark).}
 \label{fig:resOB1L}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The differences between the one-loop results, shown in
\reffi{fig:resOB1L} by \htPD{light green bars}, are much smaller
compared to observed differences at the two-loop level. They never
exceed 1.0~\gev\ for all masses in all scenarios. % In order to
account for this well understood difference we now employ a
modification of \NFH, where the the electromagnetic coupling is
reparametrised to $\alpha{(\MZ)}$. The reparametrisation accounts for
the differences between the two renormalisation schemes for
$\alpha_{G_F}$ and $\alpha{(\MZ)}$ up to one-loop order. The remaining
differences are thus electroweak effects that are formally of two-loop
and higher-orders. The mass predictions for this version are given in
\refta{tab:resOB1L}, where the described reparametrised version of
\NFH\ is labelled ``\NFHs\ $\alpha{(\MZ)}$''. When compared to the
results of ``\NCs\ OS'' at the scale $\MS$ the results of the
reparametrised version ``\NFHs\ $\alpha{(\MZ)}$'' are in better or
equally well agreement than the results of the previous version
``\NFHs'' without the reparametrisation. This can be seen by the dark
green bars in \reffi{fig:resOB1L}. For the comparison at $Q = \MTO$,
shown as blue bars in \reffi{fig:resOB1L} for the SM-like Higgs boson
also an improvement is yielded by the reparametrization of $\al$. For
the other two Higgs bosons the result is less conclusive. In the
scenarios TP3 and TP4 the reparametrisation to $\alpha{(\MZ)}$ yields
a worse agreement with the result of ``\NCs\ OS'' for the the two
heavier Higgs-fields at the scale $\mt$. The mentioned two-loop and
higher-order effects from the charge renormalisation seem to be
enhanced in these cases.
%For TP5 the reparametrised version ``\NFHs\ $\alpha{(\MZ)}$'' has
%only a very small effect on the mass of the SM-like Higgs field at
%both $\MS$ and $\mt$. \htC{MM: I do not understand why at the scale
%$\MS$ the difference is larger after adapting to $\alpha (\MZ)$ I
%would have thought that the difference should always be smaller
%then. PD: Corrections from higher-orders than the reparametrisation
%can still influence the result (see ref.~\cite{Drechsel:2016jdg},
%sec. 2.3). They enter with the finite contribution of the charge
%renormalisations constant in the Thomson limit, which is increased
%for large renormalisations scales.}


In order to verify that the observed differences between the versions
``\NCs\ OS'' and ``\NFHs\ $\alpha{(\MZ)}$'' are indeed explained by
two-loop and higher-order effects from the reparametrisation
procedure, we compared the predictions of the two versions in the
MSSM-limit of the TP scenarios. In the MSSM-limit, where $\lambda =
\kappa \rightarrow 0$, the renormalisation of $\alpha$ drops out as
well as the reparametrisation. We found that in the MSSM-limit both
codes agree within the level of $\approx~10~\mev$ for all masses.

The reparametrisation to $\alpha{(\MZ)}$ in \NFH\ yields a better
agreement with \NC. The effect on the mass prediction for the SM-like
Higgs, however, is much smaller than some of the large differences
observed for the two-loop mass prediction in \reffi{fig:total}. In the
subsequent sections a comparison between \NC\ and \NFH\ reparametrised
to $\alpha{(\MZ)}$ will be performed at the two-loop level in order to
identify the differences that are not caused by the renormalisation of
the electromagnetic coupling constant $\alpha$.



%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
 \scriptsize \centering
 \begin{tabular}{llcccccccccc}
 &
 & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
 & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
 \\\toprule
 &$Q$ 
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 & $\MS$ & $\mt$& $\MS$ & $\mt$
 \\\midrule\midrule
 \multirow{2}[4]{*}{$h_1$} & \NCs\ $\als$ mod
 & \bf 114.65 & --- 
 & \it 89.76 & \it 88.82 & \bf 125.13 & \bf 126.73 & \it 117.68 & \it 117.70
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \bf 114.65 & ---
 & \it 89.72 & \it 89.31 & \bf 125.56 & \bf 125.74 & \it 118.31 & \it 117.77
 \\
 \midrule
 \midrule
 \multirow{2}[4]{*}{$h_2$} & \NCs\ $\als$ mod
 & \it 5951.36 & --- 
 & \bf 123.98 & \bf 125.91 & \it 142.98 & \it 142.76 & \bf 122.87 & \bf 123.60
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & \it 5951.36 & --- 
 & \bf 124.26& \bf 124.88 & \it 142.98 & \it 142.59 & \bf 122.81 & \bf 123.08
 \\
 \midrule
 \midrule
 \multirow{2}[4]{*}{$h_3$} & \NCs\ $\als$ mod
 & 6370.77 & --- & 652.29 & 652.70 & 467.76 & 467.36 & 627.14 & 628.72
 \\\cmidrule{2-10}
 & \NFHs\ $\alpha(\MZ)$
 & 6370.90 & --- & 652.29 & 652.81 & 467.43 & 467.61 & 626.73 & 628.84
 \\\bottomrule
 \end{tabular}
 \caption{Masses for the \cp-even scalars for TP2--5 when using
 modified versions of \NC\ in the OS option \NCs\ \OS\ (denoted
 shortly by \NCs) and \NFH\ (\NFHs). Both codes are modified to use
 the identical numerical value of $\als$. In \NFH\ the
 reparametrisation to $\alpha{(\MZ)}$ (\NFH\ $\alpha{(\MZ)}$) is
 used. The values correspond to the two-loop result obtained with
 the on-shell renormalisation scheme for the top/stop-sectors. The
 masses for the SM-like scalar are written in bold fonts, those for
 the singlet-like scalar in italics.
%\htRG{ARE WE SURE THAT FOR TP5 AT
% SCALE MT THE LIGHTEST IS SM-LIKE? CHECK!} \htPD{PD: According to
% tab.34 in our working pdf it is correct as it stands.}
%\htRG{Ok, let's verify this once we add the mixing matrix elements.}}
}
 \label{tab:resASmod}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
\scriptsize \centering
\begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.1034} & {0.9946} & {0.0004}
 & {0.2242} & {0.2136} & {0.9509} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.1034 & 0.9946 & 0.0004
 & 0.2229 & 0.2270 & 0.9480
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {---} & {---} & {---}
 & {0.2233} & {0.2202} & {0.9495} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & {---} & {---} & {---}
 & 0.2342 & 0.2610 & 0.9365
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.0096} & {0.0006} & {1.0000}
 & {0.2757} & {0.9219} & {0.2721}
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.0092 & 0.0005 & 1.0000
 & 0.2751 & 0.9183 & 0.2846
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {---} & {---} & {---}
 & {0.2661} & {0.9234} & {0.2767} 
 \\
 & & \NFHs\ $\alpha(\MZ)$
 & {---} & {---} & {---}
 & 0.2566 & 0.9125 & 0.3185
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.9946} & {0.1034} & {0.0096}
 & {0.9347} & {0.3232} & {0.1478} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.9946 & 0.1034 & 0.0092
 & 0.9352 & 0.3243 & 0.1423
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {---} & {---} & {---}
 & {0.9377} & {0.3145} & {0.1476} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & {---} & {---} & {---}
 & 0.9377 & 0.3149 & 0.1467
 \\\bottomrule\bottomrule\\
\end{tabular}
%
\begin{tabular}{lllcccccc} 
 & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
 \\\toprule
 $i$ & $Q$ &
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 & \ZHabs{i1} & \ZHabs{i2} & \ZHabs{i3}
 \\\midrule\midrule
 \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.4837} & {0.7636} & {0.4276}
 & {0.1411} & {0.7294} & {0.6694} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.4872 & 0.8045 & 0.3398
 & 0.3319 & 0.6217 & 0.7094
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {0.4766} & {0.7877} & {0.3905}
 & {0.3382} & {0.6915} & {0.6383} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.4779 & 0.8321 & 0.2813
 & 0.3476 & 0.7708 & 0.5339
 \\\midrule\midrule
 \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.0683} & {0.4542} & {0.8883}
 & {0.3318} & {0.6022} & {0.7261}
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.0270 & 0.3751 & 0.9266
 & 0.1379 & 0.7120 & 0.6885
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {0.0421} & {0.4232} & {0.9051}
 & {0.0922} & {0.6507} & {0.7537} 
 \\
 & & \NFHs\ $\alpha(\MZ)$
 & 0.0122 & 0.3266 & 0.9451
 & 0.0482 & 0.5540 & 0.8311
 \\\midrule\midrule
 \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
 & \NCs\ $\als$ mod
 & {0.8725} & {0.4589} & {0.1675}
 & {0.9327} & {0.3245} & {0.1570} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.8729 & 0.4606 & 0.1611
 & 0.9332 & 0.3264 & 0.1506
 \\\cmidrule{2-9}
 & \multirow{2}[0]{*}{$\mt$}
 & \NCs\ $\als$ mod
 & {0.8781} & {0.4478} & {0.1685}
 & {0.9365} & {0.3138} & {0.1564} 
 \\ 
 & & \NFHs\ $\alpha(\MZ)$
 & 0.8783 & 0.4482 & 0.1662
 & 0.9364 & 0.3147 & 0.1554
 \\\bottomrule
 \end{tabular}
 \label{tab:Mixing2L}
\caption{Two-loop mixing matrix elements for TP2-5 when using the
  indicated versions of \NC\ and \NFH\ as specified in the text. \htC{RG: Ich denke in tab 8 haben wir bei TP5 und \NC\ das falsche Higgs als SM-like, oder?}
}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Treatment of the strong coupling constant \boldmath{$\als$}}
\label{sec:AsTreatment}

%Even after accounting for the different renormalisation prescription
%for the electromagnetic coupling constant the difference between the
%mass predictions seems to be unusually large. This is in particular
%true for the MSSM-like scenario\htPDd{s TP1 and} TP2. In these
%scenarios genuine NMSSM-effects are expected to be suppressed due to
%very small values of $\lambda$. 
In the following we analyze the effects of the different treatment of
$\als$ in both codes. In \refta{tab:resASmod} the mass predictions at
\order{\alt\als} are given for the case that \NC\ is modified such,
that always the hard-coded \MSbar-value of the strong coupling at the
scale \MTO, $\als^{\MSbar}{(\MTO)} = 0.10697$ as obtained with the
routines of~\cite{Chetyrkin:2000yt}, is used. The results of \NFH\ are
not affected by this procedure, since $\als^{\MSbar}{(\MTO)}$ is the
standard value that is used. The modified version of \NC\ is labelled
``\NCs\ $\als$ mod'' in the following. \htSH{As discussed above, for
 \NFH\ we continue to use the version reparametrized to $\al(\MZ)$.}
The graphical representation of
the differences is depicted in \reffi{fig:asMod}.
When both codes use the same numerical value of
$\als$ a better agreement with much smaller relative differences
between their mass predictions can be observed. The differences
between the mass predictions never exceed 1.5~\gev, and mostly stay
below $0.5~\gev$ for all masses in the TP-scenarios. In the MSSM-limit
we found again an agreement within $\approx 10~\mev$ between the codes
at \order{\alt\als}.

%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/asMod_sm.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/asMod_sg.pdf}
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/asMod_hy.pdf}
 \caption{Difference $\Delta{m} = m_h^{\NCs\ \alpha_s\ \text{mod}} - m_h^{\NFHs}$ between
 the Higgs masses of the SM-like, singlet-like and heavy Higgs at
 the two-loop level calculated at the scales \MS\ and \MTO.}
 \label{fig:asMod}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We conclude that the main source of the observed difference is the
different treatment of the strong coupling constant $\als$ (see
\refta{tab:DiffNcNfhVanilla}). Although the renormalisation
prescription and scale dependence of $\als$ represents an effect
formally of three-loop order, their effects on the Higgs mass
predictions can be sizeable \htC{PD: Citations for effect in MSSM...?}.
\htSH{The corresponding mixing matrix elements are given in
\refta{tab:Mixing2L}. We can see that \ldots}\htC{SH: $\to$ PD?!}

%% \htC{MM: The claim 'much' better is not true for
%% the heavy Higgs. This should be rephrased. Question: Where is the
%% fair blue bar for TP1 in the heavy Higgs plot? PD: It's zero, I will
%% add a comment in the description of the plot.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{MSSM-Approximation beyond one-loop in \NFH}

In \NFH\ the NMSSM contributions beyond one-loop are approximated by
the respective corrections from the MSSM (to be replaced by the NMSSM
calculations once they are available in the required scheme). At
\order{\alt\als} this has the disadvantage that the genuine NMSSM
contributions are missing, as will be discussed below. On the other
hand, it is known that other higher-order corrections beyond
\order{\alt\als} can have a sizable impact on the light \cp-even
Higgs-boson mass that can easily be of \order{5
 \gev}~\cite{Drechsel:2016jdg}. These contributions are already
approximately taken into account in \NFH.


%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L2L_sm_short.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L2L_sg_short.pdf}
 \;\;
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L2L_hy_short.pdf}
 \\
 %
 \caption{$\Delta_{h}^{\rm appr} = \Delta{m}_h^{\rm 2L} -
 \Delta{m}_h^{\rm 1L}$: size of the effect of the MSSM-approximation
 employed at \order{\alt\als} in \NFH. The used version of
 \NFH\ uses the reparametrisation to $\alpha{(\MZ)}$. }
 \label{fig:ApproxMSSM}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


As mentioned above, at \order{\alt\als} the missing genuine NMSSM
two-loop corrections in \NFH\ give rise to differences to \NC. In
order to estimate their impact we compare the two-loop mass
predictions between '\NCs\ $\als$ mod' and '\NFHs\ $\alpha{(\MZ)}$'
given in \refta{tab:resASmod}. The effect MSSM-approximation
$\Delta{m}^{\rm appr}_h$ can be obtained obtained by
%
\begin{align}
 \Delta{m}^{\rm appr}_h = \Delta{m}^{\rm 2L}_h - \Delta{m}^{\rm 1L}_h,
\end{align}
\noindent
where the $\Delta{m}^{n{\rm L}}_h$ are the differences between the
result of \NC\ and \NFH\ at the $n$-th loop order obtained from the
results given in tabs.~\ref{tab:resOB1L} and~\ref{tab:resASmod}. By
this construction the effects of the fixed-order reparametrisation are
separated from the effects of the MSSM-approximation. The results of
these comparisons are given in \reffi{fig:ApproxMSSM}. As expected the
approximation has the largest effects for the scenarios TP3--5 with
large values of $\lambda$. For the SM-like Higgs-field
$\Delta{m}_h^{\rm appr}$ never exceeds approx. $\pm 750~\mev$ at the
scale $\mt$ (dark blue bars). For the singlet-like and heavy Higgs
fields its size can increase to values of approx. $\pm
1.25~\gev$. This resembles the expected impact of the approximation as
described in ref.~\cite{Drechsel:2016jdg}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newpage
%\subsection{Genuine NMSSM Effect from Charge Renormalisation}
%
%\htC{ PD: Sven told me that the effect of the charge renormalisation
% can be obtained from the one-loop calculation alone. I'm not
% entirely convinced, since already in the MSSM the effect is
% different when studied at the one- or two-loop order. The expected
% MSSM uncertainty of $\approx 0.5~\gev$ can only be seen at the
% 2-loop level in the MSSM-limit. At which order should we obtaine the
% correct uncertainty?}\\ \htC{SH: Ich denke, dieses Kapitel m\"ussen
% wir nochmal diskutieren. Hier habe ich nichts ge\"andert. \\PD: Wie
% ich es verstehe, kann diese Sektion weg, da sie auf die Abschaetzung
% der Unsicherheiten abzielt. Das sollte Punkt 3 der Minutes vom
% 2.11. sein.}
%
%\vspace{1cm}
%\noindent
%The renormalisation of the electromagnetic coupling $\alpha$ induces a
%one-loop effect in the NMSSM, while the same procedure induces a
%two-loop effect in the MSSM. In order to disentangle the MSSM-like
%two-loop effect from the genuine NMSSM one-loop effect, the TP
%scenarios at both scales $\MS$ and $\mt$ are also evaluated in their
%MSSM limit, where $\lambda = \kappa \rightarrow 0$. % The difference
%$\Delta{m} = \Delta{m}^{\rm \NCs}_h - \Delta{m}^{\rm \NFHs}_h$
%\htC{MM: How is $\Delta{m}^{\rm \NCs}_h$, how is $\Delta{m}^{\rm
% \NFHs}_h$ defined?} in the MSSM-limit is shown as \htPD{light
% green} bars in \reffi{fig:MSSMLimit} for the two MSSM-like
%fields. For the SM-like field the result obtained with $\alpha{(\MZ)}$
%generally yields a larger mass prediction compared to the result
%obtained with $\alpha_{G_F}$. The difference between both results
%amounts to approx. 500--750~\mega\electronvolt. \htC{MM: Are you
 %talking about the 2-loop results?} For the heavy field the
%difference remains well below $\pm 100~\mega\electronvolt$.
%%
%\begin{figure}[htb]
% \centering
% \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_sm_mssm.pdf%}
% \;\;
% \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/2L_sm_mssm.pdf%}
% \\
% \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/1L_hy_mssm.pdf%}
% \;\;
% \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/2L_hy_mssm.pdf%}
%%
% \caption{Difference between the results obtained with \NFH, utilising
% $\alpha_{G_F}$ and \NC, utilising $\alpha{(\MZ)}$, in the
% MSSM-limit and in the NMSSM. In the MSSM-limit the difference is
% obtained by $\Delta{m} = \Delta{m}^{\rm \NCs}_h - \Delta{m}^{\rm
% \NFHs}_h$. In the NMSSM the difference of the MSSM-approximation
% is also taken into account, $\Delta{m} = \Delta{m}^{\rm \NCs}_h -
% \Delta{m}^{\rm \NFHs}_h - \Delta{m}_h^{\rm appr}$. The green (blue)
% bars show the results at the scale $\MS$ ($\mt$).}
% \label{fig:MSSMLimit}
%\end{figure}
%
%The respective results $\Delta{m} = \Delta{m}^{\rm \NCs}_h -
%\Delta{m}^{\rm \NFHs}_h - \Delta{m}_h^{\rm appr}$ in the actual
%TP-scenarios are given in \reffi{fig:MSSMLimit} by \htPD{dark green}
%bars, where also the effect of the MSSM-approximation in \NFH\ is
%taken into account. For the MSSM-like scenario TP2 the effect of the
%renormalisation prescription of $\alpha$ remains very small. For the
%scenarios TP3--5 the result obtained with $\alpha_{G_F}$ seems to be
%increased compared to the result obtained with $\alpha{(\MZ)}$. For
%the SM-like field this effect is considerably larger at the high scale
%$\MS$, where it can lead to differences up to $-2.4~\gev$. At the low
%scale $\mt$ this effect is considerably smaller with
%200--750~\mega\electronvolt, with the larger effects for the scenarios
%TP4 and TP5 with a sizeable singlet-admixture of at least 30\%. The
%relative effect on the mass of the heavy field remains below 0.2\%.




==> sections/files19Nov/calculationNC19Nov.tex <==
\subsection{Comparison with \boldmath{\DRbar} calculation in \NC}\label{sec:DRbar}
The final step is now to compare between different
renormalisation schemes. So far,
we compared at the one-loop level the different renormalization of
  the electromagnetic coupling constant in \NC\ and \NFH, while at the
  two-loop level we have always used an OS renormalization.
\NC\ offers, however, also the possibility to compare between OS or
\DRbar\ renormalisation of the top/stop sector, affecting the
  \order{\alt\als} corrections.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
  \scriptsize \centering
  \begin{tabular}{llcccccccc}
    &
    & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
    & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
    \\\toprule
    & $Q$ & $\MS$ & $\mt$ & $\MS$ & $\mt$
    & $\MS$ & $\mt$ & $\MS$ & $\mt$
    \\\midrule\midrule
    \multirow{2}[4]{*}{$h_1$} 
    & \NCs\ \OS
    & \bf 120.42 & --- 
    & \it 89.92 & \it 88.81 & \bf 126.44 & \bf 126.65 & \it 119.54 & \it 117.63
    \\\cmidrule{2-10}
    & \NCs\ \DRbar
     & \bf 118.57 & ---
    & \it 90.17 & \it 88.94 & \bf 126.15 & \bf 125.90 & \it 119.86 & \it 118.56
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_2$} 
    & \NCs\ \OS
   & \it 5951.36 & --- 
    & \bf 126.16 & \bf 125.80 & \it 143.32 & \it 142.73 & \bf 124.44 & \bf 123.51
    \\\cmidrule{2-10}
    & \NCs\ \DRbar
    & \it 5951.36 & --- 
    & \bf 124.88 & \bf 124.86 & \it 142.38 & \it 142.16 & \bf 123.28 & \bf 125.20
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_3$} 
    & \NCs\ \OS
     & 6370.77 & --- & 652.60 & 652.70 & 467.89 & 467.35 & 627.18 & 628.72
    \\\cmidrule{2-10}
    & \NCs\ \DRbar
     & 6371.21 & --- & 652.44 & 652.65 & 467.39 & 467.03 & 626.97 & 628.75
    \\\bottomrule
  \end{tabular}
 \caption{Masses for the \cp-even scalars for TP2-5 when using the OS or respectively \DRbar\ renormalization in the top/stop sector. 
 The masses of the SM-like scalar are written in bold fonts, those
 of the singlet-like scalar in italics.}
 \label{tab:resDRbar}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \centering
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/OSvsDRbar_sm.pdf}
 \;\;
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/OSvsDRbar_sg.pdf}
 \\
 \includegraphics[width=.4\textwidth,width=.33\textheight]{plots/OSvsDRbar_hy.pdf}
 \caption{Difference   $\Delta{m}    =   m_h^{\NCs\   {\rm    OS}}   -
   m_h^{\NCs\   \DRbar}$   from  tab.~\ref{tab:resDRbar}.    For   TP2
   higher-order corrections to the mass  of the singlet-like field are
   suppressed due to the small value of $\lambda$.}
 \label{fig:total}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%Table%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
 \scriptsize
 \centering
 \begin{tabular}{crrrrrrrr}
 & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
 & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
 \\\toprule
% $Q$ & $1500$ & $172.9$ & $1500$ & $172.9$ & $1000$ & $172.9$
% & $750$ & $172.9$ & $1500$ & $172.9$
 $Q$ & $\MS$ & $\mt$ & $\MS$ & $\mt$
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 \\\midrule\midrule
$m_t^{\DRbar}$ & 136.7 & --- & 143.9 & 154.2 & 146.9 & 155.8 & 140.0 &  152.9
\\ \midrule
 $m_{\tilde{t}_1}^{\rm \DRbar}$ & $488.4$ & --- & $940.8$ & $1195$ & $671.8$ & $839.1$
 & $1503$ & $1548$
 \\\midrule
 $m_{\tilde{t}_2}^{\rm \DRbar}$ & $2509$ & --- & $1074$ & $1267$ & $845.3$ & $949.7$
 & $1509$ & $1591$
 \\\bottomrule
 \end{tabular}
 \caption{\DRbar\ top and stop masses in the TP2-5 scenarios obtained by the routines
 of \NC. 
}
 \label{tab:DRbarstopmasses}
\end{table}

%%%%%%%%%%Table%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
  \scriptsize \centering
  \begin{tabular}{lllcccccc}
    & & & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
    \\\toprule
    $i$ & $Q$ &
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    \\\midrule\midrule
    \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$ \MS$}
    & \NCs\ \OS  
    & {0.1034} & {0.9946} & {0.0004}
    & {0.2127} & {0.1753} & {0.9613}
    \\ 
    & & \NCs\ \DRbar\
    & 0.1034 & 0.9946 & 0.0004
    & 0.2189 & 0.1962 & 0.9558
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ \OS
    & {---} & {---} & {---} 
    & {0.1881} & {0.1016} & {0.9769}
    \\ 
    & & \NCs\ \DRbar\ 
    & {---} & {---} & {---}
    & 0.2237 & 0.2221 & 0.9490
    \\\midrule\midrule
    \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$ \MS$}
    & \NCs\ \OS
    & {0.0096} & {0.0006} & {1.}
    & {0.2854} & {0.9297} & {0.2327}
    \\&&  \NCs\ \DRbar\
    & 0.0095 & 0.0006 & 1.
    & 0.2802 & 0.9257 & 0.2542
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ \OS
    & {---} & {---} & {---}
    & {0.2925} & {0.9437} & {0.1545}
    \\
    & & \NCs\ \DRbar\
    & {---} & {---} & {---}
    & 0.2656 & 0.9230 & 0.2786
    \\\midrule\midrule
    \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ \OS
    & {0.9946} & {0.1034} & {0.0096}
    & {0.9345} & {0.3238} & {0.1477}
    \\ 
    & & \NCs\ \DRbar\
    & 0.9946 & 0.1034 & 0.0095
    & 0.9346 & 0.3235 & 0.1476
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ \OS
    & {---} & {---} & {---}
    & {0.9378} & {0.3144} & {0.1475}
    \\
    & & \NCs\ \DRbar\
    & {---} & {---} & {---}
   & 0.9378 & 0.3144 & 0.1475
    \\\bottomrule\bottomrule\\
  \end{tabular}
  %
  \\
 \begin{tabular}{lllcccccc} 
    & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
    \\\toprule
    $i$ & $Q$ &
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    \\\midrule\midrule
    \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ \OS
    & {0.4852} & {0.7639} & {0.4255}
    & {0.2709} & {0.3426} & {0.9092}
    \\ 
    & & \NCs\ \DRbar\
    & 0.4863 & 0.7790 & 0.3959
    & 0.2994 & 0.4536 & 0.8394
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ \OS
    & {0.4765} & {0.8549} & {0.2053}
    & {0.0785} & {0.6226} & {0.7786}
    \\ 
    & & \NCs\ \DRbar\
    & 0.4777 & 0.8098 & 0.3407
    & 0.3114 & 0.5379 & 0.7834
    \\\midrule\midrule
    \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ \OS
    & {0.0679} & {0.4522} & {0.8893}
    & {0.2390} & {0.8813} & {0.4076}
    \\ 
    & & \NCs\ \DRbar\
    & 0.0515 & 0.4267 & 0.9029
    & 0.2017 & 0.8298 & 0.5203
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ \OS
    & {0.0526} & {0.2608} & {0.9640}
    & {0.3418} & {0.7169} & {0.6077}
    \\
    & & \NCs\ \DRbar\
    & 0.0162 & 0.3796 & 0.9250
    & 0.1623 & 0.7822 & 0.6015
    \\\midrule\midrule
    \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ \OS 
    & {0.8718} & {0.4604} & {0.1676}
    & {0.9325} & {0.3254} & {0.1569}
    \\ 
    & & \NCs\ \DRbar\
    & 0.8723 & 0.4595 & 0.1674
    & 0.9326 & 0.3251 & 0.1569
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ \OS
    & {0.8776} & {0.4485} & {0.1691}
    & {0.9365} & {0.3138} & {0.1565}
    \\ 
    & & \NCs\ \DRbar\
    & 0.8784 & 0.4474 & 0.1682
    & 0.9363 & 0.3144 & 0.1563
    \\\bottomrule
  \end{tabular}
  %
 \caption{Absolute  values  for  the  mixing matrix  elements  of  the
 \cp-even scalar sector for TP2-5  
when using the OS renormalisation or respectively the \DRbar\ renormalisation 
of the top/stop sector within \NC.
  \label{tab:ZH13DRbar}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In tab.~\ref{tab:resDRbar} the neutral Higgs boson masses for TP2-5 for
\NC\ with OS renormalisation of the top/stop sector (first line) and
with \DRbar\ renormalisation (second line) of the top/stop sector can be
found.\footnote{\htRG{Note that wherever we give values at the scale $Q=m_t$ the numerical value of the scale is taken to be the top pole mass.}}
 They are are visualised in fig.~\ref{fig:total}.
\htRG{The values of the stop and top masses in the \DRbar\ scheme can be
found in tab.~\ref{tab:DRbarstopmasses}, the stop masses as obtained in the OS scheme in tab.~\ref{tab:OS}.} 


The first option is the one employed in tab.~\ref{tab:resOB}. 
As can be inferred from the table, the different renormalisation schemes
lead in general to differences of \order{1~\gev} with a maximum
difference of $1.9~\gev$.
The effects are of similar size for both the scale $Q = \MS$ and
$Q = \mt$ and strongest pronounced for the SM-like Higgs boson, 
which is most affected by the corrections of the top/stop sector as it has the largest $\phi_2$ component. 
The numerical differences between the different renormalization
schemes indicate the size of three-loop corrections of
\order{\alt\als^2}. However, one should keep in mind that also the
comparison of the different $\als$ values, as analyzed in
\refse{sec:AsTreatment}, indicate a somewhat larger higher-order
uncertainty. 


In tab.~\ref{tab:ZH13DRbar} the mixing matrix elements for the different
 options of the renormalization of the top/stop sector can be found. 
\htRG{For TP2 the renormalization scheme has basically no 
influence on the mixing matrix elements whereas for TP3-5 in some cases 
the renormalization scheme can change the mixing matrix 
elements by up to a factor of two. Such large differences occur however only for the
mixing matrix elements that are small and only at the scale $Q=\mt$. At $Q=\MS$
the change in the mixing matrix elements is maximally 30\%. For most of the matrix elements 
the change due to the renormalization scheme is well below 10\%.
 }



Finally,   we   also   want   to   follow   up   the   discussion   of
ref.~\cite{Staub:2015aea}.  Contrary  to our scenarios, where  we used
$\MHp$  as  input, in  ref.~\cite{Staub:2015aea}  $\Ala$  was used  as
input. This corresponds to  slightly different renormalization schemes
in \NC. If $\MHp$ is input,  the charged Higgs mass is renormalized OS
and subsequently  $\Ala$ is  determined from  the charged  Higgs mass,
whereas if  $\Ala$ is given  as input  it is renormalised  \DRbar.  In
tab.~\ref{tab:resAlam}  we show  values where  the input  is given  by
$\Ala$  (first line)  and  by  $\MHp$ (second  line).  The first  line
corresponds  to   the  "out-of-the-box"   \NC\  values  as   given  in
ref.~\cite{Staub:2015aea}.   The  effect   of  the   way  $\Ala$   (or
respectively  $\MHp$) is  renormalised  is small.  Only  for the  most
singlet-like Higgs boson it can exceed  1 GeV. \htC{Any idea why?} For
all  the other  Higgs boson  it  is always  well below  1~GeV, and  in
particular  for  the  SM-like  Higgs  boson it  is  at  the  level  of
\order{100~\mev}.  In tab.~\ref{tab:ZH13Alam} the values of the mixing
matrix elements  are given.  As for the  Higgs masses  the differences
between either input $\Ala$ or  $\MHp$ input is small. \htRG{Note that
  if  $\MHp$ is  input  in \NC\,  the  $\Ala$ in  the  output file  is
  determined from $\MHp$  at tree-level. This implies  that the $\Ala$
  in the output of the computation  with input $\MHp$ will differ from
  the $\Ala$ given in ref.~\cite{Staub:2015aea}.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
  \scriptsize \centering
  \begin{tabular}{llcccccccc}
    &
    & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
    & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
    \\\toprule
    & $Q$ & $\MS$ & $\mt$ & $\MS$ & $\mt$
    & $\MS$ & $\mt$ & $\MS$ & $\mt$
    \\\midrule\midrule
    \multirow{2}[4]{*}{$h_1$} 
    & \NCs\ $\Ala$
    & \bf 118.57 & --- 
    & \it 90.88 & \it 87.78 & \bf 126.37 & \bf 125.76 & \it 120.32 & \it 118.65
    \\\cmidrule{2-10}
    & \NCs\ $\MHp$
     & \bf 118.57 & ---
    & \it 90.17 & \it 88.94 & \bf 126.15 & \bf 125.90 & \it 119.86 & \it 118.56
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_2$} 
& \NCs\ $\Ala$
   & \it 5951.36 & --- 
    & \bf 124.86 & \bf 124.68 & \it 142.59 & \it 141.28 & \bf 123.14 & \bf 125.26
    \\\cmidrule{2-10}
    & \NCs\ $\MHp$
    & \it 5951.36 & --- 
    & \bf 124.88 & \bf 124.86 & \it 142.38 & \it 142.16 & \bf 123.28 & \bf 125.20
    \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{$h_3$} 
    & \NCs\ $\Ala$
     & 6371.31 & --- & 652.48 & 652.64 & 467.42 & 467.01 & 627.00 & 628.77
    \\\cmidrule{2-10}
    & \NCs\ $\MHp$
     & 6371.21 & --- & 652.44 & 652.65 & 467.39 & 467.03 & 626.97 & 628.75
    \\\bottomrule
  \end{tabular}
 \caption{Masses for the \cp-even scalars for TP2-5 when using the \DRbar\ 
renormalization in the top/stop sector for either $\Ala$ as input or $\MHp$. 
 The masses of the SM-like scalar are written in bold fonts, those
 of the singlet-like scalar in italics.}
  \label{tab:resAlam}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb!]
  \scriptsize \centering
  \begin{tabular}{lllcccccc}
    & & & \multicolumn{3}{c}{TP2} & \multicolumn{3}{c}{TP3}
    \\\toprule
    $i$ & $Q$ &
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    \\\midrule\midrule
    \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$ \MS$}
    & \NCs\ $\Ala$  
    & {0.1034} & {0.9946} & {0.0004}
    & {0.2177} & {0.1923} & {0.9569}
    \\ 
    & & \NCs\ $\MHp$
    & 0.1034 & 0.9946 & 0.0004
    & 0.2189 & 0.1962 & 0.9558
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ $\Ala$
    & {---} & {---} & {---} 
    & {0.2212} & {0.2142} & {0.9514}
    \\ 
    & & \NCs\ $\MHp$
    & {---} & {---} & {---}
    & 0.2237 & 0.2221 & 0.9490
    \\\midrule\midrule
    \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$ \MS$}
    & \NCs\ $\Ala$
    & {0.0095} & {0.0006} & {1.}
    & {0.2811} & {0.9265} & {0.2502}
    \\&&  \NCs\ $\MHp$
    & 0.0095 & 0.0006 & 1.
    & 0.2802 & 0.9257 & 0.2542
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ $\Ala$
    & {---} & {---} & {---}
    & {0.2677} & {0.9248} & {0.2705}
    \\
    & & \NCs\ $\MHp$
    & {---} & {---} & {---}
    & 0.2656 & 0.9230 & 0.2786
    \\\midrule\midrule
    \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ $\Ala$
    & {0.9946} & {0.1034} & {0.0095}
    & {0.9347} & {0.3234} & {0.1476}
    \\ 
    & & \NCs\ $\MHp$
    & 0.9946 & 0.1034 & 0.0095
    & 0.9346 & 0.3235 & 0.1476
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ $\Ala$
    & {---} & {---} & {---}
    & {0.9378} & {0.3145} & {0.1472}
    \\
    & & \NCs\ $\MHp$
    & {---} & {---} & {---}
    & 0.9378 & 0.3144 & 0.1475
    \\\bottomrule\bottomrule\\
  \end{tabular}
  %
  \\
 \begin{tabular}{lllcccccc} 
    & & & \multicolumn{3}{c}{TP4} & \multicolumn{3}{c}{TP5}
    \\\toprule
    $i$ & $Q$ &
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    & \ZHabs{i1} & \ZHabs{i2} &  \ZHabs{i3}
    \\\midrule\midrule
    \multirow{4}[4]{*}{$1$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ $\Ala$
    & {0.4869} & {0.7849} & {0.3832}
    & {0.2967} & {0.4433} & {0.8459}
    \\ 
    & & \NCs\ $\MHp$
    & 0.4863 & 0.7790 & 0.3959
    & 0.2994 & 0.4536 & 0.8394
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ $\Ala$
    & {0.4774} & {0.8045} & {0.3534}
    & {0.3129} & {0.5451} & {0.7778}
    \\ 
    & & \NCs\ $\MHp$
    & 0.4777 & 0.8098 & 0.3407
    & 0.3114 & 0.5379 & 0.7834
    \\\midrule\midrule
    \multirow{4}[4]{*}{$2$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ $\Ala$
    & {0.0447} & {0.4158} & {0.9084}
    & {0.2055} & {0.8354} & {0.5099}
    \\ 
    & & \NCs\ $\MHp$
    & 0.0515 & 0.4267 & 0.9029
    & 0.2017 & 0.8298 & 0.5203
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ $\Ala$
    & {0.0232} & {0.3906} & {0.9203}
    & {0.1594} & {0.7772} & {0.6088}
    \\
    & & \NCs\ $\MHp$
    & 0.0162 & 0.3796 & 0.9250
    & 0.1623 & 0.7822 & 0.6015
    \\\midrule\midrule
    \multirow{4}[4]{*}{$3$} & \multirow{2}[0]{*}{$\MS$}
    & \NCs\ $\Ala$
    & {0.8723} & {0.4594} & {0.1674}
    & {0.9326} & {0.3251} & {0.1568}
    \\ 
    & & \NCs\ $\MHp$
    & 0.8723 & 0.4595 & 0.1674
    & 0.9326 & 0.3251 & 0.1569
    \\\cmidrule{2-9}
    & \multirow{2}[0]{*}{$\mt$}
    & \NCs\ $\Ala$
    & {0.8784} & {0.4476} & {0.1678}
    & {0.9363} & {0.3144} & {0.1563}
    \\ 
    & & \NCs\ $\MHp$
    & 0.8784 & 0.4474 & 0.1682
    & 0.9363 & 0.3144 & 0.1563
    \\\bottomrule
  \end{tabular}
  %
 \caption{Absolute  values  for  the  mixing matrix  elements  of  the
 \cp-even scalar sector for TP2-5  
when using the \DRbar\ renormalisation
of the top/stop sector for either $\Ala$ as input or $\MHp$.
  \label{tab:ZH13Alam}
}
\end{table}

%% 




==> sections/files19Nov/conclusion19Nov.tex <==
\section{Conclusion}
\label{sec:conclusion}

We have analyzez the Higgs-boson masses and mixing matrices in the NMSSM
based on an on-shell (OS) renormalization, applying
in particular to the top/scalar top sector. We compared the
implementation of the OS calculations in the codes \NC\ and \NFH\ up to
\order{\alt\als} (neglecting further higher-order corrections
implemented in \NFH). Since the two codes are in principle doing the
calculation at the same level of accuracy, but with differences in the
renormalization and the coupling constants, differences should give an
indication of the size of unknown higher-order corrections. 

Our work can be seen as an extension of~\cite{Staub:2015aea},
where Higgs-boson mass calculations in different \DRbar\ codes had been
analyzed. Consequently, we employed the same scenarios (TP2 -- TP5) as
in~\cite{Staub:2015aea}. (Scenarios TP1 and TP6 are shown to be not
useful in our comparison of \NC\ and \NFH.) The scenarios are defined at
the original stop mass scale $\MS$. Since
diagrammatic calculations as implemented in \NC\ and \NFH\ are in 
general designed to evaluate the Higgs-boson sector at the electroweak
scale, we also evolved the TP scenarios down to the scale of the
top-quark mass in order. All evaluations have been done at those two scales.
At both scales the original \DRbar\ parameters have been converted to OS
parameters that are subsequently used as input for \NC\ and \NFH.

We started by an ``out-of-the-box'' comparison of the two codes and
found large differences of several GeV between the two codes. In order
to disentangle the origin of the differences we first concentrated on
the one-loop Higgs-boson self-energy contributions. While both codes
perform a full one-loop calculation, a difference in the renormalization
of the electromagnetic coupling constant~$\alpha$ exists between
\NC\ and \NFH. Reparametrizing \NFH\ to the value used by \NC\ reduced
the differences somewhat at the one-loop level. 

In a second step in the two-loop \order{\alt\als} corrections we
adjusted the strong coupling constant~$\als$ in \NC, where normally
$\als^{\DRbar}(Q)$ is employed, to $\als^{\MSbar}(\mt)$ as used by
\NFH. Although this difference is formally only of three-loop order,
this change improved the agreement between the two codes by several
GeV. The remaning differences of \order{0.5 \gev} can be seen as an
effect of the genuine NMSSM corrections in the \order{\alt\als}
corrections that are implemented in \NC, but not yet in
\NFH. Conversely, the corrections beyond \order{\alt\als} implemented in
\NFH, which are taken over from the MSSM and which have been
consistently neglected for this comparison can give contributions of
\order{5 \gev} to the SM-like Higgs-boson mass. 

In a final step we used the different renormalizations of the top/stop
sector that are implemented in \NC\ (but not in \NFH). We compared the
results of the OS renormalization (as obtained before) with the results
using a \DRbar\ renormalization in the top/stop sector. Difference of
\order{1 \gev} have been found, which indicate the size of missing
three-loop corrections of \order{\alt\als^2}. However, one should keep
in mind that the comparison of the different $\als$ values (see above)
indicate a somewhat larger higher-order uncertainty.
In order to make contact with~\cite{Staub:2015aea}, we also analyzed the
differences between $\MHp$ and $\Ala$ (as used in that analysis) as 
\DRbar\ inputs, which are two options in \NC. Here only very small
differences for the SM-like Higgs boson have been found.

The various sources of differences between the calculation are important
ingrediences for a reliable estimate of the intrinsic uncertainties in
the Higgs-boson mass and mixing matrix calculations in the NMSSM.
An estimate of the size of these higher-order corrections will be given
elsewhere. 



==> sections/files19Nov/introduction19Nov.tex <==
\section{Introduction}
\label{sec:Introduction}

%\begin{itemize}
%\item mention electroweak scale as preferred scale for diagrammatic
% calculations
%\item \htC{SH: what exactly do you want here?} \htPD{PD: Stress, that
% our calculations are expected to work well for not too high SUSY
% masses and at the (renormalisation) scale $m_{ew}$. Main reason is
% the accounting for large logarithms that might appear otherwise.
% That might be important for the non experts and distinguish our work
% further from the RGE calculations.}
%\end{itemize}

%\noindent
The experimental value of the mass of the detected Higgs
boson~\cite{CMS:2015kwa},
%
\begin{align}
 m_H = 125.09 \pm 0.21(\rm{stat.}) \pm 0.11(\rm{syst.})~\giga\electronvolt,
\end{align}
\noindent
has an uncertainty of at most several permille so that only four years 
after its discovery has become an electroweak precision observable. 
In order to make full use of this high-precision measurement every model
that makes a prediction for this quantity should ideally provide a result
with a similar precision.  
Furthermore, for a reliable calculation of the Higgs boson mass 
it is important to provide a solid estimate
for the theoretical uncertainty of the available prediction
Two different sources for theoretical  uncertainties exist in 
the Higgs-boson mass predictions. One are due to the experimental
uncertainties of the SM input parameters (``parametric uncertainties''), 
the other are unknown higher-order corrections in the
Higgs-boson mass calculation itself (``intrinsic uncertainties'').

Supersymmetry (SUSY) is one of the most attractive solutions to several
shortcomings of the Standard Model (SM). It can solve the hierarchy problem,
provides a Dark Matter candidate and leads to a unification of the gauge
couplings, thus paving the way to a Grand Unified Theory. The most frequently
studied realizations of SUSY are the Minimal Supersymmetric Standard
Model (MSSM)~\htC{\cite{}} and the Next-to-Minimal Supersymmetric SM
(NMSSM)~\htC{\cite{}}. 
Contrary to the case of the SM, in the MSSM two Higgs doublets are required.
This results after electroweak symmetry breaking (EWSB) in five
physical Higgs bosons. In the $\CP$-conserving case, these are two $\CP$-even
Higgs bosons, one $\CP$-odd Higgs boson, and two charged Higgs bosons. The
NMSSM Higgs sector is extended by an additional complex superfield
resulting in the $\CP$-conserving case in three $\CP$-even,
two $\CP$-odd and two charged Higgs bosons. Contrary to the SM the mass of the
(neutral) Higgs bosons can be predicted in terms of the relevant SUSY
parameters. 
%[After fixing one Higgs boson mass
%scale (e.g.\ of the charged Higgs boson) the other Higgs boson masses can be
%calculated.] \htC{-- Why do you say this? We have to fix many more input
%parameters: $\lambda, \kappa, A_\kappa, A_\lambda, v_s,...$ in order to be able
%to calculate the masses. Assuming you think of the MSSM your sentence
%is true only at LO. I would completely leave this sentence out
%here. --} 
While supersymmetric relations lead to an upper mass bound for the
light $\CP$-even Higgs boson well below 125~GeV, the inclusion of higher
order corrections allows to shift the mass to the observed value.
However, both in the MSSM and the NMSSM, the theoretical uncertainties of
the current predictions for the mass of the SM-like Higgs boson are
significantly larger than  the experimental accuracy. 
%
For the MSSM detailed estimates for theoretical uncertainties of the
Higgs-mass predictions are available, see 
e.g.~\cite{Degrassi:2002fi,Allanach:2004rh}. Automated estimates of the
theoretical uncertainties within the MSSM can, e.g., be performed with 
\FH~\cite{Heinemeyer:1998yj,Heinemeyer:1998np,Degrassi:2002fi,Frank:2006yh,Hahn:2009zz,Hahn:2013ria,Bahl:2016brp,feynhiggs-www}.


For the NMSSM several public spectrum generators are available that
offer an automated calculation of the Higgs boson masses:
\texttt{FlexibleSUSY}~\cite{Athron:2014yba},
\htPD{\texttt{FlexibleEFTHiggs}~\cite{Athron:2016fuq}},
\texttt{NMSSMCALC}~\cite{Baglio:2013iia},
\texttt{NMSSMTools}~\cite{Ellwanger:2004xm,     Ellwanger:2005dv,
 Ellwanger:2006rn},     \texttt{SOFTSUSY}~\cite{Allanach:2001kg,
 Allanach:2013kza,        Allanach:2014nba}        and
\texttt{SPheno}~\cite{Porod:2003um,  Porod:2011nf}.   The  results
obtained by the different codes for the same set of input parameters
can differ by several $\giga\electronvolt$.

A first step towards investigating the theoretical uncertainties for
NMSSM Higgs-mass predictions focusing on calculations using a
pure $\DRbar$ renormalization has been performed
in~\cite{Staub:2015aea}. In this publication the aforementioned tools
(except \texttt{FlexibleEFTHiggs}, which did not exist then)
were used to calculate NMSSM Higgs-boson masses for six sample scenarios
with different physical properties. The sources for the differences
between the codes have been identified, and after modifying the codes to use
the same approximations they agree at the level of \order{10 \mev} 
(for the same set of higher-order corrections).
%\htC{SH: give a very few details? Did the
% codes improve by addressing the differences? Comment on this? MM: I
% think it is not so easy to answer this question in a compact
% form. And for sure in the paper no improvements are quoted. You can
% anyway not call this improvements. Different codes do different
% things and have to stick to the approximations they use to be
% consistent. I think with my way of writing it, it is clear that the
% differences are based on different approximations. For details, the
% reader has to go to the original reference then.} 
However, this comparison did not account for differences resulting from the
use of different renormalisation schemes. Among the tested tools only
\texttt{NMSSMCALC} offers the option to use another renormalization scheme,
namely a mixed $\DRbar$/on-shell (OS) scheme, so that a comparison between
different codes using this scheme was not possible in~\cite{Staub:2015aea}. 
In this work, we will extend \cite{Staub:2015aea} by comparing
codes incorporating a $\DRbar$/OS scheme, namely 
\texttt{NMSSMCALC} and the NMSSM-extended version of
\texttt{FeynHiggs} \cite{Drechsel:2016jdg}.
The next step would then be the comparison between the $\DRbar$/ OS and the
pure $\DRbar$ calculations of the codes  mentioned above.  Sticking
here exclusively to the codes \texttt{NMSSMCALC} and \texttt{FeynHiggs},
with  the  latter  applying  a  mixed $\DRbar$/on-shell renormalization
scheme only, we instead investigate  the  differences  within 
\texttt{NMSSMCALC} for the two renormalization schemes. These steps yield
important ingrediences for an estimate of the intrinsic uncertainties for the
Higgs-boson mass calculations in the NMSSM.

%% This section focuses on the comparison of the predictions for
%% Higgs-masses   implemented   in   \texttt{NMSSMCALC}   and
%% \texttt{NMSSM-FeynHiggs}. It aims at an identification of all sources
%% for differences  in their mass-predictions  and eliminating all
%% differences  beside those  that  are caused  by the  different
%% renormalisation scheme.  Since this task requires thorough knowledge
%% about both codes it is performed in close collaborations between the
%% authors of \texttt{NMSSMCALC} and \texttt{NMSSM-FeynHiggs} and is
%% currently work in progress. The results for modified versions of \NC\
%% have been obtained by its authors.

%% First a brief description of the studied scenarios will be given
%% followed by a short classification of the possible sources of
%% uncertainties Subsequently a short description of the differences
%% between the codes \texttt{NMSSMCALC} and \texttt{NMSSM-FeynHiggs} will
%% be provided together with the means to identify those that are
%% unrelated to the renormalisation-scheme dependence.  Finally the
%% present status of the ongoing comparison will be presented.


The paper is organised as follows. In sec.~\ref{sec:NMSSM} we introduce
our notation for the relevant NMSSM parameters. 
In sec.~\ref{sec:Codes} we describe
the codes \NC\ and \NFH\ together with the relevant differences
between them. The analysed numerical scenarios and their treatment is
described in sec.~\ref{sec:Scenarios}. The obtained results for the
masses and mixing matrices are discussed and their differences are analyzed 
in sec.~\ref{sec:Results}. The
conclusions can be found in sec.~\ref{sec:conclusion}.


==> sections/files19Nov/scenarios19Nov.tex <==
\section{Description of the Scenarios}
\label{sec:Scenarios}

\subsection{The five test-point scenarios}

In \citere{Staub:2015aea}, six test-point (TP) scenarios
were proposed for comparing the Higgs-mass predictions obtained
by different tools using the \DRbar\ scheme. They will also be
used here for the comparison between \NC\ and \NFH\, to facilitate
later on the comparison to ref.~\cite{Staub:2015aea}.
This will allow an easy comparison between the two results. The
definitions of the TP scenarios are 
recapitulated in \refta{tab:TPDefinition}, where all parameters
are given at the indicated scale, both at the high scale \MS\, 
at which they were originally defined, and the scale
of the top-quark on-shell mass $\MTO$.%
\footnote{In the original
definition of the scenarios in ref.~\cite{Staub:2015aea} $\TB$ is
given by its \DRbar-value at the scale of the $Z$-boson mass
$\MZ$, while in \refta{tab:TPDefinition} we give the
corresponding \DRbar-value at the indicated scale, either \MS\ of
\MTO. The values for $\TB$ given here are obtained with
\texttt{FlexibleSUSY} as described in the text.}%
~For completeness we repeat the different physical features
of these scenarios as given in \citere{Staub:2015aea}:
%
\begin{itemize}
\item[TP1:] MSSM-like point.
\item[TP2:] MSSM-like point with large stop splitting. 
\item[TP3:] Point with light singlet and $\lambda$ close to the
 perturbativity limit.
\item[TP4:] Point with heavy singlet and $\lambda$ close to the
 perturbativity limit.
\item[TP5:] Point with slightly lighter singlet. Additional matter needed
 for perturbativity; inspired by~\cite{King:2012is}.
%% \htPD{
%% \item[TP6:] Point with huge $\lambda$ \htC{RG: I propose to leave it away here
%% and I will change instead the order of the following two sentences. SH: I
%% agree.} 
%% }
\end{itemize}
\noindent
The scenario TP6 of \citere{Staub:2015aea}
is characterised by a very large value of $\lambda$. It will be omitted
from this comparison, since the MSSM-approximation employed in \FH\ for
the contributions beyond one-loop order is expected
to yield unreliable results for very large values of $\lambda \gg 0.8$. 
Furthermore, this scenario requires new physics well below the GUT
scale to avoid the non-perturbative regime.
All TP scenarios, using a \DRbar\ renormalisation, contain 
an (MS)SM-like Higgs-field with a two-loop mass around
$125~\gev$. 
%
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
 \scriptsize
 \centering
 \begin{tabular}{crrrrrrrrrrrrrr}
 & $Q$ & \TB & $\lambda$ & $\kappa$ & $\Al$ & $\Ak$ & $\mueff$ &
 $M_1$ & $M_2$ & $M_3$ & $A_t$ & $A_b$ & $M_{\tilde{t}_L}$ & $M_{\tilde{t}_R}$
 \\\toprule
 \multirow{2}[4]{*}{TP1} &
 \MS & $9.599$ & $0.100$ & $0.100$ & $-10.00$ & $-10.00$ & $900.0$ & $500.0$ & 
 $1000$ & $3000$ & $3000$ & $0$ & $1500$ & $1500$
 \\\cmidrule{2-15}
 & $\mt$ & $9.903$ & $0.098$ & $0.100$ & $-198.6$ & $-9.738$ & $886.6$ & $478.1$ & 
 $979.4$ & $3261$ & $2154$ & $-585.2$ & $1907$ & $1838$
 \\\midrule\midrule
 \multirow{2}[4]{*}{TP2} &
 \MS & $9.621$ & $0.050$ & $0.100$ & $-200.0$ & $-200.0$ & $1500$ & 
 $1000$ & $2000$ & $2500$ & $-2900$ & $0$ & $2500$ & $500$
 \\\cmidrule{2-15}
 & $\mt$ & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---
 \\\midrule\midrule
 \multirow{2}[4]{*}{TP3} &
 \MS & $2.881$ & $0.670$ & $0.100$ & $650.0$ & $-10.00$ & $200.0$ &
 $200.0$ & $400.0$ & $2000$ & $1000$ & $1000$ & $1000$ & $1000$
 \\\cmidrule{2-15}
 & $\mt$ & $2.967$ & $0.648$ & $0.097$ & $574.0$ & $-43.68$ & $195.3$ &
 $192.4$ & $391.9$ & $2145$ & $619.8$ & $691.5$ & $1233$ & $1211$
 \\\midrule\midrule
 \multirow{2}[4]{*}{TP4} &
 \MS & $1.920$ & $0.670$ & $0.200$ & $405.0$ & $0$ & $200.0$ & $120.0$ & $200.0$ &
 $1500$ & $1000$ & $1000$ & $750.0$ & $750.0$
 \\\cmidrule{2-15}
 & $\mt$ & $1.975$ & $0.649$ & $0.195$ & $344.3$ & $0.195$ & $195.3$ & $116.0$
 & $195.7$ & $1591$ & $726.5$ & $801.5$ & $891.9$ & $874.4$
 \\\midrule\midrule
 \multirow{2}[4]{*}{TP5} &
 \MS & $2.864$ & $0.670$ & $0.200$ & $570.0$ & $-25.00$ & $200.0$ &
 $135.0$ & $200.0$ & $1400$ & $0$ & $0$ & $1500$ & $1500$
 \\\cmidrule{2-15}
 & $\mt$ & $2.967$ & $0.643$ & $0.193$ & $549.3$ & $-63.47$ & $194.4$ & 
 $128.7$ & $194.3$ & $1526$ & $-234.8$ & $-251.9$ & $1579$ & $1546$
 %% \\\midrule\midrule
 %% \multirow{2}[4]{*}{TP6} &
 %% $1500$ & $3$ & $1.6$ & $1.61$ & $375$ & $-1605$ & $614$ &
 %% $200$ & $400$ & $2000$ & $0$ & $0$ & $1500$ & $1500$
 %% \\\cmidrule{2-15}
 %% & $172.9$ & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---
 \\\bottomrule
 \end{tabular}
 \caption{Definition of the TP scenarios. All parameters are given as
 \DRbar\ parameters at the indicated scale $Q$. All dimensionful
parameters are given in $\gev$. The remaining 
parameters, common to all points, are the diagonal soft-SUSY-breaking
parameters in the sfermion mass matrices, 
$M_{\tilde{f}_L} = M_{\tilde{f}_R} = 1500~\gev$ and the trilinear
sfermion-Higgs coupling $A_f = 0$ at the high scale. 
\MS\ is given by $\tfrac{1}{2}(M_{\tilde t_L} + M_{\tilde t_R})$, and 
$\mt = 172.9~\gev$. 
The scenario TP2 yields tachyonic stop-masses at the scale \MTO. }
 \label{tab:TPDefinition}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The generic scale for physics of the Higgs boson with a mass of 
$\sim 125~\gev$ is the electroweak (EW) scale. Furthermore, the diagrammatic
corrections to the Higgs-boson self-energies in \NC\ and \NFH\ are designed to
calculate the Higgs-boson mass at the order of the EW scale, 
in contrast to calculations using the RGE method that allow for large scale
splittings within the calculation.%
\footnote{As stated above, the contributions from resummed logarithms in
\FH\ are not included in our comparison.}%
~Consequently, in our analysis we will evaluate these scenarios
at their original scale $\MS (= \tfrac{1}{2} (M_{\tilde t_L} + M_{\tilde t_R})$,
the arithmetic mean of the two diagonal soft SUSY-breaking parameters in the
scalar top mass matrix), as well as at the scale of the
OS top-quark mass $\MTO = 172.9~\gev$~\htC{}.
In the latter case this means that the scenarios are evolved
from their original scale \MS\ to the scale \MTO\ with 
{\tt FlexibleSUSY}~\cite{Athron:2014yba,Staub:2009bi,Staub:2010jh,Staub:2012pb,Staub:2013tta,Allanach:2001kg,Allanach:2013kza}. 
\htC{SH: 7 refs??}
These parameters are then used as input for \NC\ in order to obtain the
necessary OS quantities. The parameters at the scale \MTO\ are given in
\refta{tab:TPDefinition}, together with the original parameters
at the scale \MS. The scenario TP2 yields tachyonic stop-masses at the scale
\MTO. Consequently, TP2 is evaluated only at the scale~\MS.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Conversion from \boldmath{\DRbar} to OS parameters}
\label{sec:drbaros}

In \NC\ it is possible to perform calculations with either the OS or
\DRbar\ renormalisation scheme in the top/stop sector. In \NFH\ the
OS scheme is mandatory for the scalar top quarks, while it is
possible to choose the \DRbar\ or \MSbar\ scheme for the top-quark
mass. Both codes are capable of converting \DRbar\ input parameters into OS
parameters at the input scale by using the well-known OS shifts of the
MSSM~\cite{Degrassi:2001yf}%
\footnote{Since only corrections up to
 \order{\alt\als} are discussed in this work, only
 one-loop shifts of \order{\als} for the scalar top quarks
 are necessary. These are identical in both the MSSM and NMSSM.}.
For our comparison we used the routines of only one code, \NC, in
order to prevent effects that originate from different implementations of
these shifts.
\htRG{
The shifts in \NC\ are computed as
\begin{equation}
  X^{(\OS)}=X^{(\DRbar)}-\delta X^{\rm fin}
  \hspace*{1cm}\text{  with   } \hspace*{1cm}
  X= \msqd, \, \mstop{R}, \, \At \,.
\end{equation} 
$X^{\rm fin}$ denotes the finite part of the respective counterterm obtained in the OS scheme as given in ref.~\cite{Muhlleitner:2014vsa}.
They are computed iteratively using the OS parameters}\htSH{, until convergence is reached.}

%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
 \scriptsize
 \centering
 \begin{tabular}{crrrrrrrrrr}
 & \multicolumn{2}{c}{TP1} & \multicolumn{2}{c}{TP2} & \multicolumn{2}{c}{TP3}
 & \multicolumn{2}{c}{TP4} & \multicolumn{2}{c}{TP5}
 \\\toprule
% $Q$ & $1500$ & $172.9$ & $1500$ & $172.9$ & $1000$ & $172.9$
% & $750$ & $172.9$ & $1500$ & $172.9$
 $Q$ & $\MS$ & $\mt$ & $\MS$ & $\mt$ & $\MS$ & $\mt$
 & $\MS$ & $\mt$ & $\MS$ & $\mt$
 \\\midrule\midrule
 $A_t^{\rm OS}$ 
 & $2758$ & $2651$ & $-2525$ & --- & $940.6$ & $933.4$ & $953.0$ & $917.2$ & $-87.80$ & $-25.83$
 \\\midrule
 $M_{\tilde{t}_{\rm L}}^{\rm OS}$ 
 & $1507$ & $1181$ & $2542$ & --- & $1003$ & $856.2$ & $750.4$ & $655.5$ & $1547$ & $1494$
 \\\midrule
 $M_{\tilde{t}_{\rm R}}^{\rm OS}$ 
 & $1507$ & $1055$ & $513$ & --- & $1003$ & $822.2$ & $750.4$ & $629.5$ & $1547$ & $1460$
 \\\midrule\midrule
 $\MHp$ & 2759 & 2755 & 6373 & --- & 641.6 & 642.1 & 455.7 & 455.4 & 615.4 & 617.3
 \\\midrule
 $m_{\tilde{t}_1}^{\rm OS}$ & $1355$ & $904.3$ & $507.0$ & --- & $939.9$ & $761.7$ & $667.2$ & $547.0$
 & $1548$ & $1469$
 \\\midrule
 $m_{\tilde{t}_2}^{\rm OS}$ & $1661$ & $1321$ & $2554$ & --- & $1088$ & $940.9$ & $859.4$ & $764.2$
 & $1565$ & $1504$
 \\\bottomrule
 \end{tabular}
 \caption{OS parameters in the TP scenarios obtained by the routines
 of \NC. Here $A_t^{\OS}$ is the trilinear soft-breaking
 parameter in the stop sector, while $M_{\tilde{t}_L}^{\OS}$ and
 $M_{\tilde{t}_R}^{\OS}$ are the diagonal soft SUSY-breaking 
 parameters in the stop-sector for the \SUL\ doublet and singlet,
 respectively. $\MHp$ denotes the on-shell renormalised mass of
 the charged Higgs boson and $\mstop{i}^{\OS}$
 denotes the obtained on-shell masses of the two stops.
}
 \label{tab:OS}
\end{table}
%%%%%%%%%%%%%%%%%% T A B L E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The current, preliminary version of \NFH\ requires an OS mass of the
charged Higgs boson as input. In order to obtain this quantity
from the \DRbar\ parameters specified in \refta{tab:TPDefinition},
we used routines implemented in \NC. These calculate a two-loop
pole mass for the charged Higgs for the given input parameters using
the \DRbar\ stop-sector parameters. The result is treated as the
OS mass for this comparison and is used as an input value for both
codes, \NFH\ and \NC.%
\footnote{The choice of using \DRbar\ stop-sector parameters in the evaluation
of $\MHp$ (and not the ones converted to OS) later facilitates the comparison
with a pure \DRbar\ calculation.}%
~The OS shifted
stop-sector parameters and the resulting stop masses as obtained
with the routines of \NC\ are given in \refta{tab:OS}. An
overview of the procedure of how the Higgs masses and mixing
matrices from the original scenarios are obtained is given in
\reffi{fig:Alg}.



%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htb!]
 \centering
 \includegraphics{pictures/start2.pdf}
 \caption{Steps performed to obtain predictions for the masses and
 mixing matrices of the \cp-even Higgs fields at the scale $Q$. The
 red dashed line denotes the actual calculation of the Higgs
 masses. It is independent of the RGE evolution and the on-shell
 conversion of the input parameters.
}
\label{fig:Alg}
\end{figure}
%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> sections/inputUncertainties.tex <==
\section{Identification of Input-Uncertainties}

The initial task for the comparison in this section is to identify the
input uncertainties  in order  to isolate the  intrinsic uncertainties
from  higher-order  corrections.   This  is  done  by  separating  any
treatment  of  the  provided  input  parameters  from  the  Higgs-mass
calculation and  by providing adapted  versions of both codes  for the
comparison.


\subsection{RGE-Evolution and On-Shell Conversion of the Input Parameters}

For  the calculation in  the TP-scenario  at the  low scale  the input
parameters  have  to be  evolved  from  $Q$  to $m_t^{\rm  OS}$.   The
RGE-evolution      is      performed      by      \texttt{FlexibleSUSY
  1.2.2}~\cite{Athron:2014yba},    which    includes   the    two-loop
RGE-evolution in the NMSSM for the soft-breaking parameters.

After the input  parameters have been evaluated at  either the high or
the low  scale, all necessary  input-parameters are calculated  by the
built-in routines  of \texttt{NMSSMCalc}.  The  parameters obtained by
\NC\ include the on-shell  values for the trilinear breaking parameter
$A_t$   and    the   soft-breaking   masses    $M_{\tilde{t}_L}$   and
$M_{\tilde{t}}$ in the stop-sector as well as the on-shell mass of the
charged  Higgs $M_{H^\pm}$.   The  on-shell value  for $M_{H^\pm}$  is
calculated  with  one-loop  corrections  for the  one-loop  Higgs-mass
predictions  and  two-loop  corrections  for  the  two-loop  Higgs-mass
predictions, respectively.  By this  procedure of using the same input
parameters  in  both  codes  possible higher-order  effects  from  the
RGE-evolution and on-shell conversion are avoided.



\subsection{Adapted Versions of \NC\ and \NFH}

In  order to  address the  different treatments  of $\alpha_s$  in the
Higgs  self-energies at  the two-loop  level,  the two  codes will  be
adjusted such that they use  an identical, fixed value for $\alpha_s$.
Further   adaptions   are   provided   for  the   treatment   of   the
renormalisation of  the electromagnetic coupling  constant $\alpha$ in
order to  separate this effect  from the influence of  $\alpha_s$. The
different  settings are  listed together  with their  abbreviations in
tab.~\ref{tab:LegendNCComparison}. A more  detailed explanation of the
adaptions will  be given together with the  obtained numerical results
in the following section~\ref{sec:NumericalResultsComparison}.
%
\begin{table}[hbt]
  \centering
  \begin{tabular}{lcccl}
    & $\alpha$ & $\Delta_\alpha$ & $\alpha_s$ & comments\\
    \toprule
    \texttt{NMSSM-FH} $\alpha_{G_F}$ 
    & $\alpha_{G_F}$ & \checkmark & $\alpha_s^{\overline{\text{MS}}}{\left(m_t\right)}$
    & vanilla
    \\
    \texttt{NMSSM-FH} $\alpha{\left(M_Z\right)}$
    & $\alpha{\left(M_Z\right)}$ & \checkmark & $\alpha_s^{\overline{\text{MS}}}{\left(m_t\right)}$
    \\
    \texttt{NMSSM-FH} $\alpha{\left(M_Z\right)}(-)$ 
    & $\alpha{\left(M_Z\right)}$ & -- & $\alpha_s^{\overline{\text{MS}}}{\left(m_t\right)}$
    & unphysical
    \\
    \midrule
    \texttt{NMSSMCalc}
    & $\alpha{\left(M_Z\right)}$ & -- & $\alpha_s^{\overline{\text{DR}}}{\left(Q\right)}$ 
    & vanilla
    \\
    \texttt{NMSSMCalc} $\alpha_s^{\rm mod}$
    & $\alpha{\left(M_Z\right)}$ & -- & $\alpha_s^{\overline{\text{MS}}}{\left(m_t\right)}$
    \\
    \texttt{NMSSMCalc} $(-)$
    & $\alpha{\left(M_Z\right)}$ & -- & $\alpha_s^{\overline{\text{MS}}}{\left(m_t\right)}$
    & uses $\delta{v}^{\overline{\text{DR}}}$
    \\
    \bottomrule\\
  \end{tabular}
  \caption{   The   headings   specify   the  used   value   for   the
    electromagnetic   coupling   constant    $\alpha$,   whether   the
    reparametrisation $\Delta_\alpha$  for the used value  of $\alpha$
    has been applied and which  value for the strong coupling constant
    $\alpha_s$ is  used.  In  the versions  marked with  ``$(-)$'' the
    chosen  value for  $\alpha$ does  neither fit  the renormalisation
    scheme nor  has a reparametrisation been  applied (see text).  They represent
    inconsistent and thus unphysical calculations created only for the
    purpose of this comparison.}
  \label{tab:LegendNCComparison}
\end{table}



==> sections/introduction__Ramona_Gr__ber_s_conflicted_copy_2016-11-26_.tex <==
\section{Introduction}
\label{sec:Introduction}

\begin{itemize}
\item mention  electroweak scale  as preferred scale  for diagrammatic
  calculations \htC{SH: what exactly do you want here?}
\end{itemize}

\noindent
The  experimental  value  of  the mass  of  the  detected  Higgs
signal~\cite{CMS:2015kwa},
%
\begin{align}
  m_H = 125.09 \pm 0.21(\rm{stat.}) \pm 0.11(\rm{syst.})~\giga\electronvolt,
\end{align}
\noindent
has an \htSH{uncertainty} of only  several permille. It  is thus, already
four years 
after its  discovery, an (electroweak) precision  observable.  In order
to make full  use of this high-precision measurement  every model that
provides  a prediction  for  this quantity  should  ideally provide  a
result  with  a  similar  precision.  
%If  a  prediction  with  similar precision is unavailable  
\htSH{Furthermore, for a reliable calculation of the Higgs boson mass(es)}
it is important to provide  a solid estimate
for the  theoretical uncertainties of the  available prediction. 
Two different  sources  for  theoretical   uncertainties  exist  in \htSH{the
Higgs-boson mass} predictions.  One are the experimental \htSH{uncertainties
of the input parameters (``parametric uncertainties''), 
the other are unknown higher-order corrections in the
Higgs-boson mass calculatin itself (``intrinsic uncertainties'').}

\htSH{Supersymmetry (SUSY) is one of the most attractive solutions to several
shortcomings of the Standard Model (SM). It can solve the hierarchy problem,
provides a Dark Matter candidate and leads to a unification of the gauge
couplings, thus paving the way to a Grand Unified Theory. The most frequently
studied realizations of SUSY are the Minimal Supersymmetric Standard
Model MSSM~\htC{\cite{}} and the Next-to-Minimal Supersymmetric SM
(NMSSM)~\htC{\cite{}}.  
Contrary to the case of the SM, in the MSSM two Higgs doublets are required.
This results in five physical Higgs bosons instead of the single Higgs
boson in the SM.  In lowest order these are two $\CP$-even Higgs bosons, 
one $\CP$-odd Higgs boson, and two charged Higgs bosons. The NMSSM contains an
additional Higgs singlet (see below), resulting in total in three $\CP$-even,
two $\CP$-odd and two charged Higgs bosons. After fixing one Higgs boson mass
scale (e.g.\ of the charged Higgs boson) the other Higgs boson masses can be
calculated. 

In particular, one of the $\CP$-even Higgs bosons can be
identified with the observed Higgs boson at $\sim 125 \gev$. However,}
\htRG{both in
the MSSM  and the NMSSM, the theoretical
uncertainties of the current predictions of the mass of the SM-like Higgs
boson are significantly larger than the experimental} \htSH{accuracy}.
%
For the  MSSM detailed estimates for theoretical  uncertainties of the
Higgs-mass predictions  are available, see e.g.~\cite{Degrassi:2002fi,
  Allanach:2004rh}.  At least  one tool, \texttt{FeynHiggs}~\cite{Heinemeyer:1998yj,Heinemeyer:1998np,Degrassi:2002fi,Frank:2006yh,Hahn:2009zz,Hahn:2013ria,Bahl:2016brp,feynhiggs-www}, provides
routines for an automated estimate of the theoretical uncertainties of
its Higgs-mass prediction. \htC{RG: I would either make sure it is only one tool
or rewrite the sentence as: Automated
estimates of the theoretical uncertainties within the MSSM can e.g. 
be performed with FeynHiggs. SH: as far as I know, only FH provides this
feature. }

For the  NMSSM several public  spectrum generators are  available that
offer      an     automated      calculation      of     Higgs masses:
\texttt{FlexibleSUSY}~\cite{Athron:2014yba},
\texttt{NMSSMCALC}~\cite{Baglio:2013iia},
\texttt{NMSSMTools}~\cite{Ellwanger:2004xm,           Ellwanger:2005dv,
  Ellwanger:2006rn},           \texttt{SOFTSUSY}~\cite{Allanach:2001kg,
  Allanach:2013kza,                Allanach:2014nba}               and
\texttt{SPheno}~\cite{Porod:2003um,    Porod:2011nf}.    The   results
obtained by the  different codes for the same  set of input parameters
can  differ by several  $\giga\electronvolt$.

A first  step towards investigating the  theoretical uncertainties for
NMSSM Higgs-mass predictions \htSH{focusing on calculations using a pure 
$\DRbar$ renormalization} has been performed
in~\cite{Staub:2015aea}.   In  this  publication the aforementioned tools
were  used to  calculate  NMSSM  Higgs masses for  six  sample
scenarios  with different  physical  properties. The  sources for  the
differences between  the codes have  been identified. After  they have
been modified to address the differences,
\htC{SH: give a very few details? Did the codes improve by addressing the
  differences? Comment on this?}
an agreement at the level of \order{10 \mev} 
(for    the   same    set   of higher-order corrections) has been  achieved.  
However, this comparison
did   not   account \htRG{for differences resulting from the} 
use  of   different renormalisation schemes. Among the tested tools only
\texttt{NMSSMCALC} offered the option to use a mixed $\DRbar$/on-shell
\htSH{(OS)} scheme , hence a  comparison between different $\DRbar$/on-shell
schemes was not  performed in~\cite{Staub:2015aea}. 
\htRG{In this work, we will extend \cite{Staub:2015aea} by comparing codes
based on different $\DRbar$/OS schemes, 
namely \texttt{NMSSMCALC} and the NMSSM-extended version of \texttt{FeynHiggs}
 \cite{Drechsel:2016jdg}.}
%  In order to  improve on
%this  situation  a  comparison   between  \texttt{NMSSMCALC}  and  the
%NMSSM-extended version  of \texttt{FeynHiggs} developed in  this work,
%called \NFH\  in the  following, is  currently performed.  
% It follows
%closely   the   comparison  performed   in~\cite{Staub:2015aea}   with
%necessary  adaptions and  extensions for  the on-shell  calculation as
%described  below.
   In a  subsequent  step  a comparison  between  the
$\DRbar$/ and the \htSH{pure} $\DRbar$ calculations of the codes mentioned
above  is  necessary. \htSH{Here we investigate the differences within
  \texttt{NMSSMCALC} for the two renormalization schemes.}   
After  these   steps  an  estimate  of \htSH{intrinsic} uncertainties can be
obtained. 

%% This  section  focuses  on  the  comparison  of  the  predictions  for
%% Higgs-masses      implemented      in      \texttt{NMSSMCALC}      and
%% \texttt{NMSSM-FeynHiggs}.  It aims at an identification of all sources
%% for  differences   in  their  mass-predictions   and  eliminating  all
%% differences   beside  those   that   are  caused   by  the   different
%% renormalisation scheme.   Since this task  requires thorough knowledge
%% about both codes  it is performed in close  collaborations between the
%% authors  of  \texttt{NMSSMCALC}  and \texttt{NMSSM-FeynHiggs}  and  is
%% currently work in progress. The  results for modified versions of \NC\
%% have been obtained by its authors.

%% First  a brief  description of  the  studied scenarios  will be  given
%% followed  by  a  short  classification  of  the  possible  sources  of
%% uncertainties  Subsequently  a short  description  of the  differences
%% between the codes \texttt{NMSSMCALC} and \texttt{NMSSM-FeynHiggs} will
%% be  provided  together with  the  means  to  identify those  that  are
%% unrelated  to  the  renormalisation-scheme  dependence.   Finally  the
%% present status of the ongoing comparison will be presented.


The paper is organised as follows. \htRG{In sec.~\ref{sec:NMSSM} we introduce our
 notation of the relevant NMSSM parameters.} In sec.~\ref{sec:Codes} we describe
the  codes  \NC\ and  \NFH\  together  with the  relevant  differences
between them. The analysed numerical  scenarios and their treatment is
described in  sec.~\ref{sec:Scenarios}. The  obtained results  for the
masses an mixing matrices are  given in sec.~\ref{sec:Results} and the
observed  differences  discussed  in  sec.~\ref{sec:Discussion}.   The
conclusions can be found in sec.~\ref{sec:conclusion}.


==> sections/results.tex <==
\clearpage

\section{Numerical Results}
\label{sec:NumericalResultsComparison}


In this  section the Higgs-mass predictions for  the (MS)SM-like field
in  the TP-scenarios  will be  discussed.   The scenario  TP6 will  be
omitted, since the MSSM-approximation is not expected to be viable for
its ``extreme''  value of $\lambda  \approx 1.6$.  While  the complete
results   for  all  \CP-even   Higgs-masses  can   be  found   in  the
appendix~\ref{sec:InputNMSSMCalcComparisonLetter},  this  section will
focus  on  the  differences   between  the  mass-predictions  for  the
(MS)SM-like  Higgs-field of  \NC\  and \NFH.   Each  scenario will  be
evaluated at the high scale $Q$ and the low scale $m_t^{\rm OS}$.
\noindent
Additionally  a ``rough''\footnote{The  input parameters  evaluated at
  either   scale  will   be   fixed  after   the  RGE-evolution   with
  non-vanishing  values for $\lambda$  and $\kappa$,  and subsequently
  the  MSSM-limit,  involving  $\lambda,\  \kappa \rightarrow  0$,  is
  taken.   For  a  future  comparison with  $\DRbar$-calculations  the
  MSSM-limit should be applied before any RGE-evolution takes place, to
  ensure that both codes calculate results in the same scenario. Since
  $\lambda$  and   $\kappa$  have   the  largest  effect   on  genuine
  NMSSM-parameters, the error of this approach is expected to be minor
  for the present calculation.  Also  for the purpose of the presented
  results   the   ``rough''   MSSM-limit   is  sufficient   since   no
  RGE-evolution is  implemented in either \NC\ or  \NFH.  } MSSM-limit
of each scenario was evaluated.

In the following  a short discussion of the  singlet-admixture will be
provided before  the numerical results are  presented. Subsequently the
theoretical  uncertainties  caused by  the  input  parameters and  the
MSSM-approximation of \NFH\ are presented together with an explanation
of    the    adapted   versions    of    the    codes   outlined    in
tab.~\ref{tab:LegendNCComparison}.  In the last  section the two codes
will be compared for their standard mass-predictions.


\subsection{Singlet-admixture}

The  singlet-admixture  to the  fields  $h_i$  beyond lowest-order  is
defined by  the wave function  normalisation matrix $\hat{\mathbf{Z}}$
and  the tree-level  mixing matrix  $\mathbf{U}_{e(0)}$ as  defined in
eq.~\eqref{eq:Uen}.  However, in this section we use the approximation
for the matrix $\mathbf{U}_{e(n)}$ as described in sec.~\ref{sec:Uen}.
The  approximate  matrices  $\mathbf{U}_{e(n)}$  are obtained  by  the
eigenvalue decomposition  from the iterative pole  determination as an
approximation  for the wave  renormalisation factors.   The quantities
$\mathbf{U}_{e(n)}$   are  approximately   unitary  matrices   with  a
unitarity violation of typically less than $1\permil$, if the obtained
mass  from   from  the  iterative   procedure  is  of  the   order  of
$\mathcal{O}{(100~\giga\electronvolt)}$.   Since  at lowest-order  the
singlet-admixture  to the fields  $h_i$ is  determined by  the squared
matrix-elements $|\mathbf{U}_{e(0)}|^2_{i3}$,  we will assume  that at
higher-orders    the    matrix-elements   $|\mathbf{U}_{e(n)}|^2_{i3}$
approximate             the            singlet-admixture            to
$h_i$\footnote{In~\cite{Staub:2015aea} the dominantly singlet- and the
  (MS)SM-like   fields  are   identified  primarily   by   the  matrix
  $\mathbf{U}_{e(n)}$. }.


For     the     TP-scenarios      numerical     values     for     the
$|\mathbf{U}_{e(0)}|^2_{i3}$    and   $|\mathbf{U}_{e(n)}|^2_{i3}$    are
presented in tab.~\ref{tab:SingletAdmixture}.  The depicted values for
$|\mathbf{U}_{e(n)}|^2_{i3}$ are  obtained by the pole  determination for
the mass of the the lightest \CP-even Higgs-field.
%
\begin{table}[htb]
  \centering
  \begin{tabular}{cccccccccc}
    %% \toprule
    &  & \
    & \multicolumn{3}{c}{Comparison I}
    & \
    & \multicolumn{3}{c}{Comparison II}
    \\
    & & \
    & $|\mathbf{U}_{e(n)}|^2_{13}$ & $|\mathbf{U}_{e(n)}|^2_{23}$ & $|\mathbf{U}_{e(n)}|^2_{33}$
    & \
    & $|\mathbf{U}_{e(n)}|^2_{13}$ & $|\mathbf{U}_{e(n)}|^2_{23}$ & $|\mathbf{U}_{e(n)}|^2_{33}$
    \\
    \toprule
    \multirow{3}{*}{TP1}
    & $n = 0$
    & \
    & 0 & 1 & 0
    & \
    & 0 & 1 & 0
    \\
    & $n = 2$ 
    & \
    & 0 & 1 & 0 
    & \
    & 0 & 1 & 0 
    \\\midrule
    \multirow{3}{*}{TP2}
    & $n = 0$
    & \
    & 0 & 1 & 0
    & \
    & -- & -- & --
    \\
    & $n = 2$ 
    & \
    & 0 & 1 & 0 
    & \
    & -- & -- & --
    \\\midrule
    \multirow{3}{*}{TP3}
    & $n = 0$
    & \
    & 0.84 & 0.14 & 0.02
    & \
    & 0.95 & 0.03 & 0.02
    \\
    & $n = 2$ 
    & \
    & 0.92 & 0.06 & 0.02 
    & \
    & 0.96 & 0.02 & 0.02
    \\\midrule
    \multirow{3}{*}{TP4}
    & $n = 0$
    & \
    & 0 & 0.97 & 0.03
    & \
    & 0 & 0.97 & 0.03
    \\
    & $n = 2$ 
    & \
    & 0.17 & 0.80 & 0.03
    & \
    & 0.02 & 0.95 & 0.03
    \\\midrule
    \multirow{3}{*}{TP5}
    & $n = 0$
    & \
    & 0.03 & 0.95 & 0.02
    & \
    & 0.13 & 0.84 & 0.02
    \\
    & $n = 2$ 
    & \
    & 0.31 & 0.67 & 0.02
    & \
    & 0.28 & 0.69 & 0.02
    \\\bottomrule\\
  \end{tabular}
  \caption{  Singlet-admixture $|\mathbf{U}_{e(0)}|^2_{i3}$  at lowest
    order      and     approximate      two-loop     singlet-admixture
    $|\mathbf{U}_{e(2)}|^2_{i3}$ to the fields $h_i$ for the high scale
    $Q$ (comparison  I) and the  low scale $m_t^{\rm  OS}$ (comparison
    II).   The  mass  hierarchy  $m_{h_1}  <  m_{h_2}  <  m_{h_3}$  is
    assumed.}
  \label{tab:SingletAdmixture}
\end{table}

At  two-loop order  in each  scenario TP1  \ldots 4  one field  can be
identified   to    be   dominantly   singlet-like.     For   TP5   the
singlet-admixture  is significant for  both lighter  Higgs-fields. For
TP4 the singlet-admixture to $h_1$  at the low scale $m_t^{\rm OS}$ is
an order  of magnitude smaller than  at the high scale  $Q$.  This may
lead  to   smaller  higher-order   effects  from  the   genuine  NMSSM
corrections.




\subsection{Higher-order effects from $\alpha_s$}


The codes \NC\ and \NFH\ have  a different standard value that is used
internally for  the strong  coupling-constant $\alpha_s$: In  \NC\ the
$\DRbar$ renormalised  value for $\alpha_s$ is evaluated  at the scale
specified  in  the  SLHA-Input  file,  while  \NFH\  always  uses  the
$\MSbar$-value of $\alpha_s$  at the pole mass of  the top-quark.  The
value for  $\alpha_s$ is fixed intentionally, since  \NFH\ is designed
to calculate the Higgs-mass at the electroweak scale. The strong scale
dependence of $\alpha_s$ can lead to vastly different two-loop results
for   the   Higgs-masses,   since   all  two-loop   contributions   of
$\mathcal{O}{(\alpha_t   \alpha_s)}$  are  directly   proportional  to
$\alpha_s$.   In  fig.~\ref{fig:ASmodMZext}  the absolute  differences
between  the  two  mass-predictions  for  the  dominantly  (MS)SM-like
Higgs-field  obtained by the  standard (vanilla)  version of  \NC\ and
\NFH\ are  shown in orange  for all TP-scenarios  at the high  and low
scale.  In  order to eliminate  the influence of different  values for
the  electromagnetic coupling  constants,  the used  \NFH-modification
includes  the  reparametrisation  for  $\alpha{(M_Z)}$ if  not  stated
otherwise.     It     is    abbreviated    with    ``\texttt{NMSSM-FH}
$\alpha{(M_Z)}$''.   The  comparison  for  TP2  at the  low  scale  is
unphysical, since the scenario  yields negative squared masses for the
stop-squarks after the RGE-evolution.  Throughout this section it will
be treated as  if the difference between the codes  were zero to allow
an easy  comparison between charts  depicting the low-  and high-scale
results.
\begin{figure}[htbp]
  \centering
  %% \includegraphics[width=.9\textwidth]{pictures/chartASmodMZext_1.pdf}
  %% \\
  %% \includegraphics[width=.9\textwidth]{pictures/chartASmodMZext_2.pdf}
  \caption{ Absolute  difference between the two-loop  predictions for
    the mass  of the  dominantly (MS)SM-like  Higgs-field of  \NC\ and
    ``\NFH\      $\alpha{(M_Z)}$''      (orange,     $\Delta{m}      =
    |m_{h_i}^{(\texttt{NC})}                                         -
    m_{h_i}^{(\texttt{N-FH}\ \alpha{(M_Z)})}|$),  ``\NC $\alpha_s^{\rm
      mod}$''  and  ``\NFH\  $\alpha{(M_Z)}$''  (brown,  $\Delta{m}  =
    |m_{h_i}^{(\texttt{NC\      }      \alpha_s^{\rm     mod})}      -
    m_{h_i}^{(\texttt{N-FH}\     \alpha{(M_Z)})}|$),     and     ``\NC
    $\alpha_s^{\rm  mod}$''  and ``\NFH\  $\alpha{(M_Z)}(-)$''  (blue,
    $\Delta{m}  =  |m_{h_i}^{(\texttt{NC\  }  \alpha_s^{\rm  mod})}  -
    m_{h_i}^{(\texttt{N-FH}\  \alpha{(M_Z)}(-))}|$).  The  upper chart
    shows the comparison at the high scale, the lower chart at the low
    scale.}
  \label{fig:ASmodMZext}
\end{figure}


For  the calculation  at the  high scale  the differences  between the
mass-predictions can  exceed $5~\giga\electronvolt$, while  at the low
scale      the       difference      generally      remains      below
$1~\giga\electronvolt$.  This behaviour is  a pure  MSSM-effect, since
also  TP2 with  a  very  small value  for  $\lambda$ is  significantly
affected. It  can be directly traced  back to the  scale dependence of
$\alpha_s$. The values at the different scales $Q$ in the TP-scenarios
are    shown    in    the    $\DRbar$-    and    $\MSbar$-scheme    in
tab.~\ref{tab:RunningAS}.
%
\begin{table}[htb]
  \centering
  \begin{tabular}{ccc}
    \toprule
    $Q$ & $\alpha_s^{\MSbar}{(Q)}$ & $\alpha_s^{\DRbar}{(Q)}$
    \\
    \midrule
    $m_t^{\rm OS}$ & 0.10697 & 0.10789
    \\
    $750~\giga\electronvolt$ & 0.09065 & 0.09131     
    \\
    $1000~\giga\electronvolt$ & 0.08803 & 0.08865     
    \\
    $1500~\giga\electronvolt$ & 0.08458 & 0.08515     
    \\
    \bottomrule\\
  \end{tabular}
  \caption{The strong coupling constant at the different scales $Q$ of
    the  TP-scenarios  and  the  top-quark  mass  $m_t^{\rm  OS}$.  As
    starting  value  $\alpha_s{(M_Z)} =  0.1184$~\cite{McNeile:2010ji}
    was used.  }
  \label{tab:RunningAS}
\end{table}
\noindent
The  shown  values  for  $\alpha_s^{\MSbar}$ were  obtained  with  the
results of~\cite{Chetyrkin:2000yt} including corrections up to partial
four-loop  order   as  implemented  in  \NC,  while   the  values  for
$\alpha_s^{\DRbar}$   were   obtained   with   the   two-loop   result
of~\cite{Baer:2002ek}.   The scale  variation has  a larger  effect on
$\alpha_s$ than the \MSbar\ to \DRbar\ conversion.

In   tab.~\ref{tab:AlphaSInfluence}  the   two-loop   shifts  to   the
(MS)SM-like Higgs-boson masses,
%
\begin{align}
  m_{h_i}^{(\rm 2L)}
  =
  m_{h_i}^{(\rm tree)} + \Delta{m_{h_i}^{(\rm 1L)}} + \Delta{m_{h_i}^{(\rm 2L)}}
  =
  m_{h_i}^{(\rm 1L)} + \Delta{m_{h_i}^{(\rm 2L)}}
\end{align}
\noindent
with
%
\begin{align}
  \Delta{m_{h_i}^{(\rm 2L)}} = m_{h_i}^{(\rm 2L)} - m_{h_i}^{(\rm 1L)},
\end{align}
\noindent
are given for the vanilla version  of \NC\ and \NFH\ reparametrised to
$\alpha{(M_Z)}$  together  with  the  change of  the  strong  coupling
constant at the  high scale $\alpha_s^{\DRbar}{(Q)}$, that  is used in
\NC, relative to its $\MSbar$ value at $m_t^{\rm OS}$, that is used in
\NFH.
%
\begin{table}[htb]
  \centering
  \begin{tabular}{ccccc}
    \toprule
    & & \multicolumn{2}{c}{$\Delta{m^{(\rm 2L)}}/\giga\electronvolt$}
    \\
    & $Q/\giga\electronvolt$ & \NC & \texttt{NMSSM-FH} & $\Delta{\alpha_s}_{\rm rel}$ 
    \\\midrule
    TP1 & 1500 & 19.692 & 25.263 & $\approx 20\%$\\
    TP2 & 1500 & 20.253 & 26.014 & $\approx 20\%$\\
    TP3 & 1000 & 10.896 & 13.196 & $\approx 17\%$\\
    TP4 & 750  &  4.571 &  5.675 & $\approx 15\%$\\
    TP5 & 1500 & 11.603 & 13.875 & $\approx 20\%$\\
    \bottomrule\\
  \end{tabular}
  \caption{
    Two-loop shifts $\Delta{m} = |m^{\rm (2L)} - m^{\rm (1L)}|$ for 
    \NC\ and \NFH\ with $\alpha{(M_Z)}$
    and relative  difference between the values of the strong
    coupling constant in the $\MSbar$-scheme at the top-quark
    pole mass $m_t^{\rm (OS)}$ and in the  $\DRbar$-scheme at
    the high scale $Q$,
    $\delta{\alpha}_{\rm rel} = (\alpha_s{(m_t^{\rm (OS)})} - \alpha_s{(Q)})/\alpha_s{(m_t^{\rm (OS)})}$
  }
  \label{tab:AlphaSInfluence}
\end{table}
\noindent
The  majority  of  the  difference  between  the  two-loop  shifts  of
\NC\   (abbreviated  as   \texttt{NC})  and   \NFH\  (abbreviated   as
\texttt{N-FH}) in tab.~\ref{tab:AlphaSInfluence} at the high scale can
be explained by $\Delta{\alpha_s}_{\rm rel}$, since
%
\begin{align}
  \Delta{m}^{\texttt{N-FH}} \left(1 - \Delta{\alpha_s}_{\rm rel}\right) \approx \Delta{m}^{\texttt{NC}}.
\end{align}

The calculation at the low scale is only influenced by the $\MSbar$ to
$\DRbar$ conversion,  and the  low-scale mass-predictions are  in much
better agreement with each other than the high-scale mass-predictions,
that are also affected also by the RGE-evolution of $\alpha_s$.

In order to eliminate the  influence of an RGE-evolving $\alpha_s$ and
its renormalisation scheme conversion,  \NC\ was modified such that it
uses the same value $\alpha_s^{\MSbar}{(m_t^{\rm OS})}$ as \NFH.  This
version  is labelled  ``\NC\ $\alpha_s^{\rm  mod}$''.   The difference
between  the two-loop mass  predictions of  this modified  version and
``\texttt{NMSSM-FH}   $\alpha{(M_Z)}$''   is   shown   in   brown   in
fig.~\ref{tab:RunningAS}.  For the calculation  at the high scale both
codes  show much more  similar results  with a  difference of  at most
$430~\mega\electronvolt$.   At  the  low  scale the  modified  version
``\NC\ $\alpha_s^{\rm  mod}$'' yields  a more similar  mass prediction
for  the  MSSM-like  scenario  TP1  and  TP5.  For  TP3  and  TP4  the
differences  between  the   two  predictions  are  slightly  increased
compared the comparison with the unmodified version of \NC\ and can be
attributed to the  $\MSbar$--$\DRbar$-conversion of $\alpha_s$ and the
two-loop MSSM-approximation of \NFH.

The residual  differences are increased  for larger singlet-admixtures
and increased difference  between the mass-scale of the  stops and the
renormalisation scale.
%
\begin{table}[htb]
  \centering
  \begin{tabular}{cccccc}
    \toprule
    & \multicolumn{2}{c}{Comparison I} & \ & \multicolumn{2}{c}{Comparison II}
    \\
    & $m_{\tilde{t}_1}$ & $m_{\tilde{t}_2}$ &  \ & $m_{\tilde{t}_1}$ & $m_{\tilde{t}_2}$
    \\
    \midrule
    TP1 & 1360.25 & 1656.14 & \ & 1547.21 & 1564.19
    \\
    TP2 & 2553.68 & 507.225 & \ & -- & --
    \\
    TP3 & 941.474 & 1085.45 & \ & 941.784 & 1085.16
    \\
    TP4 & 669.224 & 855.688 & \ & 760.14 & 549.379
    \\
    TP5 & 1547.21 & 1564.19 & \ & 1503.75 & 1468.22
    \\
    \bottomrule\\
  \end{tabular}
  \caption{Stop-squark  masses in  $\giga\electronvolt$ at  tree-level
    for the calculation  at the high scale $Q$ (comparison  I) and low
    scale $m_t^{\rm OS}$ (comparison II).}
  \label{tab:TreelevelStopMassesTP}
\end{table}
\noindent
These    behaviours   can    be   observed    in   both    charts   in
fig.~\ref{fig:ASmodMZext}:   The  residual  differences   between  the
predictions   of  ``\texttt{NMSSM-FH}  $\alpha{(M_Z)}$''   and  ``\NC\
$\alpha_s^{\rm    mod}$'',   that   are    depicted   in    brown   in
fig.~\ref{fig:ASmodMZext}, are  smaller at  the high scale,  where the
renormalisation  scheme   $\mu_{\rm  r}$   is  chosen  close   to  the
stop-masses (tab.~\ref{tab:TreelevelStopMassesTP}).  They are somewhat
enhanced  for   the  scenarios  with  larger   mass-splitting  in  the
stop-sector, most notably for  TP3 and TP4.  The extreme mass-splitting
for TP2 is mitigated by  the small values of $\lambda$, which suppress
genuine NMSSM-corrections.


In  order   to  eliminate  the  theoretical   uncertainty  induced  by
$\alpha_s$ for all subsequent studies both \NC\ and \NFH\ will use the
same fixed value  for $\alpha_s^{\MSbar}{(m_t^{(\rm OS)})} = 0.10697$.
For  all  following studies  this  modification  is  considered to  be
included if not stated otherwise. Hence, the addition ``$\alpha_s^{\rm
  mod}$'' for the $\alpha_s$-modified  version of \NC\ will be dropped
in the following.


\subsection{Effects of the MSSM-Approximation}


The   residual  differences   between  \NC\   and  ``\texttt{NMSSM-FH}
$\alpha{(M_Z)}$'', depicted in brown in fig.~\ref{fig:ASmodMZext}, are
caused by  the different  renormalisation schemes for  $\delta{v}$ and
$\dZe$,  respectively, and  the two-loop  MSSM-approximation  of \NFH.
They      correlate     to      the     difference      studied     in
sec.~\ref{subsec:comparison},  but have  a  generally somewhat  larger
impact than the  effects observed in that section.  Scenario TP3 bares
the  closest  resemblance of  the  physical  situation  in the  sample
scenario from section~\ref{subsec:comparison}.  Both scenarios feature
a  light  singlet-like  state (tab.~\ref{tab:HiggsMassesTreeTP})  with
relatively  small  mass-splitting  in  the  stop-sector  and  a  large
gluino-mass.

In order  to disentangle the  effects from the  renormalisation scheme
and the  approximation a further  comparison is performed,  where \NC\
and  \NFH\  were  modified  such   that  both  codes  use  a  $\DRbar$
renormalisation  scheme  for the  vacuum  expectation-value $v$  while
using  $\alpha{(M_Z)}$ \textit{without} applying  a reparametrisation.
These  versions are  labelled ``\NC\  $(-)$''  and ``\texttt{NMSSM-FH}
$\alpha{(M_Z)}(-)$''.   These  modified  versions  do  not  reflect  a
physical calculation,  since they use  a value for $\alpha$  that does
not  fit  the applied  renormalisation  condition  without applying  a
reparametrisation.  However, the  residual two-loop difference between
the    these    versions,    that    is   depicted    in    blue    in
fig.~\ref{fig:ASmodMZext}, provides  an insight  into the size  of the
genuine NMSSM  two-loop corrections.  For the calculation  at the high
scale  they remain below  $90~\mega\electronvolt$ in  all TP-scenarios
and are largest for TP5, where the singlet-admixture to the dominantly
(MS)SM-like field  is largest.  For  the calculation at the  low scale
the    residual    differences   are    slightly    larger,   up    to
$210~\mega\electronvolt$, for TP5.

Thus the MSSM-approximation can be  expected to lead to an effect that
is  minor compared  to  the effect  of  the different  renormalisation
schemes. The  effect of the differences in  the renormalisation scheme
is   enhanced   compared   to   the   effect   observed   earlier   in
section~\ref{subsec:comparison}  for  the   sample  scenario  that  is
similar to  TP3. This  enhancement is driven  by the larger  values of
$\lambda$.     The   uncertainty    arising    from   employing    the
MSSM-approximation  can be seen  to be  insignificant compared  to the
other  theoretical uncertainties  for all  TP-scenarios.   The largest
(but  still  numerically  small)  effect  occurs  to  TP5,  where  the
increased singlet-admixture  to the  (MS)SM-like field accounts  for a
larger impact of the MSSM-approximation.


\subsection{Higher-order effects from the  Reparametrisation}

In \NFH\  the reparametrisation procedure  for $\alpha$ is  applied at
the tree-level, leading to a reparametrised result at one-loop order.
Beyond one-loop  order the reparametrisation shifts  are considered to
be negligible higher-order  effects.  However, a reparametrisation for
the  genuine  NMSSM   one-loop  Higgs-contributions  would  result  in
contributions  that are  formally of  the same  order as  the two-loop
contributions   from   the   Higgs-sector.    The  impact   of   these
contributions  can  be  estimated   for  the  TP-scenarios.   For  the
comparison  of  \DRbar-calculations  in~\cite{Staub:2015aea} the  code
\texttt{SPheno} includes two-loop corrections from the Higgs-sector in
the gaugeless limit.  The corresponding numerical results are given in
tab.~\ref{tab:SPHENOResultsTP}   for   convenience\footnote{While  the
  two-loop MSSM-corrections  seem to have  a very small effect  on the
  results in all TP-scenarios, they  have been found to yield a larger
  effect   for    the   calculation   with    mixed   on-shell/\DRbar\
  renormalisation schemes in certain scenarios.}.
%
\begin{table}
  \centering
  \begin{tabular}{lccccc}
    \toprule
    & $\mathcal{O}{(\alpha_t \alpha_s)}$
    & $\mathcal{O}{(\alpha_t \alpha_s, \alpha_b \alpha_s)}$ & 'full' & $\Delta{m_1}$ & $\Delta{m_2}$ 
    \\
    && + MSSM &&
    \\\midrule
    TP1 & 124.84 & 123.84 & 123.84 & $<0.01$ & $<0.01$
    \\
    TP2 & 123.81 & 123.08 & 123.05 & 0.73 & 0.03
    \\
    TP3 & 127.55 & 126.59 & 126.10 & 0.96 & 0.49
    \\
    TP4 & 128.23 & 127.52 & 126.33  & 0.71 & 1.19
    \\
    TP5 & 126.12 & 125.12 & 124.85 & 1.00 & 0.27
    \\\bottomrule\\
  \end{tabular}
  \caption{Results for  the (MS)SM-like Higgs-mass for  the high scale
    as obtained  with \texttt{SPHENO}  from~\cite{Staub:2015aea}.  The
    orders  of the  included two-loop  NMSSM-contributions are  stated,
    where ``MSSM'' refers to the  $\DRbar$ results for the corrections
    that  are included  in \texttt{FeynHiggs}  and 'full'  denotes the
    corresponding   NMSSM-contributions   plus   the   correction   from
    the    Higgs-sector  in  the  gaugeless   limit,  that  means  corrections
    including the  couplings $\lambda$ and $\kappa$.   The differences
    $\Delta{m_i}$  denote   the  impact   of  the   MSSM  corrections,
    $\Delta{m_1}$, and the  Higgs-sector contributions, $\Delta{m_2}$.
    The  corrections of  $\mathcal{O}{(\alpha_b \alpha_s)}$  alone are
    negligible for all scenarios.}
  \label{tab:SPHENOResultsTP}
\end{table}

While the  Higgs-sector contributions at the two-loop  level give rise
to a small  mass-shift for the MSSM-like scenarios  TP1 and TP2, their
effect on the mass of  the (MS)SM-like fields reside between $0.3$ and
$1.2~\giga\electronvolt$ for  TP3-5.  As mentioned above,  a change in
the parametrisation of $\alpha$1 at the one-loop level induces a shift
that is  of the order of  the two-loop contributions  from the Higgs-m
and gauge-sector.   It can therefore  give an indication  of possible
effects of unknown higher-order effects of this order.


\subsection{Higher-order effects from $\alpha$}

In fig.~\ref{fig:GFMZComparison2L} the differences $\Delta{m}$ between
the  two-loop mass-predictions  using the  values  $\alpha{(M_Z)}$ and
$\alpha_{G_F}$,  and  the  corresponding renormalisation  schemes  are
depicted.  In order to disentangle the effects that are genuine to the
NMSSM, the difference between the corresponding Higgs-mass predictions
in the MSSM are depicted in orange.  For the original TP-scenarios two
results  are presented.   In brown  the difference  between  the \NFH\
versions  with   the  reparametrisations  to   $\alpha_{G_F}$  and  to
$\alpha{(M_Z)}$ are depicted, while the difference between the vanilla
versions      of      \NFH\      with      corrections      up      to
$\mathcal{O}{\alpha_t\alpha_s}$ only and \NC\ is depicted in blue.

\begin{figure}[htbp]
  \centering
  %% \includegraphics[width=.9\textwidth]{pictures/chart2LGFMZUni_1.pdf}
  %% \\
  %% \includegraphics[width=.9\textwidth]{pictures/chart2LGFMZUni_2.pdf}
  \caption{Absolute  difference between  the  two-loop mass-prediction
    parametrised  in terms of  $\alpha{(M_Z)}$ and  $\alpha_{G_F}$ for
    the      MSSM-limit     (orange,      $\Delta{m}      =     \left|
      m_{h_i}^{(\texttt{NC})}  -  m_{h_i}^{(\texttt{N-FH})} \right|$),
    between the  two reparametrisations in \NFH\  (brown, $\Delta{m} =
    \left|       m_{h_i}^{(\texttt{N-FH}       \alpha{(M_Z)})}       -
      m_{h_i}^{(\texttt{N-FH})}\right|$),  and  between  the  original
    versions with  corrections up to $\mathcal{O}{(\alpha_t\alpha_s)}$
    (blue,     $\Delta{m}     =    \left|m_{h_i}^{(\texttt{NC})}     -
      m_{h_i}^{(\texttt{N-FH})}\right|$), of the TP-scenarios.}
  \label{fig:GFMZComparison2L}
\end{figure}

Both for the calculation at the  high and the low scale the difference
between     the    MSSM-results     ranges    between     $500$    and
$700~\mega\electronvolt$, with  marginally larger differences  for the
calculation at the low scale.

For the MSSM-like scenarios TP1  and TP2 the genuine NMSSM-effects are
small at  both scales.  They remain  below $50~\mega\electronvolt$ for
both the results obtained with only one or two different codes.

For TP3-5 the difference  between the reparametrised versions of \NFH\
is  generally smaller  than  the difference  in  the MSSM-limit.   The
comparison of  the vanilla  versions of \NC\  and \NFH\  yields larger
differences, since it accounts  also for the different renormalisation
schemes.   The size  of  this additional  difference  between the  two
comparisons   for   the  TP-scenarios   (brown   and   blue  bars   in
fig.~\ref{fig:GFMZComparison2L})  closely  resembles  the  differences
obtained  for  the  comparison  between \NC\  and  ``\texttt{NMSSM-FH}
$\alpha{(M_Z)}$'' (brown  bars in fig.~\ref{fig:ASmodMZext}).   For an
estimate  of  the  remaining  theoretical uncertainties  from  unknown
higher-order corrections all  the above effects have to  be taken into
account.

The genuine NMSSM-effects are more important for scenarios with rather
large  values  for $\lambda$  (TP3-5),  where  the  difference can  be
altered by up to  $500~\mega\electronvolt$ compared to the MSSM-result
at  the high  scale.   For  TP5 that  means  that the  MSSM-difference
(orange) is almost completely  absorbed by genuine NMSSM-effects.  For
scenarios  with large  mass-splitting in  the stop-sector  the genuine
NMSSM-effects are somewhat enhanced (TP3, TP4) as well as for a larger
singlet-admixture (TP5).

For the calculation  at the low scale the  genuine NMSSM-effects alter
the  MSSM-result  by   at  most  $200~\mega\electronvolt$.   From  the
obtained results neither  at the high nor at the  low scale a tendency
can be deduced that indicates a  general increase or a decrease of the
differences  due to  genuine NMSSM-effects.   However,  the difference
between the calculation using only  one and both codes (brown and blue
bars  in  fig.~\ref{fig:GFMZComparison2L})   is  increased  for  large
mass-splitting   in  the   stop-sector   (TP3,  TP4)   and  a   larger
singlet-admixture (TP5).

The presented results indicate  that the renormalisation scheme of the
electromagnetic  coupling  constant $\alpha$  can  have a  significant
numerical  impact  on  the  mass-prediction  even  for  a  (MS)SM-like
Higgs-field  of   up  to  $1~\giga\electronvolt$   from  the  combined
MSSM-like and  genuine NMSSM-effects.  The comparison  between the two
codes based on somewhat  different schemes reveals differences that go
beyond the ones obtained from changing the parametrisation in a single
code.


\subsection{Higher-order effects from the Top-/Stop-sector}

In this  section results for  the comparison of  ``\NC\ $\alpha_s^{\rm
  mod}$''  with $\DRbar$-renormalised  masses in  the top-/stop-sector
and the standard version of \NFH\ with on-shell renormalised masses in
the         top-/stop-sector          are         presented         in
tab.~\ref{eq:HOEffectFromTopStops}.   The scenarios were  evaluated at
the scale $m_t^{\rm  OS}$.  The results are preliminary,  in the sense
that the $\DRbar$-option  in \NC\ only accounts for  the conversion of
the top-mass and stop-sector parameters, but not for the determination
of  the on-shell  mass  for the  charged  Higgs. In  NC\ the  on-shell
charged  Higgs mass  is determined  with top-  and stop-masses  in the
chosen  renormalisation  scheme,  while  the  results  for  \NFH\  are
obtained for  the on-shell  mass for the  charged Higgs  obtained with
on-shell top- and stop-masses.
%
\begin{table}[htb]
  \centering
  \begin{tabular}{llccccc}
    \toprule
    %% &
    & TP1 & TP2 & TP3 & TP4 & TP5
    \\\midrule
    %% \multirow{2}{*}{NMSSM} &
    \NC\ $\alpha_s^{\rm mod}$ & 
    116.94 & -- & 128.34 & 132.29 & 123.84
    \\
    %% &
    \texttt{NMSSM-FH} $\mathcal{O}{\left(\alpha_t \alpha_s\right)}$ & 
    113.19 & -- & 123.39 & 128.25 & 121.78
    \\
    \texttt{NMSSM-FH} & 
    121.70 & -- & 126.30 & 131.13 & 123.48
    \\
    \bottomrule\\
  \end{tabular}
  \caption{Results  for the  (MS)SM-like Higgs-field  obtained in  the
    TP-scenarios  from the  codes ``\NC\  $\alpha_s^{\rm mod}$''  with
    $\DRbar$-renormalised  masses  in  the  top-/stop-sector  and  
    \NFH\ evaluated once including only the corrections up to 
    $\mathcal{O}{(\alpha_t \alpha_s)}$ and once including all 
    corrections of $\mathcal{O}{\left(\alpha_s\alpha_t,
        \alpha_t^2,   \alpha_s\alpha_b, \alpha_t\alpha_b\right)}$
    with on-shell renormalised masses in the top-/stop-sector.}
  \label{eq:HOEffectFromTopStops}
\end{table}
\noindent
The  differences  between  the  two  codes  for  contributions  up  to
$\mathcal{O}{(\alpha_t  \alpha_s)}$   employing  a  \DRbar\   and  the
on-shell renormalisation of the  stop-sector are found to be sizeable,
reaching up  to $5~\giga\electronvolt$ for TP3. The  inclusion for the
additional MSSM corrections result in a sizeable shift compared to the
results   including    only   correction   of   $\mathcal{O}{(\alpha_t
  \alpha_s)}$,  reaching up to  $8.5~\giga\electronvolt$ for  TP1. For
all   TP-scenarios   the  results   including   the  additional   MSSM
contributions  in  the on-shell  scheme  for  the top-/stop-sector  are
generally  closer to  the result  with a  \DRbar\ scheme  in  the same
sector  including   only  corrections  up   to  $\mathcal{O}{(\alpha_t
  \alpha_s)}$.


==> sections/sections <==
\section{The two codes: \NC\ and \FH}
\label{sec:Codes}

%\htPD{PD:   Should  we   rather  ``copy''   the  structure
% of~\cite{Staub:2015aea} for this section?}
%
%\htPD{
%\begin{itemize}
%\item describe differences
%\item for summary see tab.~\ref{tab:DiffNcNfhVanilla}
%\end{itemize}
%}

In this section we will give a brief overview about the higher-order
corrections to Higgs-boson masses included in \FH\ and \NC,
together with the different renormalization schemes employed.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Incorporation of higher-order contributions}
\label{sec:calcho}

The masses of the \cp-even Higgs bosons are obtained from the complex
poles of the full propagator matrix. The inverse propagator matrix
for the three \cp-even Higgs bosons $h_i$ from
eq.~\eqref{eq:MixMatrices} is a $3 \times 3$ matrix that reads
%
\begin{align}
 \Delta^{-1}{\left(k^2\right)} = \mathi
 \left[k^2\mathds{1} - \mathbf{M}_{hh}
 + \mathbf{\hat{\Sigma}}_{hh}{\left(k^2\right)}
 \right].
\end{align}
\noindent
Here $\mathbf{M}_{hh}$ denotes the diagonalised mass matrix of the
\cp-even Higgs fields at tree level, and $\mathbf{\hat{\Sigma}}_{hh}$
denotes the matrix of their renormalised self-energy corrections. The
three complex poles of the propagator in the \cp-even Higgs sector are
given by the values of the external momentum $k$ for which the
determinant of the inverse propagator-matrix vanishes,
%
\begin{align}
 \det\left[
 \Delta^{-1}{\left(k^2\right)}
 \right]_{k^2 = M_{h_i}^2 - \mathi \Gamma_{h_i} M_{h_i}} \overset{!}{=} 0
 , \ i \in \{1,2,3\}.
\end{align}
\noindent
The real parts of the three poles are identified with the the square
of the Higgs-boson masses $m_{h_i}$ in the \cp-even sector, while the
complex parts include their total widths $\Gamma_{h_i}$. The
renormalised self-energy matrix $\mathbf{\hat{\Sigma}}_{hh}$ at
one-loop order is evaluated in \NC~\cite{Ender:2011qh, Graf:2012hh}
and \FH~\cite{Drechsel:2016jdg} by taking into account the full
contributions from the NMSSM (differences in the
renormalization schemes are discussed below). 
At two-loop order
\texttt{NMSSMCALC} includes the leading (S)QCD corrections from
the top/stop sector of \order{\alt\als} in the 
NMSSM~\cite{Muhlleitner:2014vsa}, while \FH\ uses all available corrections
from the MSSM, that are included in the MSSM-version of
\FH~\cite{Heinemeyer:1998yj,Hahn:2009zz,Heinemeyer:1998np,Degrassi:2002fi,Frank:2006yh,Hahn:2013ria,Bahl:2016brp,feynhiggs-www}, 
as an approximation%
\footnote{Updates beyond the \FH\ version 2.10.2 (used for
this comparison) also take into account momentum dependent two-loop 
contributions~\cite{Borowka:2014wla, Degrassi:2014pfa} 
and improved resummations of large logarithmic
corrections~\cite{Bahl:2016brp}. These updates are not relevant for the
comparison between the two codes up to \order{\alt\als}.}%
,
%
\begin{subequations}
 \label{eq:SEapprox}
 \begin{align}
 \NC:\
 &\mathbf{\hat{\Sigma}}_{hh}^{\tt NC}{\left(k^2\right)}
 =
 \left.
 \mathbf{\hat{\Sigma}}^{(\text{1L})}_{hh}{\left(k^2\right)}
 \right|^{\text{NMSSM}} +
 \left.
 \mathbf{\hat{\Sigma}}^{(\text{2L})}_{hh}{\left(k^2\right)}
 \right|_{k^2=0}^{\text{NMSSM }\order{\alt\als}},
 \\
 \FH:\
 &\mathbf{\hat{\Sigma}}_{hh}^{\FH}{\left(k^2\right)}
 =
 \left.
 \mathbf{\hat{\Sigma}}^{(\text{1L})}_{hh}{\left(k^2\right)}
 \right|^{\text{NMSSM}} +
 \Big[
 \left.\mathbf{\hat{\Sigma}}^{(\text{2L})}_{hh}{\left(k^2\right)}
 \right|^{\order{\alt\als}}+
 \order{\alt^2,\alb\als,\alt\alb}
 \nonumber\\
 & \mbox{}\hspace{80mm} + \mbox{resummed logs} \Big]_{k^2=0}^{\text{MSSM}}.
 \end{align}
\end{subequations}
\noindent
In order to facilitate the comparison between \NC\ and \NFH\ we
only include the MSSM corrections of \order{\alt\als}
in \NFH, if not stated otherwise.

The mixing matrix elements including higher-order corrections are denoted by
\ZH{ij}. They are given by the unitary matrices that diagonalise the
mass-matrix at the tree-level, $\mathbf{U}_{e(0)}$, and the 
loop-corrected mass matrix for zero external momentum,
$\mathbf{U}_{e(1)}$,
%
\begin{align}
  \mathbf{U^{h}} = \mathbf{U}_{e(1)} \mathbf{U}_{e(0)},
\label{Uh}
\end{align}
\noindent
where
%
\begin{align}
  {\rm diag}{\left(M^2_{h_1}, M^2_{h_2}, M^2_{h_3}\right)}
  =
  \mathbf{U}_{e(1)}
  \left[{\rm diag}{\left(m^2_{h_1}, m^2_{h_2}, m^2_{h_3}\right)} + \mathbf{\hat{\Sigma}}_{hh}{\left(p^2=0\right)}\right]
  \mathbf{U}_{e(1)}^\dagger.
\end{align}
%
Here the  capital $m_{h_i}$ and $M_{h_i}$ denote the Higgs-boson masses at
the tree-level and at the higher order, respectively.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Renormalisation Scheme: Higgs- and electroweak sectors}
\label{sec:RenSchemeHEW}

The independent parameters appearing in  the linear and bilinear terms
of the Higgs potential in  \refeq{eq:HiggsPot} have to be renormalised
in  order  to evaluate  higher-order  corrections  to the  Higgs-boson
masses.  \NC\  and  \FH\  offer  different  choices  for  the  set  of
independent    parameters    and     the    applied    renormalisation
schemes. \htC{[Reference to explanation.]}  For the presented work the
set  of common  independent parameters  in  the Higgs  sector for  the
comparison of the \DRbar/on-shell versions of both codes reads
%
\begin{align}
 \underbrace{\MZ,\ \MW,\ \MHp, T_{\phi_{\{1,2,s\}}}}_{\text{on-shell}}, 
\underbrace{\TB,\ \lambda,\ \mueff,\ \kappa,\ \Ak}_{\DRbar},
\end{align}
\noindent
with the applied renormalisation scheme. In \NC\ the scheme can
be varied: If $\MHp$ is set as input parameter, it will be
renormalised OS, if instead the trilinear soft-SUSY breaking
parameter $A_{\lambda}$ is used as input parameter it is
renormalised $\DRbar$.
The gauge-boson masses, however,
are still renormalised OS and the tadpole coefficients are
renormalised to vanish.

Using the former option, $\MHp$ as input, up to the one-loop
level the two codes differ only by their treatment of the
renormalisation of the coupling constant $\alpha$ in the
electromagnetic sector. While for \NC\ $\alpha$ is renormalised to
$\alpha(\MZ)$, \FH\ employs a dependent renormalisation scheme
(employing a \DRbar\ renormalization of $v$) with a subsequent
reparametrisation~\cite{Drechsel:2016jdg} to the value $\alpha_{G_F}$,
derived from the Fermi constant $G_F$ (to match exactly the MSSM
evaluation). In the Higgs-boson mass calculation in the
MSSM-limit the charge renormalisation constant drops out at the
discussed levels of the calculation and thus its impact is an effect
genuine to the NMSSM. The differences between \NC\ and \FH\ in
the higher-order contribution to the Higgs-boson self-energies
at the one-loop level are summarized in the upper row
of~\refta{tab:DiffNcNfhVanilla}.

\begin{table}[h]
 \centering
 \begin{tabular}{lcccc}
 & \NC & & \NFH
 \\\toprule
 \multirow{2}{*}{1-loop} & 
 $\alpha{\left(M_Z\right)}$ & \multirow{2}{*}{$\leftrightarrow$} & $\alpha_{G_F}$
 \\
 & renormalised & & reparametrised
 \\
 \midrule
 \multirow{2}{*}{2-loop} & 
 $\als^{\DRbar}\left(Q_{\rm input}\right)$ & 
 $\leftrightarrow$ &
 $\als^{\MSbar}\left(\mt\right)$ 
 \\
 &
 \multirow{2}{*}{NMSSM \order{\alt\als}} &
 \multirow{2}{*}{$\leftrightarrow$} &
 MSSM \order{\alt\als, \alt^2, \alb\als, \alt\alb}
 \\
 & & &
 + resummed logarithms
 \\\bottomrule
 \end{tabular}
 \caption{Calculational differences between the original (vanilla)
 versions of \NC\ and \NFH\ as used for this comparison. The used
 values for the electromagnetic and strong couplings is stated,
 where $\alpha_{G_F}$ denotes the electromagnetic coupling constant
 calculated from the Fermi constant.}
 \label{tab:DiffNcNfhVanilla}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Renormalisation Scheme: top/stop Sector}
\label{sec:RenSchemeTST}

\noindent
For the two-loop \order{\alt\als} corrections the top quark mass and
the stop parameters need to be renormalised.  
In \NC\ either  the OS  or the  \DRbar\ renormalisation  scheme for  the
top/stop sector can be used. Apart from section~\ref{sec:DRbar}, where
we indicate explicitly the renormalisation scheme of the top/stop sector,
we employ the OS scheme in \NC\ throughout this work.  
\par
The set of independent input parameters is chosen to be 
\begin{equation}
  \mt, \; \msqd,\; \mstop{R}, \text{ and } \;\At\,,
  \label{eq:stopsectren}
\end{equation}
where $\mt$ denotes the top quark mass, $\msqd$ and $\mstop{R}$ 
the soft-SUSY breaking masses of left-handed and right-handed fields, respectively, and $\At$
is the soft SUSY-breaking trilinear coupling of the stop sector. The counterterms can be found
in ref.~\cite{Muhlleitner:2014vsa}. 
No additional counterterms of the sbottom sector are needed since the bottom mass is set to zero in the charged Higgs self-energies.

\NFH\ uses the OS renormalisation scheme
\htSH{in the top/stop sector}, details can be found in
\htSH{refs.~\cite{Heinemeyer:2007aq,Degrassi:2001yf}}. Even though 
the renormalization scheme of
\htSH{refs.~\cite{Heinemeyer:2007aq,Degrassi:2001yf}}  uses the mixing
angle of the stops and the stop masses as input parameter, 
the schemes of ref.~\cite{Muhlleitner:2014vsa} and
\htSH{refs.~\cite{Heinemeyer:2007aq,Degrassi:2001yf}} are equivalent.
\htC{SH: Heidi, kannst du das checken? Mehr Details?}

 

%% \htPD{ For the top- and stop-sector the renormalisation transformation
%%   of  the top-  and stop-masses  together with  the stop-mixing  angle
%%   $\theta_{\tilde{t}}$ read
%% %
%% \begin{align}
%%   m_t \rightarrow m_t + \delta{m_t}
%%   ,\quad
%%   m^2_{\tilde{t}_i} \rightarrow m^2_{\tilde{t}_i} + \delta{m^2_{\tilde{t}_i}}
%%   ,\quad
%%   \theta_{\tilde{t}} \rightarrow \theta_{\tilde{t}} + \delta{\theta_{\tilde{t}}}.
%% \end{align}
%% \noindent
%% The     mass     counterterms     are     obtained     by     on-shell
%% renormalisation-conditions as described in sec.~\ref{sec:OSscheme},
%% %
%% \begin{align}
%%   \delta{m_t^{\text{OS}}}
%%   % \frac{1}{2} \text{Re}\left[\Sigma_{\psi\psi}{\left(p^2\right)}\right]_{\slashed{p}=m_t}
%%   ={}&\frac{1}{2} 
%%   \text{Re}\left[
%%     \Sigma^{(\slashed{p},L)}_{tt}{\left(p\right)} + 
%%     \Sigma^{(\slashed{p},R)}_{tt}{\left(p\right)} +
%%     \Sigma^{(S,L)}_{tt}{\left(p\right)} +
%%     \Sigma^{(S,R)}_{tt}{\left(p\right)}
%%   \right]_{\slashed{p}=m_t}
%%   \\
%%   \delta{m_{\tilde{t}_i}^{2,\text{OS}}}
%%   ={}&\text{Re}
%%   \Sigma_{\tilde{t}_i\tilde{t}_i}{\left(m_{\tilde{t}_i}^2\right)},
%% \end{align}
%% \noindent
%% while the counterterm for the mixing angle reads
%% %
%% \begin{align}
%%   \delta{\theta_{\tilde{t}}}
%%   =
%%   \frac{1}{2} 
%%   \frac{\text{Re}\left[
%%       \Sigma_{\tilde{t}_1 \tilde{t}_2}{\left(m^2_{\tilde{t}_1}\right)}
%%       - \Sigma_{\tilde{t}_1 \tilde{t}_2}{\left(m^2_{\tilde{t}_2}\right)}
%%       \right]
%%   }{
%%     m^2_{\tilde{t}_1} - m^2_{\tilde{t}_2}
%%   }.
%% \end{align}
%% \noindent
%% The finite shifts for the conversion between the $\DRbar$ and on-shell
%% scheme for the  top-quark and stop-squark masses and  the mixing angle
%% are  given   by  the  finite  contributions   of  the  renormalisation
%% constants,
%% %
%% \begin{align}
%%   \Delta{m_t} = \delta{m_t^{\rm OS}} - \delta{m_t^{\DRbar}}
%%   ,\quad
%%   \Delta{m^2_{\tilde{t}_i}} = \delta{m^2_{\tilde{t}_i^{\rm OS}}} - \delta{m^2_{\tilde{t}_i^{\DRbar}}}
%%   ,\quad
%%   \Delta{\theta_{\tilde{t}}} = \delta{\theta_{\tilde{t}}^{\rm OS}} - \delta{\theta_{\tilde{t}}^{\DRbar}}
%% \end{align}
%% \noindent
%% Thus  the  finite  shifts  for  the conversion  of  the  soft-breaking
%% parameters    of   the    stop-sector,   $M_{\tilde{t}_{\text{L}}}^2$,
%% $M_{\tilde{t_{\rm R}}}^2$  and  $A_t$,  from  the  $\DRbar$  scheme  into  the
%% on-shell scheme for the top-quark  and stop-squark masses in the NMSSM
%% with real parameters read
%% %
%% \begin{subequations}
%% \begin{align}
%%   \begin{split}
%%     \Delta{M_{\tilde{t}_{\text{L}}}^2}
%%     % ={}&\delta{M_{\tilde{t}_{\text{L}}}^{2, \text{OS}}} - \delta{M_{\tilde{t}_{\text{L}}}^{2, \DRbar}}
%%     % \\
%%     ={}&\left(\mathbf{U}_{\tilde{f}}\right)_{11}^2 \Delta{m_{\tilde{t}_1}^2} +
%%     \left(\mathbf{U}_{\tilde{f}}\right)_{12}^2 \Delta{m_{\tilde{t}_2}^2} -
%%     2\frac{
%%       \left(\mathbf{U}_{\tilde{f}}\right)_{12}\left(\mathbf{U}_{\tilde{f}}\right)_{22}
%%     }{
%%       m^2_{\tilde{t}_1} - m^2_{\tilde{t}_2}
%%     }\ \Delta{\theta_{\tilde{t}}} - 2 m_t \Delta{m_t}
%%   \end{split}
%%   \\
%%   \begin{split}
%%     \Delta{M_{\tilde{t}_{\rm R}}^2}
%%     % ={}&\Delta{M_{\tilde{t}}^{2, \text{OS}}} - \Delta{M_{\tilde{t}}^{2, \DRbar}}
%%     % \\
%%     ={}&\left(\mathbf{U}_{\tilde{f}}\right)_{21}^2 \Delta{m_{\tilde{t}_1}^2} +
%%     \left(\mathbf{U}_{\tilde{f}}\right)_{22}^2 \Delta{m_{\tilde{t}_2}^2} -
%%     2\frac{
%%       \left(\mathbf{U}_{\tilde{f}}\right)_{11}\left(\mathbf{U}_{\tilde{f}}\right)_{21}
%%     }{
%%       m^2_{\tilde{t}_1} - m^2_{\tilde{t}_2}
%%     }\ \Delta{\theta_{\tilde{t}}} - 2 m_t \Delta{m_t}
%%   \end{split}
%%   \\
%%   \begin{split}
%%     \Delta{A_t}
%%     % ={}&\Delta{A_t^{\text{OS}}} - \Delta{A_t^{\DRbar}}
%%     % \\
%%     ={}&\frac{1}{m_t}
%%     \left[
%%       \left(\mathbf{U}_{\tilde{f}}\right)_{11}\left(\mathbf{U}_{\tilde{f}}\right)_{12}
%%       \left(\Delta{m_{\tilde{t}_1}^2} - \Delta{m_{\tilde{t}_2}^2}\right) +
%%       \left(m^2_{\tilde{t}_1} - m^2_{\tilde{t}_2}\right)\Delta{\theta_{\tilde{t}}} -
%%       X_t \Delta{m_t}
%%       \right].
%%   \end{split}
%% \end{align}
%% \end{subequations}
%% \noindent
%% The  corrections  that  have  to  be included  in  the  top  and  stop
%% self-energies for the Higgs-mass calculation depends on the considered
%% two-loop   contributions.     If   only   two-loop    corrections   of
%% $\mathcal{O}{(\alpha_t\alpha_s)}$  are  considered,  only  corrections
%% from (S)QCD have to be considered.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Treatment of QCD corrections}

In \NC\ the $\DRbar$-value of the strong coupling constant
$\als^{\DRbar}$ is calculated at the input scale $Q$ of the
parameters specified in the SLHA input-file by applying the formulae given 
in~\cite{Chetyrkin:2000yt,Baer:2002ek}. In \NFH\ the
$\MSbar$-value of strong coupling constant $\als^{\MSbar}$ is
calculated at the scale $\mt$ independent of the input scale $Q$%
%
%\footnote{\htSH{This has partially be changed starting from version
% \texttt{2.12.1}.} \htC{MM: In which sense? And do you use it here
% then? This footnote is confusing.}}.%
%
~In both codes the obtained value is 
subsequently used for the calculation of the on-shell shift and the
evaluation of the two-loop contributions to the Higgs mass. As stressed above, 
\NC\ includes corrections up to \order{\alt\als}, and consequently for our
comparison we restrict the \NFH\ evaluation to this order as well.
The treatment of the two-loop contributions is summarized in the lower row of
\refta{tab:DiffNcNfhVanilla}. 
%\htC{MM: You describe here, what you have already given in Table~1. This is
%not good. You should first explain the differences in the 
%2loop calculations, as you do here. And then you should give the
%Table 1. Also, it would be good to comment in text on what you write
%in Table 1 on the corrections included in the codes at 2-loop leve.}




